A structured jet explains the extreme GRB 221009A

Long duration gamma-ray bursts (GRBs) are powerful cosmic explosions, signaling the death of massive stars. Among them, GRB 221009A is by far the brightest burst ever observed. Due to its enormous energy ($E_\textrm{iso}\!\approx$10$^{55}$ erg) and proximity ($z\!\approx$0.15), GRB 221009A is an exceptionally rare event that pushes the limits of our theories. We present multi-wavelength observations covering the first three months of its afterglow evolution. The X-ray brightness decays as a power-law with slope $\approx\!t^{-1.66}$, which is not consistent with standard predictions for jetted emission. We attribute this behavior to a shallow energy profile of the relativistic jet. A similar trend is observed in other energetic GRBs, suggesting that the most extreme explosions may be powered by structured jets launched by a common central engine.

==> GRB 221009A Science Format (Final Version) (1)/affiliations.tex <==
\begin{center}
    \scriptsize
    % \footnotesize
    \baselineskip24pt
    {$^{1}$ Department of Physics, The George Washington University, 725 21st Street NW, Washington, DC 20052, USA } \\ 
    {$^{2}$ Astronomy, Physics and Statistics Institute of Sciences (APSIS), Washington, DC 20052, USA }\\
    {$^{3}$ Department of Astronomy, University of Maryland, College Park, MD 20742-4111, USA }\\
    {$^{4}$ Astrophysics Science Division, NASA Goddard Space Flight Center, 8800 Greenbelt Rd, Greenbelt, MD 20771, USA }\\
    {$^{5}$ Department of Physics, University of Rome ``Tor Vergata'', via della Ricerca Scientifica 1, I-00133 Rome, Italy}\\
    {$^{6}$ INAF - Istituto di Astrofisica e Planetologia Spaziali, via Fosso del Cavaliere 100, 00133 Rome, Italy} \\
    {$^{7}$ Perimeter Institute for Theoretical Physics, 31 Caroline St. N., Waterloo, ON, N2L 2Y5, Canada }\\
    {$^{8}$ Department of Natural Sciences, The Open University of Israel, P.O Box 808, Ra’anana 4353701, Israel }\\
    {$^{9}$ Astrophysics Research Center of the Open university (ARCO), P.O Box 808, Ra’anana 4353701, Israel }\\
    {$^{10}$ Physics Department, University of Bath, Claverton Down, Bath BA2 7AY, United Kingdom}\\
    {$^{11}$ The Pennsylvania State University, 525 Davey Lab, University Park, PA 16802, USA} \\
    {$^{12}$ Istituto Nazionale di Ricerche Metrologiche, I-10135 Torino, Italy}\\
    {$^{13}$ INAF - Istituto di Radioastronomia, via Gobetti 101, I-40129 Bologna, Italy}\\
    {$^{14}$ Sternberg Astronomical Institute, Lomonosov Moscow State University, 119234, Universitetsky, 13, Moscow, Russia} \\
    {$^{15}$ Instituto de Radioastronom\'ia y Astrof\'isica, Universidad Nacional Aut\'onoma de M\'exico, Antigua Carretera } \\ 
    {a P\'atzcuaro $\#$ 8701, Ex-Hda. San Jos\'e de la Huerta, Morelia, Michoac\'an, C.P. 58089, M\'exico } \\
    {$^{16}$ Division of Physics, Mathematics and Astronomy, California Institute of Technology, Pasadena, CA 91125, USA}\\
    {$^{17}$ Joint Space-Science Institute, University of Maryland, College Park, MD 20742, USA}\\
    {$^{18}$ Instituto de Ciencias Nucleares, Universidad Nacional Aut\'onoma de M\'exico, %Apartado Postal 70-264, 
    04510 M\'exico, CDMX, Mexico}\\
    {$^{19}$ Department of Astronomy, University of Cape Town, Private Bag X3, Rondebosch 7701, South Africa}\\
    {$^{20}$ South African Astronomical Observatory, PO Box 9, 7935 Observatory, Cape Town, South Africa}\\
    {$^{21}$ School of Earth and Space Exploration, Arizona State University, Tempe, AZ 85287, USA }\\
    {$^{22}$ Observatorio Astronomico Felix Aguilar (OAFA), %Avda Benavides 8175, Rivadavia, El Leonsito, 
    San Juan 5400, Argentina} \\
    {$^{23}$ Facultad de Ciencias Exactas Fisicas y Naturales, San Juan National University, San Juan 5400, Argentina}\\
    {$^{24}$ Instituto de Astronom\'ia, Universidad Nacional Aut\'onoma de M\'exico, 04510 M\'exico, CDMX, Mexico }\\
    {$^\dagger$ Neil Gehrels Fellow}\\
    {$^\ast$Correspondence to: oconnorb@gwmail.gwu.edu, eleonora.troja@uniroma2.it}
\end{center}


==> GRB 221009A Science Format (Final Version) (1)/authors.tex <==




% \author{
% B. O'Connor$^{1,2,3,4\ast}$, 
% E. Troja$^{5,6}$, 
% G. Ryan$^{7}$,
% P. Beniamini$^{8,9}$,
% H. van Eerten$^{10}$, \\
% J. Granot$^{8,9,1}$,
% S. Dichiara$^{11}$,
% R. Ricci$^{12,13}$,
% V. Lipunov$^{14}$, \\
% J. Gillanders$^{5}$, 
% R. Gill$^{15}$,
% M. Moss$^{1}$,
% S. Anand$^{16}$, \\
% I. Andreoni$^{4,17}$, 
% R. L. Becerra$^{18}$,
% D. A. H. Buckley$^{19}$,
% N. R. Butler$^{20}$, \\
% S. B. Cenko$^{4,17}$, 
%  A. Chasovnikov$^{14}$, 
% J. Durbak$^{3,4}$,
% C. Francile$^{21,22}$,  \\
% E. Hammerstein$^{3}$,
% A. J. van der Horst$^{1}$,
% M. Kasliwal$^{16}$, \\
% C. Kouveliotou$^{1,2}$,
% A. S. Kutyrev$^{3,4}$,
% W. H. Lee$^{23}$, \\
% G. Srinivasaragavan$^{3}$,
% V. Topolev$^{14}$,
% A. M. Watson$^{23}$,
% K. Zhirkov$^{14}$ \\ 
% \\
% \footnotesize{$^{1}$ Department of Physics, The George Washington University, 725 21st Street NW, Washington, DC 20052, USA } \\ 
% \footnotesize{$^{2}$ Astronomy, Physics and Statistics Institute of Sciences (APSIS), The George Washington University, Washington, DC 20052, USA }\\
% \footnotesize{$^{3}$ Department of Astronomy, University of Maryland, College Park, MD 20742-4111, USA }\\
% \footnotesize{$^{4}$ Astrophysics Science Division, NASA Goddard Space Flight Center, 8800 Greenbelt Rd, Greenbelt, MD 20771, USA }\\
% \footnotesize{$^{5}$ Department of Physics, University of Rome - Tor Vergata, via della Ricerca Scientifica 1, 00100 Rome, IT }\\
% \footnotesize{$^{6}$ \textcolor{red}{INAF} }\\
% \footnotesize{$^{7}$ Perimeter Institute for Theoretical Physics, 31 Caroline St. N., Waterloo, ON, N2L 2Y5, Canada }\\
% \footnotesize{$^{8}$ Department of Natural Sciences, The Open University of Israel, P.O Box 808, Ra’anana 4353701, Israel }\\
% \footnotesize{$^{9}$ Astrophysics Research Center of the Open university (ARCO), The Open University of Israel, P.O Box 808, Ra’anana 4353701, Israel }\\
% \footnotesize{$^{10}$ Physics Department, University of Bath, Claverton Down, Bath BA2 7AY, United Kingdom}\\
% \footnotesize{$^{11}$ Department of Astronomy and Astrophysics, The Pennsylvania State University, 525 Davey Lab, University Park, PA 16802, USA} \\
% \footnotesize{$^{12}$ Istituto Nazionale di Ricerche Metrologiche, I-10135 Torino, Italy}\\
% \footnotesize{$^{13}$ INAF-Istituto di Radioastronomia, via Gobetti 101, I-40129 Bologna, Italy}\\
% \footnotesize{$^{14}$ Department of Physics, Sternberg Astronomical Institute, Lomonosov Moscow State University, 119234, Universitetsky, 13, Moscow, Russia} \\
% \footnotesize{$^{15}$ Instituto de Radioastronom\'ia y Astrof\'isica, Universidad Nacional Aut\'onoma de M\'exico, Antigua Carretera a P\'atzcuaro} \\ \footnotesize{$\#$ 8701, Ex-Hda. San Jos\'e de la Huerta, Morelia, Michoac\'an, C.P. 58089, M\'exico } \\
% \footnotesize{$^{16}$ Division of Physics, Mathematics and Astronomy, California Institute of Technology, Pasadena, CA 91125, USA}\\
% \footnotesize{$^{17}$ Joint Space-Science Institute, University of Maryland, College Park, MD 20742, USA}\\
% \footnotesize{$^{18}$ Instituto de Ciencias Nucleares, Universidad Nacional Aut\'onoma de M\'exico, Apartado Postal 70-264, 04510 M\'exico, CDMX, Mexico }\\
% \footnotesize{$^{19}$ South African Astrophysical Observatory, PO Box 9, 7935 Observatory, Cape Town, South Africa}\\
% \footnotesize{$^{20}$ School of Earth and Space Exploration, Arizona State University, Tempe, AZ 85287, USA }\\
% \footnotesize{$^{21}$ Observatorio Astronomico Felix Aguilar (OAFA), Avda Benavides 8175, Rivadavia, El Leonsito, San Juan 5400, Argentina} \\
% \footnotesize{$^{22}$ Facultad de Ciencias Exactas Fisicas y Naturales, San Juan National University, Casilla de Correo 49, San Juan 5400, Argentina}\\
% \footnotesize{$^{23}$ Instituto de Astronom\'ia, Universidad Nacional Aut\'onoma de M\'exico, Apartado Postal 70-264, 04510 M\'exico, CDMX, Mexico }\\
% \footnotesize{$^\ast$Correspondence to: oconnorb@gwmail.gwu.edu}
% }


% \author{
% B. O'Connor$^{1,2,3,4\ast}$, 
% E. Troja$^{5,6}$, 
% G. Ryan$^{7}$,
% P. Beniamini$^{8,9}$,
% H. van Eerten$^{10}$, \\
% J. Granot$^{8,9,1}$, 
% S. Dichiara$^{11}$,
% R. Ricci$^{12,13}$,
% V. Lipunov$^{14}$, 
% J. Gillanders$^{5}$, 
% R. Gill$^{15}$, \\
% M. Moss$^{1}$, 
% S. Anand$^{16}$, 
% I. Andreoni$^{4,17}$, 
% R. L. Becerra$^{18}$, 
% D. A. H. Buckley$^{19}$,\\
% N. R. Butler$^{20}$, 
% S. B. Cenko$^{4,17}$, 
%  A. Chasovnikov$^{14}$, 
% J. Durbak$^{3,4}$, 
% C. Francile$^{21,22}$,   \\
% E. Hammerstein$^{3}$,
% A. J. van der Horst$^{1}$,
% M. Kasliwal$^{16}$, 
% C. Kouveliotou$^{1,2}$, \\
% A. S. Kutyrev$^{3,4}$,  
% W. H. Lee$^{23}$, 
% G. Srinivasaragavan$^{3}$, 
% V. Topolev$^{14}$, \\
% A. M. Watson$^{23}$,
% K. Zhirkov$^{14}$ \\
% \\
% \scriptsize{$^{1}$ Department of Physics, The George Washington University, 725 21st Street NW, Washington, DC 20052, USA } \\ 
% \scriptsize{$^{2}$ Astronomy, Physics and Statistics Institute of Sciences (APSIS), Washington, DC 20052, USA }\\
% \scriptsize{$^{3}$ Department of Astronomy, University of Maryland, College Park, MD 20742-4111, USA }\\
% \scriptsize{$^{4}$ Astrophysics Science Division, NASA Goddard Space Flight Center, 8800 Greenbelt Rd, Greenbelt, MD 20771, USA }\\
% \scriptsize{$^{5}$ Department of Physics, University of Rome - Tor Vergata, via della Ricerca Scientifica 1, 00100 Rome, IT }\\
% \scriptsize{$^{6}$ INAF - Istituto di Astrofisica e Planetologia Spaziali, via Fosso del Cavaliere 100, 00133 Rome, Italy} \\
% \scriptsize{$^{7}$ Perimeter Institute for Theoretical Physics, 31 Caroline St. N., Waterloo, ON, N2L 2Y5, Canada }\\
% \scriptsize{$^{8}$ Department of Natural Sciences, The Open University of Israel, P.O Box 808, Ra’anana 4353701, Israel }\\
% \scriptsize{$^{9}$ Astrophysics Research Center of the Open university (ARCO), P.O Box 808, Ra’anana 4353701, Israel }\\
% \scriptsize{$^{10}$ Physics Department, University of Bath, Claverton Down, Bath BA2 7AY, United Kingdom}\\
% \scriptsize{$^{11}$ The Pennsylvania State University, 525 Davey Lab, University Park, PA 16802, USA} \\
% \scriptsize{$^{12}$ Istituto Nazionale di Ricerche Metrologiche, I-10135 Torino, Italy}\\
% \scriptsize{$^{13}$ INAF - Istituto di Radioastronomia, via Gobetti 101, I-40129 Bologna, Italy}\\
% \scriptsize{$^{14}$ Sternberg Astronomical Institute, Lomonosov Moscow State University, 119234, Universitetsky, 13, Moscow, Russia} \\
% \scriptsize{$^{15}$ Instituto de Radioastronom\'ia y Astrof\'isica, Universidad Nacional Aut\'onoma de M\'exico, Antigua Carretera } \\ 
% \scriptsize{a P\'atzcuaro $\#$ 8701, Ex-Hda. San Jos\'e de la Huerta, Morelia, Michoac\'an, C.P. 58089, M\'exico } \\
% \scriptsize{$^{16}$ Division of Physics, Mathematics and Astronomy, California Institute of Technology, Pasadena, CA 91125, USA}\\
% \scriptsize{$^{17}$ Joint Space-Science Institute, University of Maryland, College Park, MD 20742, USA}\\
% \scriptsize{$^{18}$ Instituto de Ciencias Nucleares, Universidad Nacional Aut\'onoma de M\'exico, %Apartado Postal 70-264, 
% 04510 M\'exico, CDMX, Mexico}\\
% \scriptsize{$^{19}$ South African Astrophysical Observatory, PO Box 9, 7935 Observatory, Cape Town, South Africa}\\
% \scriptsize{$^{20}$ School of Earth and Space Exploration, Arizona State University, Tempe, AZ 85287, USA }\\
% \scriptsize{$^{21}$ Observatorio Astronomico Felix Aguilar (OAFA), %Avda Benavides 8175, Rivadavia, El Leonsito, 
% San Juan 5400, Argentina} \\
% \scriptsize{$^{22}$ Facultad de Ciencias Exactas Fisicas y Naturales, San Juan National University, San Juan 5400, Argentina}\\
% \scriptsize{$^{23}$ Instituto de Astronom\'ia, Universidad Nacional Aut\'onoma de M\'exico, 04510 M\'exico, CDMX, Mexico }\\
% \scriptsize{$^\ast$Correspondence to: oconnorb@gwmail.gwu.edu}
% }



==> GRB 221009A Science Format (Final Version) (1)/custom-acronyms.tex <==

\newcommand\aj{AJ}%        % Astronomical Journal 
\newcommand\psj{PSJ}%       % Planetary Science Journal
\newcommand\araa{ARA\&A}%  % Annual Review of Astron and Astrophys 
\newcommand\apj{ApJ}%    % Astrophysical Journal 
\newcommand\apjl{ApJL}     % Astrophysical Journal, Letters 
\newcommand\apjs{ApJS}%    % Astrophysical Journal, Supplement 
\newcommand\ao{ApOpt}%   % Applied Optics 
\newcommand\apss{Ap\&SS}%  % Astrophysics and Space Science 
\newcommand\aap{A\&A}%     % Astronomy and Astrophysics 
\newcommand\aapr{A\&A~Rv}%  % Astronomy and Astrophysics Reviews 
\newcommand\aaps{A\&AS}%    % Astronomy and Astrophysics, Supplement 
\newcommand\azh{AZh}%       % Astronomicheskii Zhurnal 
\newcommand\baas{BAAS}%     % Bulletin of the AAS 
\newcommand\icarus{Icarus}% % Icarus
\newcommand\jaavso{JAAVSO}  % The Journal of the American Association of Variable Star Observers
\newcommand\jrasc{JRASC}%   % Journal of the RAS of Canada 
\newcommand\memras{MmRAS}%  % Memoirs of the RAS 
\newcommand\mnras{MNRAS}%   % Monthly Notices of the RAS 
\newcommand\pra{PhRvA}% % Physical Review A: General Physics 
\newcommand\prb{PhRvB}% % Physical Review B: Solid State 
\newcommand\prc{PhRvC}% % Physical Review C 
\newcommand\prd{PhRvD}% % Physical Review D 
\newcommand\pre{PhRvE}% % Physical Review E 
\newcommand\prl{PhRvL}% % Physical Review Letters 
\newcommand\pasp{PASP}%     % Publications of the ASP 
\newcommand\pasj{PASJ}%     % Publications of the ASJ 
\newcommand\qjras{QJRAS}%   % Quarterly Journal of the RAS 
\newcommand\skytel{S\&T}%   % Sky and Telescope 
\newcommand\solphys{SoPh}% % Solar Physics 
\newcommand\sovast{Soviet~Ast.}% % Soviet Astronomy 
\newcommand\ssr{SSRv}% % Space Science Reviews 
\newcommand\zap{ZA}%       % Zeitschrift fuer Astrophysik 
\newcommand\nat{Nature}%  % Nature 
\newcommand\iaucirc{IAUC}% % IAU Cirulars 
\newcommand\aplett{Astrophys.~Lett.}%  % Astrophysics Letters 
\newcommand\apspr{Astrophys.~Space~Phys.~Res.}% % Astrophysics Space Physics Research 
\newcommand\bain{BAN}% % Bulletin Astronomical Institute of the Netherlands 
\newcommand\fcp{FCPh}%   % Fundamental Cosmic Physics 
\newcommand\gca{GeoCoA}% % Geochimica Cosmochimica Acta 
\newcommand\grl{Geophys.~Res.~Lett.}%  % Geophysics Research Letters 
\newcommand\jcp{JChPh}%     % Journal of Chemical Physics 
\newcommand\jgr{J.~Geophys.~Res.}%     % Journal of Geophysics Research 
\newcommand\jqsrt{JQSRT}%   % Journal of Quantitiative Spectroscopy and Radiative Trasfer 
\newcommand\memsai{MmSAI}% % Mem. Societa Astronomica Italiana 
\newcommand\nphysa{NuPhA}%     % Nuclear Physics A 
\newcommand\physrep{PhR}%       % Physics Reports 
\newcommand\physscr{PhyS}%        % Physica Scripta 
\newcommand\planss{Planet.~Space~Sci.}%  % Planetary Space Science 
\newcommand\procspie{Proc.~SPIE}%      % Proceedings of the SPIE 
\newcommand\actaa{AcA}%  % Acta Astronomica
\newcommand\caa{ChA\&A}%  % Chinese Astronomy and Astrophysics
\newcommand\cjaa{ChJA\&A}%  % Chinese Journal of Astronomy and Astrophysics
\newcommand\jcap{JCAP}%  % Journal of Cosmology and Astroparticle Physics
\newcommand\na{NewA}%  % New Astronomy
\newcommand\nar{NewAR}%  % New Astronomy Review
\newcommand\pasa{PASA}%  % Publications of the Astron. Soc. of Australia
\newcommand\rmxaa{RMxAA}%  % Revista Mexicana de Astronomia y Astrofisica

%% added feb 9, 2016
\newcommand\maps{M\&PS}% Meteoritics and Planetary Science
\newcommand\aas{AAS Meeting Abstracts}% American Astronomical Society Meeting Abstracts
\newcommand\dps{AAS/DPS Meeting Abstracts}% American Astronomical Society/Division for Planetary Sciences Meeting Abstracts


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%% Some Useful Abbreviations %%%%% 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\cxo}{{\it Chandra~}}
\newcommand{\rxte}{{\it RXTE~}}
\newcommand{\asca}{{\it ASCA~}}
\newcommand{\rosat}{{\it ROSAT~}}
\newcommand{\einstein}{{\it EINSTEIN}}
\newcommand{\ginga}{{\it GINGA}}
\newcommand{\bbxrt}{{\it BBXRT}}
\newcommand{\suzaku}{{\it Suzaku}}
\newcommand{\xmm}{{\it XMM-Newton~}}
\newcommand{\sax}{{\it BeppoSAX}}
\newcommand{\ec}{$\eta$~Car}
\newcommand{\glast}{{\it GLAST}}
\newcommand{\swift}{{\it Swift~}}
\newcommand{\integral}{\textit{INTEGRAL~}}
\newcommand{\nustar}{\textit{NuSTAR~}}
\newcommand{\hst}{{\it HST}}
\newcommand{\ms}{$M_{\odot}$}
\newcommand{\rs}{$R_{\odot}$}
\newcommand{\ls}{$L_{\odot}$}
\newcommand{\kms}{km~s$^{-1}$}
\newcommand{\fluxcgs}{ergs~s$^{-1}$~cm$^{-2}$}
\newcommand{\lumcgs}{ergs~s$^{-1}$}
\def\gtrsim{\mathrel{\hbox{\rlap{\hbox{\lower4pt\hbox{$\sim$}}}\hbox{$>$}}}}

\def \arcsec {\hbox{$^{\prime\prime}$}}
\def\eg#1{\textcolor{red}{#1}}


==> GRB 221009A Science Format (Final Version) (1)/obs.tex <==

\noindent \textbf{Observations and Data Analysis} 

\noindent \textbf{\textit{X-ray Observations}} 

\noindent \textit{Swift} 

The \textit{Neil Gehrels Swift Observatory} X-ray Telescope (XRT) began settled observations of GRB 221009A at 14:13:30 UT on 2022-10-09, approximately 143 s after the \textit{Swift}/BAT trigger and 3198 s after the \textit{Fermi}/GBM trigger. The afterglow was clearly detected and localized to RA, DEC (J2000) = $19^{h}13^m 03^{s}.85$, $+\ang{19;46;22.7}$ with an accuracy of \ang{;;3.5} (90$\%$ confidence level) \cite{Evans2009}. 
We obtained the XRT lightcurve from the \textit{Swift}-XRT GRB Lightcurve Repository\footnote{\url{https://www.swift.ac.uk/xrt_curves/}}. The lightcurve has been shifted in time by 3198 s to apply the \textit{Fermi}/GBM trigger as $T_0$. 
We further used the XRT Repository tools to create time-sliced spectra, in both windowed timing (WT) and photon counting (PC) modes, at multiple epochs for use in modeling the broadband spectral energy distribution of the GRB afterglow. 

\noindent \textit{XMM-Newton} 

We observed GRB 221009A using \textit{XMM-Newton} on November 10, 2022 through Directory's Discretionary Time (DDT; PI: Troja), corresponding to 32.72 d after the GRB trigger. The observations were performed in full frame mode using the thin filter, and lasted for 100 ks with a mid-time of 32.72 d. The data were reduced and analyzed using tasks with the Science Analysis System (\texttt{SAS v18.0.0}) software. We used a circular region of $60\arcsec$ to extract source photons. The background photons were taken from a nearby source-free circular region of $60\arcsec$.  We grouped the spectrum to a minimum of 1 count per bin and obtained the response matrix and ancillary response files using the \texttt{rmfgen} and \texttt{arfgen} tasks. 

\noindent \textit{NuSTAR} 

\textit{NuSTAR} observed GRB 221009A on five epochs at mid-times of 1.82, 5.92, 10.72, 23.93, and 31.95 d after the \textit{Fermi} trigger (see Table \ref{tab:Xobservations}). These data were obtained under two DDT programs (co-PIs: Margutti and Racusin; PI: Troja). The initial observations were first reported by \cite{GCN32695,GCN32788}. \textit{NuSTAR} is comprised of two identical focal plane modules, FPMA and FPMB, covering the $3-79$ keV energy range. The GRB afterglow is detected in each epoch. We reduced the data using the \textit{NuSTAR} Data Analysis Software pipeline (\texttt{NuSTARDAS}) within \texttt{HEASoft v6.29c}. The data were processed using \texttt{nupipeline}, and then lightcurves and spectra were extracted using \texttt{nuproducts}. In the initial observation at 1.8 d, source spectra were extracted from a 100\arcsec{} radius region centered on the transient. The background was similarly extracted from a 100\arcsec{} radius source-free region. For each of the latter observations, we used a 60\arcsec{} radius for both source and background regions. 


\noindent \textbf{\textit{Optical/Near-Infrared Observations}}

\noindent \textit{MASTER}

MASTER is a system of wide-field fully robotic 40-cm telescopes with identical scientific equipment and real-time auto-detection at every observatory \cite{Lipunov2004,Lipunov2010,Kornilov2012}. The MASTER telescopes are MASTER-Amur, -Tunka, -Ural, -Kislovodsk, -Tavrida (Russia), -SAAO (South Africa), -IAC (Spain), -OAFA (Argentina). The MASTER Global Robotic Net \cite{Lipunov2010} began observing GRB 221009A using MASTER-SAAO on 2022-10-09 at 17:33:54 UT, corresponding to 0.18 d after the \textit{Fermi} trigger. The MASTER auto-detection system discovered the optical counterpart, MASTER OT J191303.43+194623.1 \cite{GCN32634}, as a transient in the initial image. The observations were obtained in the \textit{clear} ($C$) filter. Further observations were obtained with MASTER-OAF starting on 2022-10-09 at 23:56:38 UT, corresponding to 0.46 d after the trigger (see Table \ref{tab:MASTERobservations}). Aperture photometry was calibrated using 20 reference stars, and we applied a further correction to convert to the AB magnitude system. We note that earlier observations by MASTER-Tunka and MASTER-Amur, beginning at 93 s after the \textit{Fermi} trigger (2022-10-09 14:11:50 UT), were severely impacted by clouds and were unable to detect the source. 


\noindent \textit{COATLI}

We observed the field of GRB 221009A with the 50-cm COATLI telescope at the Observatorio Astronómico Nacional on the Sierra de San Pedro Mártir in Baja California, México, and the HUITZI f/8 imager. We observed in $griz$ filters similar to Pan-STARRS1 (hereafter PS1; \cite{Chambers2016}) and took multiple 30 second images each night. The images were reduced using a custom pipeline, and then stacked to create a final image. Photometry was calculated for each stack using PSF fitting and calibrated relative to the PS1 catalog using all available field stars.

\noindent \textit{Gemini}

Target of Opportunity (ToO) observations of GRB 221009A were performed with the 8.1-m Gemini South Telescope in Cerro Pachon, Chile using GMOS-S and Flamingos-2 (hereafter F2) under two DDT programs (GS-2022B-DD-104, PI: O'Connor; GS-2022B-DD-103, PI: Rastinejad). The observations were first reported by \cite{GCN32749,GCN32750,GCN32860}.
Data were obtained at 4.4, 17.4 and 25.4 d. The observations were carried out in the $i$ filter with GMOS-S, and $J$, $H$, and $K_s$ filters with F2 (see Table \ref{tab:Optobservations}). We reduced and analyzed these data using the \texttt{DRAGONS}\footnote{\url{https://dragons.readthedocs.io/}} software \cite{Labrie2019}. The afterglow is clearly detected in each observation. 
%\textcolor{purple}{Using the initial images, we localize the GRB to RA, DEC (J2000) = $19^{h}13^m 03^{s}.85$, $+\ang{19;46;22.7}$ with an accuracy of $XXX\arcsec$.} 
We performed PSF photometry using \texttt{SExtractor} \cite{Bertin1996} and \texttt{PSFEx} \cite{Bertin2013}. The photometry was calibrated using nearby point-sources in the Two Micron All Sky Survey (2MASS) catalog \cite{Skrutskie2006}. We then applied a standard conversion between the Vega and AB magnitude systems.

\noindent \textit{Lowell Discovery Telescope} 

We obtained ToO observations with the Large Monolithic Imager (LMI) mounted on the 4.3-meter LDT at the Lowell Observatory in Happy Jack, AZ starting at 3.6 d after the GRB and continuing observations for 8 weeks under multiple programs (program PIs: Cenko, Hammerstein, O'Connor), see Table \ref{tab:Optobservations}. We first reported the initial observations in \cite{GCN32739,GCN32799}. The data were reduced with a custom pipeline \cite{Toy2016} that makes use of standard CCD reduction techniques in the IRAF\footnote{IRAF is distributed by the National Optical Astronomy Observatory, which is operated by the Association of Universities for Research in Astronomy (AURA) under cooperative agreement with the National Science Foundation (NSF).} package including bias subtraction, flat-fielding, and cosmic ray rejection \cite{vanDokkum2001}. Photometry was performed in the same manner as for Gemini, and calibrated against stars in the PS1 catalog. % (Pan-STARRS1, hereafter PS1) \cite{Chambers2016}. 

\noindent \textit{Palomar 200-inch}

We obtained data with the Palomar 200-in Wide InfraRed Camera (WIRC) in the $J$, $H$, and $K_s$ bands starting at 18:26:50 UT on 2022-11-02, taking 9 dithered images in each band for a total exposure of 495 s in $J$ and 330 s in $H$ and $K_s$ (Table \ref{tab:Optobservations}). The data were reduced using a \texttt{Python}-based reduction pipeline that uses standard image reduction techniques \cite{De2020}. The dithered images in each filter were astrometrically aligned and stacked to create a single composite image. The pipeline performed photometric calibration using the 2MASS point source catalog. 


\noindent \textit{Other Optical and Near-Infrared Data} 


We analyzed publicly available \textit{HST} observations (PI: Levan) obtained in WFC3/UVIS $F625W$ and $F775W$ filters and WFC3/IR $F098M$, $F125W$, and $F160W$ filters. The data were reduced and analyzed as detailed in \cite{OConnor2022}. 

We further supplemented our dataset with optical and infrared observations reported in GCN circulars \cite{GCN.32769, GCN.32818, GCN.32684, GCN.32743, GCN.32752, GCN.32652, GCN.32755, GCN.32646, GCN.32804, GCN.32678, GCN.32811, GCN.32758, GCN.32803, GCN32765hostz, GCN.32670,GCN.32662, GCN.32852, GCN.32795, GCN.32809, GCN.32753,GCN.32771, GCN.32756, GCN.32709}. 

%\textit{HST} observations were carried out at 29.7, 40.6, and 55.7 d after the GRB trigger (see Table \ref{tab:Optobservations}). Data were acquired in the WFC3/UVIS $F625W$ and $F775W$ filters and WFC3/IR $F098M$, $F125W$, and $F160W$ filters through a DDT request (PI: Levan). The initial observation was first reported by \cite{GCN32921}. 
%We reduced the data using standard procedures within the \texttt{DrizzlePac} package \cite{Gonzaga2012}. The source is clearly detected in all filters with a marginal extension of the source to the NE in the infrared filters, likely due to the underlying host galaxy at $z=0.1505$. The galaxy is not identified in the initial WFC3/UVIS images, likely due to extinction from the Milky Way, but is found in the deep $F625W$ images from 2022 December 4. %\textcolor{purple}{Based on these \textit{HST} images we derive a more precise localization of the GRB to RA, DEC = XXX....}. 
%We performed photometry of the source complex using a circular region of radius $0.3\arcsec$ centered on the transient. The zeropoints were taken from the photometry keywords in the image headers. %These measurements include the unknown host contribution. 



\noindent \textit{\textbf{Radio Observations}}

The Australia Telescope Compact Array (ATCA) observed GRB 221009A as part of the DDT project CX515 on 2022-10-15, 2022-10-24, 2022-11-04, 2022-11-19, 2022-12-28, and 2023-01-27 (Table \ref{tab:Radioobservations}). The initial observation at 5.8 d after the GRB was first reported by \cite{GCN32763,GCN32766}. In the first two epochs, the three pairs of Intermediate Frequencies (IFs) were used 16.7/21.2 GHz, 33/35 GHz, 45/47 GHz and in the next two only 16.7/21.2 GHz and 33/35 GHz were used. In the last two epochs, corresponding to 80 and 110 d after the GRB, observations were obtained at 5.5 and 9 GHz. In all observing runs the array operated in continuum mode with the Compact Array Broadband Backend using 2048 channels over 2-GHz bandwidth per IF. The radio sources used as bandpass, primary and phase calibrator were 1921-293, 1934-638 and 1923+210, respectively. The phase calibrator was also used for reference pointing checks every hour. Standard procedures in the data reduction software package \texttt{MIRIAD}
% (\textcolor{red}{CITE})
\cite{Sault1995_MIRIAD}
were used to flag, calibrate the complex gains and image the phase calibrator and target. A robustness parameter value of two was used, and a 6-km baseline antenna was deselected during imaging.

We further used the \texttt{MIRIAD} task \texttt{calred} on the phase calibrator 1923+210 to test for phase decorrelation due to atmospheric turbulence. The task \texttt{calred} estimates the triple product amplitude, and, therefore, is unaffected by atmospheric turbulence induced phase decorrelation effects. A comparison between triple product and map flux density can be used to estimate the decorrelation factor. We found no significant decorrelation in the flux densities measured on the I-stokes restored maps, apart from three frequencies (35, 45 and 47 GHz) in Epoch 2 (2022-10-24; 14.7 d post-burst) at a level of 19\%, 14\% and 12\% respectively and on Epoch 4 (2022-11-19; 41 d post-burst) at 33 and 35 GHz of 4\% and 3\%, respectively. 
Seeing monitor data show a maximum rms path length of 
$\approx$500 microns during our second epoch (14.7 d) which, for a calibration interval of 15 min, is expected to result in a 25-50\% amplitude decorrelation above 30 GHz. Due to the large uncertainties, we exclude this epoch from our spectral analysis. 
No significant decorrelation is expected for observations at frequencies below 10 GHz (e.g., 80 and 110 d). 

The resulting flux densities and 5$\sigma$ upper limits are presented in Table \ref{tab:Radioobservations}. The errors are derived from summing in quadrature the statistical and systematic uncertainty (map rms and 5\% of the total flux as residual of gain calibration, respectively).



We supplemented our radio observations with data reported in GCN circulars  \cite{GCN32653,GCN32655,GCN32949,GCN32676}. 


==> GRB 221009A Science Format (Final Version) (1)/oldapj.tex <==

\textcolor{purple}{Below are the contents of the ApJ Version as of 1/18/22.}

\begin{sciabstract}
 ABSTRACT GOES HERE
\end{sciabstract}

\section*{Introduction}
\label{sec: intro}


Gamma-ray bursts (GRBs) are among the peculiar and enigmatic phenomena in the universe. They consist of brief flashes of gamma-ray radiation detected by low orbit satellites with an all sky rate of about 1 or 2 events per day. Their fluence (flux integrated over the duration of the gamma-ray signal) ranges between few times $10^{-7}$ to $10^{-4}$ erg cm$^{-2}$ in the $10-1000$ keV energy band (as observed by Fermi/GBM; \cite{vonKienlin2020}).
They are grouped into two main sub-classes based on their duration and spectral hardness \cite{Kouveliotou1993}. Long duration GRBs (lasting $\gtrsim 2$ s) are produced by the core-collapse of rapidly-rotating massive stars (collapsars) \cite{Woosley2006}.
%\textcolor{purple}{Link supernova detections from nearby GRBs to how we know they are produced by massive-stars... no more than 1 sentence on environment/star forming regions...}


These explosions display a broad range of gamma-ray energy between $E_{\gamma,\textrm{iso}}=10^{48-54}$ erg. Due to their extreme energy, they are detectable by high-energy satellites in the early Universe ($z\approx 2-4$), with only the most energetic detectable further back in time. 

Despite the large number of GRBs detected so far, only few of them were observed at very high energies (VHE; $>$100 GeV): GRB 180720B \cite{Abdalla2019}, GRB 190114C \cite{Magic2019}, GRB 190829A \cite{Hess2021} and GRB 201216C
% (Blanch O. et al., 2020, GCN Circ., 29075, 1).
\cite{Blanch2020GCN}.
The study of this signal can provides key information about the nature of the emission and the radiative processes in play. %\textcolor{red}{(This paper states 201216C is the fith, so are we missing one? https://arxiv.org/pdf/2204.05811.pdf)}\textcolor{blue}{it really depends if you consider also 201015A or not. but that was reported as a tentative detection https://gcn.gsfc.nasa.gov/gcn3/28659.gcn3}

In this paper we present an analysis of the multi-wavelength observations obtained for the \textit{Swift} and \textit{Fermi} detected GRB 221009A. The combination of its close proximity ($z=0.1505$; \cite{GCN32648xshooterz}), and extreme energetics ($E_{\gamma,\textrm{iso}}\approx2\times 10^{54}$ erg, 10-1000 keV; \cite{GCN32642}) led to GRB 221009A being the brightest GRB ever observed in nearly 55 years of observations (with a measured fluence that is more than 1 orders of magnitude brighter than GRB 130427A, the second brightest event observed by \textit{Fermi} so far). In addition, GRB 221009A broke the record for highest energy photon detected from a GRB (18 TeV; \cite{GCN32677}), and is only the fifth GRB associated with very high energy (VHE; $>100$ GeV) photons \cite{Abdalla2019,Magic2019,Hess2021}. A claim of a 250 TeV photon-like air shower associated to this GRB was made Carpet-2 \cite{ATel15669}, but later refuted due to a coincident Galactic TeV source \cite{ATel15675}.

Nearby events represent a unique tool to probe theoretical models of multi-wavelength afterglow emission up to very high energy. The standard paradigm (e.g., fireball model; \cite{Rees1992}) features a forward shock (FS) that amplifies the magnetic field and accelerates the electrons in the shocked circumburst medium to a relativistic power-law energy distribution, which then cool via synchrotron radiation (e.g., \cite{Granot2002}. Unless the outflow is highly magnetized as it is decelerated by the external medium, this deceleration is mediated by a reverse shock (RS) that forms and travels back into the ejecta (e.g., \cite{Kobayashi2000}).

 %Inverse Compton (IC) effects should also be taken into account in the parametrization of these radiative processes in order to have a self consistent modeling (...). 
Low redshift events provide a unique probe of emission processes not detectable at larger distances.
In point of fact, inverse Compton (IC) could be recognized as the mechanism responsible for the VHE TeV emission in recent GRBs (e.g., \cite{Abdalla2019, Magic2019}). This component can only be seen at low redshift due to the effect of the extragalactic background scattering \cite{Franceschini2008, Dominguez2011, Gilmore2012, Finke2022}. The proximity of GRB 221009A combined with its outstanding brightness provide us with a once-in-a-lifetime opportunity to constrain the physics of the afterglow and the jet structure of a nearby collapsar GRB.

We present observations optical and infrared obtained with MASTER, the Lowell Discovery Telescope (LDT), Palomar 200-inch (P200), Gemini-South, \textit{Hubble Space Telescope} (\textit{HST}), X-ray observations with \textit{XMM-Newton} and \textit{NuSTAR}, and radio observations from the Australia Telescope Compact Array (ATCA). We interpret the observed multi-wavelength emission as originating from the combination of a reverse- and forward-shock (RS and FS, respectively).


The paper is outlined as follows: \textcolor{purple}{Fill in once we have a final structure of the paper...}

In this work, we adopt a standard $\Lambda$-CDM cosmology \cite{Planck18}. Confidence intervals are expressed at the $1\sigma$ level, and upper limits at $3\sigma$. We apply the convention $F_\nu\propto t^{\alpha}\nu^{\beta}$ throughout. 

\textcolor{purple}{Make sure FS, RS, OIR is all defined in the right place...}


\section{Observations and Data Reduction}
\label{sec: observations}

\subsection{Prompt gamma-rays}


GRB 221009A triggered \textit{Fermi} GBM \cite{GCN32636,GCN32642} and \textit{Fermi} LAT \cite{GCN32658}, among many other high-energy satellites (\textit{INTEGRAL}, \textit{Konus-Wind}, \textit{AGILE}, \textit{SRG}, \textit{GRBAlpha}) \cite{GCN32660,GCN32663,GCN32668, GCN32685, GCN32650} on 2022-10-09 at 13:16:59 UT (hereafter referred to as $T_0$). Due to an issue with the \textit{Fermi} automatic notice, the GRB was not identified until $\sim$ 1 hour later when, after exiting the SAA, \textit{Swift} BAT triggered on the afterglow \cite{GCN32632}. 

The GRB emission had a duration of a few hundred seconds, with multiple emission episodes. Due to the GRB's extreme brightness, the majority of satellites were saturated during the main emission episode. A lower limit to the GRB fluence was reported for \textit{Fermi} GBM as $\sim2.9\times 10^{-2}$ erg cm$^{-2}$ s$^{-1}$ in the 10-1000 keV energy band \cite{GCN32642}, \textit{Konus-Wind} reported $\sim5.2\times 10^{-2}$ erg cm$^{-2}$ s$^{-1}$ (20 keV - 10 MeV) \cite{GCN32668}, and \textit{INTEGRAL} determined $\sim1.3\times 10^{-2}$ erg cm$^{-2}$ s$^{-1}$ (75 keV - 1 MeV) \cite{GCN32660}. Despite these estimates being lower limits, this event is the brightest GRB ever detected by almost two orders of magnitude. At the putative redshift of $z=0.1505$ \cite{GCN32648xshooterz,GCN32686GTCz,GCN32765hostz}, these values correspond to an isotropic equivalent energy in the range $8\times 10^{53}$ erg (75 keV - 1 MeV) to $3\times 10^{54}$ erg (20 keV - 10 MeV), among a short list of the most energetic GRBs to date \cite{Atteia2017} and very similar to GRB 160625B \cite{Zhang2018}. 






\subsection{\textit{Swift}}
\label{sec: Swift}

The \textit{Swift} X-ray Telescope (XRT) began settled observations of GRB 221009A at 14:13:30 UT on 2022-10-09, approximately 143 s after the \textit{Swift}/BAT trigger and 3198 s after the \textit{Fermi}/GBM trigger. The afterglow was clearly detected and localized to RA, DEC (J2000) = $19^{h}13^m 03^{s}.85$, $+\ang{19;46;22.7}$ with an accuracy of \ang{;;3.5} (90$\%$ confidence level (CL)) \cite{Evans2009}. 
We obtained the XRT lightcurve from the \textit{Swift}-XRT GRB Lightcurve Repository\footnote{\url{https://www.swift.ac.uk/xrt_curves/}}. The lightcurve has been shifted in time by 3198 s to apply the \textit{Fermi}/GBM trigger as $T_0$. 
We further used the XRT Repository tools to create time-sliced spectra, in both windowed timing (WT) and photon counting (PC) modes, at multiple epochs for use in modeling the broadband spectral energy distribution (SED) of the GRB afterglow. 



\subsection{\textit{XMM-Newton}}
\label{sec: XMM}


%https://xmmweb.esac.esa.int/cgi-bin/xmmobs/public/obs_view.tcl?search_instrument=0&action=Get+Selection&search_obs_id=0913991901


We observed GRB 221009A using \textit{XMM-Newton} on November 10, 2022 through Directory's Discretionary Time (PI: Troja), corresponding to 32.72 d after the GRB trigger. The observations were performed in full frame mode using the thin filter, and lasted for 100 ks with a mid-time of 32.72 d. The data were reduced and analyzed using tasks with the Science Analysis System (\texttt{SAS v18.0.0}) software. We used a circular region of $60\arcsec$ to extract source photons. The background photons were taken from a nearby source-free circular region of $60\arcsec$.  We grouped the spectrum to a minimum of 1 count per bin and obtained the response matrix and ancillary response files using the \texttt{rmfgen} and \texttt{arfgen} tasks. 


\subsection{\textit{NuSTAR}}
\label{sec: nustar}


\textit{NuSTAR} observed GRB 221009A on five epochs at mid-times of 1.82, 5.92, 10.72, 23.93, and 31.95 d after the \textit{Fermi} trigger (see Table \ref{tab:Xobservations}). These data were obtained under two DDT programs (co-PIs: Margutti and Racusin; PI: Troja). The initial observations were first reported by \cite{GCN32695,GCN32788}. \textit{NuSTAR} is comprised of two identical focal plane modules, FPMA and FPMB, covering the $3-79$ keV energy range. The GRB afterglow is detected in each epoch. We reduced the data using the \textit{NuSTAR} Data Analysis Software pipeline (\texttt{NuSTARDAS}) within \texttt{HEASoft v6.29c}. The data were processed using \texttt{nupipeline}, and then lightcurves and spectra were extracted using \texttt{nuproducts}. In the initial observation at 1.8 d, source spectra were extracted from a 100\arcsec{} radius region centered on the transient. The background was similarly extracted from a 100\arcsec{} radius source-free region. For each of the latter observations, we used a 60\arcsec{} radius for both source and background regions. 


\subsection{Gemini}
\label{sec: gemini}

Target of Opportunity (ToO) observations of GRB 221009A were performed with the 8.1-m Gemini South Telescope in Cerro Pachon, Chile using GMOS-S and Flamingos-2 (hereafter F2) under two Director's Discretionary Time Programs (GS-2022B-DD-104, PI: O'Connor; GS-2022B-DD-103, PI: Rastinejad). The observations were first reported by \cite{GCN32749,GCN32750,GCN32860}.
Data were obtained at 4.4, 17.4, 25.4, and 26.4 d. The observations were carried out in the $i$ filter with GMOS-S, and $J$, $H$ $K_s$ filters with F2 (see Table \ref{tab:Optobservations}). We reduced and analyzed these data using the \texttt{DRAGONS}\footnote{\url{https://dragons.readthedocs.io/}} software \cite{Labrie2019}. The afterglow is clearly detected in each observation. 
%\textcolor{purple}{Using the initial images, we localize the GRB to RA, DEC (J2000) = $19^{h}13^m 03^{s}.85$, $+\ang{19;46;22.7}$ with an accuracy of $XXX\arcsec$.} 
We performed PSF photometry using \texttt{SExtractor} \cite{Bertin1996} and \texttt{PSFEx} \cite{Bertin2013}. The photometry was calibrated using nearby point-sources in the Two Micron All Sky Survey (2MASS;) \cite{Skrutskie2006} catalog. We then applied a standard conversion between the Vega and AB magnitude systems.

%First, we ran \texttt{SExtractor} to identify bright, unsaturated and isolated point-like objects.  We selected them based on their SNR, FWHM, \texttt{CLASS\_STAR} parameter ($>$\,$0.8$), and ellipticity ($<$\,$0.2$). We further imposed  \texttt{FLAGS}\,$<$\,$1$, which excludes sources that are saturated, blended, or too close to the image boundary. These point-like sources were then passed to \texttt{PSFEx} \cite{Bertin2011,Bertin2013} to estimate the image PSF. This was then fed to \texttt{SExtractor}


\subsection{Lowell Discovery Telescope}
\label{sec: LDT}

We obtained ToO observations with the Large Monolithic Imager (LMI) mounted on the 4.3-meter LDT at the Lowell Observatory in Happy Jack, AZ starting at 3.6 d after the GRB (PI: Cenko) and continuing observations for 8 weeks (see Table \ref{tab:Optobservations}). We first reported the initial observations in \cite{GCN32739,GCN32799}. The data were reduced with a custom pipeline \cite{Toy2016} that makes use of standard CCD reduction techniques in the IRAF\footnote{IRAF is distributed by the National Optical Astronomy Observatory, which is operated by the Association of Universities for Research in Astronomy (AURA) under cooperative agreement with the National Science Foundation (NSF).} package including bias subtraction, flat-fielding, and cosmic ray rejection \cite{vanDokkum2001}. Photometry was performed in the same manner as for Gemini, and calibrated against stars in the catalog (Pan-STARRS1, hereafter PS1) \cite{Chambers2016}. 

\subsection{MASTER}
\label{sec: master}

MASTER is a system of wide-field fully robotic 40-cm telescopes with identical scientific equipment and real-time auto-detection at every observatory \cite{Lipunov2004,Lipunov2010,Kornilov2012}. The MASTER telescopes are MASTER-Amur, -Tunka, -Ural, -Kislovodsk, -Tavrida (Russia), -SAAO (South Africa), -IAC (Spain), -OAFA (Argentina). The MASTER Global Robotic Net \cite{Lipunov2010} began observing GRB 221009A using MASTER-SAAO on 2022-10-09 at 17:33:54 UT, corresponding to 0.18 d after the \textit{Fermi} trigger. The MASTER auto-detection system discovered the optical counterpart, MASTER OT J191303.43+194623.1 \cite{GCN32634}, as a transient in the initial image. The observations were obtained in the \textit{clear} ($C$) filter. Further observations were obtained with MASTER-OAF starting on 2022-10-09 at 23:56:38 UT, corresponding to 0.46 d after the trigger (see Table \ref{tab:MASTERobservations}). Aperture photometry was calibrated using 20 reference stars, and we applied a further correction to convert to the AB magnitude system. We note that earlier observations by MASTER-Tunka and MASTER-Amur, beginning at 93 s after the \textit{Fermi} trigger (2022-10-09 14:11:50 UT), were severely impacted by clouds and were unable to detect the source. 



%MASTER network usually works in the Johnson-Cousins UBVRI photometric system. Thus, we use a conversion coefficient to work in AB system: $m_{AB} = m_{C}+k_{AB}$ where $k_{AB} = -2.5\log_{10}(\frac{F_{Vega}}{3631 Jy\cdot \Delta \nu })\approx -0.09$. $F_{Vega} = 1.6\cdot 10^{18}$ is zero point of MASTER clear band in UBVRI photometric system. MASTER work only in visible range, thus $ \Delta \nu = (7.89-3.84)\cdot 10^{14}=4.05\cdot 10^{14}$ marks constraints of this range. The \textit{clear} filter is similar to the \textit{GAIA} $G$-band.

%Best fit temporal slope for MASTER is $-0.84 \pm 0.16$ which agrees with that derived from the other bands (approx 0.9).

\subsection{Hubble Space Telescope}
\label{sec: HST}

%\begin{figure} 
%\centering
%\includegraphics[width=\columnwidth]{figs/GRB221009A_FC_HST_RGB.pdf}
%\caption{RGB image of the field of GRB 221009A: red is $\textit{HST}/F160W$, green is $\textit{HST}/F098M$, blue is $\textit{HST}/F606W$. The position of the GRB is marked by the white circle. An extension of the source to the North-East is due to the underlying host galaxy at $z=0.1505$. 
%}
%\label{fig: FC}
%\end{figure}

\textit{HST} observations were carried out at 29.7, 40.6, and 55.7 d after the GRB trigger (see Table \ref{tab:Optobservations}). Data were acquired in the WFC3/UVIS $F625W$ and $F775W$ filters and WFC3/IR $F098M$, $F125W$, and $F160W$ filters through a DDT request (PI: Levan). The initial observation was first reported by \cite{GCN32921}. 
We reduced the data using standard procedures within the \texttt{DrizzlePac} package \cite{Gonzaga2012}. The source is clearly detected in all filters with a marginal extension of the source to the NE in the infrared filters (see Figure \ref{fig: FC}), likely due to the underlying host galaxy at $z=0.1505$. %The galaxy is not identified in the initial WFC3/UVIS images, likely due to extinction from the Milky Way, but is found in the deep $F625W$ images from 2022 December 4. %\textcolor{purple}{Based on these \textit{HST} images we derive a more precise localization of the GRB to RA, DEC = XXX....}. 
We performed photometry of the source complex using a circular region of radius $0.3\arcsec$ centered on the transient. The zeropoints were taken from the photometry keywords in the image headers. %These measurements include the unknown host contribution. 



%\textcolor{purple}{In order to estimate the host contribution we also performed aperture photometry in a $1\arcsec$ aperture (DOES THIS MESS WITH STAR SPIKE?? USE DECEMBER 4 EPOCH TO AVOID THAT) and find a difference of XX mag, leading to an inferred host galaxy contribution of XX (can also do in December 4 F625W epoch)}


\subsection{\textit{ATCA}}
\label{sec: ATCA}

The Australia Telescope Compact Array (ATCA) observed GRB 221009A as part of the DDT project CX515 on 2022-10-15, 2022-10-24, 2022-11-04, 2022-11-19 and 2022-12-28 (Table \ref{tab:Radioobservations}). The initial observation at 5.8 d after the GRB was first reported by \cite{GCN32763,GCN32766}. In the initial two epochs, the three pairs of Intermediate Frequencies (IFs) were used 16.7/21.2 GHz, 33/35 GHz, 45/47 GHz and in the next two only 16.7/21.2 GHz and 33/35 GHz were used. In the last epoch, corresponding to 80 d after the GRB, observations were obtained at 5.5 and 9 GHz. In all observing runs the array operated in continuum mode with the Compact Array Broadband Backend using 2048 channels over 2-GHz bandwidth per IF. The radio sources used as bandpass, primary and phase calibrator were 1921-293, 1934-638 and 1923+210, respectively. The phase calibrator was also used for reference pointing checks every hour. Standard procedures in the data reduction software package \texttt{MIRIAD}
% (\textcolor{red}{CITE})
\cite{Sault1995_MIRIAD}
were used to flag, calibrate the complex gains and image the phase calibrator and target. A robustness parameter value of two and 6-km baseline antenna was deselected during imaging. The resulting flux densities and 3$\sigma$ upper limits are presented in Table \ref{tab:Radioobservations}. The errors are derived from summing in quadrature the statistical and systematic uncertainty (map rms and 5\% of the total flux as residual of gain calibration, respectively).


\section{Data Analysis}
\label{sec: analysis}


\subsection{Multi-wavelength Lightcurve}
\label{sec: lightcurve}

The afterglow of GRB 221009A displays a single break in the temporal decay of both the X-ray and optical/infrared (OIR) lightcurves (Figure \ref{fig: lightcurve}). By modeling the X-ray lightcurve with a broken power-law, we determine an initial decay index $\alpha_{\textrm{X},1}=-1.52\pm0.01$ steepening to $\alpha_{\textrm{X},2}=-1.66\pm0.01$ after $t_{\textrm{break},X}=0.82\pm0.07$ d. 

On the other hand, the OIR lightcurves, spanning $grizJHK$ and the MASTER \textit{C} filter, display a shallower decay and a more significant temporal break. We find an initial power-law decay of $\alpha_{\textrm{OIR},1}=-0.88\pm0.05$, which steepens to $\alpha_{\textrm{OIR},2}=-1.42\pm0.11$ at around $t_{\textrm{break,OIR}}=0.63\pm0.13$ d. In this analysis we have supplemented our dataset with observations reported in GCN Circulars
% (\textcolor{red}{CITE ALL THE GCNs}).
% \jg{these are the refs for all GCNs included in the email I received... 
% 32662, 32646, 32652, 32755, 32795, 32743, 32670, 32684, 32709, 32678, 32753, 32752, 32765, 32758, 32771, 32769, 32811, 32804, 32809, 32803, 32818, 32852}
\cite{
GCN.32769, GCN.32818, GCN.32684, GCN.32743, GCN.32752,
GCN.32652, GCN.32755, GCN.32646, GCN.32804, GCN.32678,
GCN.32811, GCN.32758, GCN.32803, GCN32765hostz, GCN.32670,
GCN.32662, GCN.32852, GCN.32795, GCN.32809, GCN.32753,
GCN.32771, GCN.32709}.

%We note that while the initial GCN data provides a sparse view of the early optical evolution, the data obtained by MASTER over this period is significantly more well-sampled. It is important to note that the observed decay based on GCN data alone is slightly shallower than the inferences from MASTER alone which yields an initial decay of $\alpha_{\textrm{MASTER},1}=-0.66\pm0.10$ with a break at around $0.6$ d.

The OIR and X-ray break times are separated by $0.19\pm0.15$ d. This may suggest that while the break could be achromatic, it is not immediately favored by the best-fit models. %This may be an artifact of the transition between WT mode and PC mode data obtained by \textit{Swift} XRT, as when masking\footnote{\url{https://www.swift.ac.uk/xrt_live_cat/01126853/}} the data obtained between 0.64 and 1.03 d, the best-fit break time is $\sim$\,$0.57$ d.  

Using the multi-epoch ATCA observations at 16.7 and 21.2 GHz we find that the temporal decline is well-described by a $t^{-1.0\pm0.2}$ evolution. Moreover, we observe a very steep decay of at least $t^{-2.4}$ at 45 GHz and 47 GHz between 5.78 and 14.72 d, hinting that the radio emission may be dominated by a separate component than the X-ray and OIR. 


\begin{figure} 
\centering
%\includegraphics[width=\columnwidth]{figs/GRB221009A_lc.pdf}
\includegraphics[width=\columnwidth]{figs/GRB221009A_lc_wRadio.pdf}
\caption{Multi-wavelength lightcurve of GRB 221009A. The OIR data is not corrected for Galactic extinction $A_V=4.09$ mag. The XRT and \textit{XMM-Newton} represent the X-ray flux density at 1 keV, whereas the flux density from \textit{NuSTAR} observations is obtained at 5 keV. OIR data represented as empty squares were compiled from GCN circulars.
}
\label{fig: lightcurve}
\end{figure}




\subsection{X-ray Spectroscopy}

%\textcolor{red}{Need to mention the harder initial WT mode spectrum... very important to the discussion and significance of spectral evolution while also showing independent of this initial spectrum the NuSTAR data shows an evolution, as observed for GRB 130427A (Kouveliotou et al. 2013).}

We began by analyzing the \textit{Swift}/XRT data ($0.3-10$ keV) obtained in Photon Counting (PC) mode between $10^5$ and $10^6$ s after the BAT trigger with a total exposure of 52.6 ks. We modeled the spectra using \texttt{XSPEC v12.12.0} \cite{Arnaud1996}. We applied the ISM abundance table from \cite{Wilms2000} and the photoelectric absorption cross-sections from \cite{Verner1996}. The best fit model parameters were determined by minimizing the Cash statistic \cite{Cash1979}. We applied the model \texttt{tbabs$*$ztbabs$*$pow} with fixed redshift $z=0.1505$ \cite{GCN32648xshooterz,GCN32686GTCz,GCN32765hostz}. The Galactic hydrogen column density was frozen to $N_H=5.36\times10^{21}$ cm$^{-2}$ \cite{Willingale2013}. The best fit parameters in this time range are $N_{H,z}=(1.3\pm0.1)\times 10^{22}$ cm$^{-2}$ and photon index $\Gamma=-1.73\pm0.05$. 

As a comparison, we analyzed the initial WT mode spectra obtained by XRT starting at $\sim$\,1 hr after the \textit{Fermi} trigger. This initial spectra displays a harder photon index of $\Gamma=-1.65\pm0.02$, hinting at spectral evolution in the X-rays from early times.

To further explore the X-ray spectral evolution, we turned to the \textit{NuSTAR} data ($3-79$ keV). We fit the FPMA and FPMB spectra simultaneously, allowing for the normalization of FMPB to vary. The normalization of FPMA was fixed to unity. The FPMB normalization varied by $\lesssim5\%$ compared to unity, likely due to a rip in the multi-layer insulation of FPMB \cite{Madsen+2020}. We applied the model \texttt{con$*$tbabs$*$ztbabs$*$pow} with $N_H$ and $N_{H,z}$ fixed to the values identified from our fit to the XRT data. The unabsorbed flux was derived using the \texttt{cflux} command. The data obtained at 23.93 and 31.95 d were fit between the 3-50 keV energy range, as this was where we found that the background began to dominate. The results of the \textit{NuSTAR} analysis are displayed in Table \ref{tab: nustar}. We observe a softening of the photon index between $-1.81\pm0.1$ at 1.82 d and $-2.1\pm0.17$ at 31.95 d. The latter value is consistent with the initial photon index, $\Gamma=-2.08\pm0.03$,  determined by \textit{Swift} BAT \cite{Krimm2022}.

We additionally analyzed the \textit{XMM-Newton} data obtained at 32.72 d by performing a joint fit with the \textit{NuSTAR} data obtained in a similar period, allowing for a normalization factor between the two spectra. We derive $N_{H,z}=(1.4\pm0.2)\times 10^{22}$ cm$^{-2}$ and photon index $\Gamma=-1.97\pm0.09$. 

A joint fit including X-ray data obtained at $<1$ d with XRT in WT mode (0.05, 0.25 and 0.44 d), XRT and \textit{NuSTAR} data at 1.8, 5.9, 10.72, and 23.93, and \textit{XMM-Newton} and \textit{NuSTAR} at $\sim$ 32 d yields a value of $N_{H,z}=(1.31\pm0.02)\times 10^{22}$ cm$^{-2}$, which is consistent with our estimates based on individual spectra. The photon index and normalization were allowed to vary between epochs. If we exclude the data obtained during the first orbit (0.05 d) and link the photon index as well, we derive $N_{H,z}=(1.29\pm0.02)\times 10^{22}$ cm$^{-2}$ and $\Gamma=-1.85\pm0.01$. Thus, $\Gamma=-1.85$ is the mean photon index obtained between 0.25 and 32 d. 



\begin{table}
    \centering
    \caption{Results of our \textit{NuSTAR} spectral analysis.  \textcolor{red}{[[[It is crucial to have a similar table for Swift/XRT as well as the optical/NIR spectral slope for different times (despite the "systematic" uncertainty due to extinction, the time dependence has important relevant information)]]]}
    }
    \label{tab: nustar}
    \begin{tabular}{lccc}
    \hline
    \hline
   \textbf{Time} & \textbf{$\Gamma$} & \textbf{$F_X$ (3-79 keV)} \\
   \textbf{(d)} & --   & \textbf{(erg cm$^{-2}$ s$^{-1}$)} \\
    \hline
    \hline
     1.82   & $1.81\pm0.01$ &  $(3.21\pm0.03)\times 10^{-10}$\\ %Cstat = 110 for 1153 dof
     5.92   & $1.89\pm0.03$ &  $(4.65\pm0.11)\times 10^{-11}$  \\ %Cstat = 537 for 546 bins
     10.72  & $1.88\pm0.05$ &  $(1.53\pm0.08)\times 10^{-11}$ \\ %Cstat = 218 for 226 dof
     23.93  & $1.94\pm0.12$ &  $(3.4\pm0.4)\times 10^{-12}$ \\ %Fit between 0-30 keV
     31.95 & $2.10\pm0.17$  & $(1.8\pm0.3)\times 10^{-12}$ \\ %Fit between 0-20 keV / Cstat = 820 for 845 dof
     \hline
     \hline
    \end{tabular}
\end{table}


\begin{figure} 
\centering
\includegraphics[width=0.5\columnwidth]{figs/GRB221009A_SED_figure.pdf}
\includegraphics[width=0.5\columnwidth]{figs/GRB221009A_gamma_times.pdf}
\caption{Observed spectral energy distributions (SEDs) of GRB 221009A between 0.05 and 41 d. The solid line is the combination of a FS and RS, while the dotted line shows the RS contribution. The data have been corrected for extinction and absorption: $E(B-V)=1.3$ mag and $N_H=1.3\times10^{22}$ cm$^{-2}$. 
}
\label{fig: SEDs}
\end{figure}

\subsection{Spectral Energy Distributions}
\label{sec: SEDs}

Based on our analysis of the X-ray spectra, we observe an evolving photon index from harder to softer values.  Due to this, in what follows we model the broadband spectral energy distributions (SEDs) with a smoothly broken power-law to account for possible spectral evolution with time. Moreove, the distinct decay slopes between the OIR and X-ray bands may suggest that the X-ray and OIR data lie on separate power-law segments of the synchrotron spectrum \cite{Granot2002}.


We utilized \texttt{XSPEC} to model the SEDs using an absorbed smoothly-broken power-law model. We took into account both absorption and extinction in the Milky Way and the host galaxy using the commands \texttt{redden$*$zdust$*$tbabs$*$ztbabs}\footnote{The \texttt{XSPEC} command \texttt{redden} takes into account extinction within the Milky Way \cite{Cardelli1989}, whereas  \texttt{zdust} corrects for dust in the host galaxy \cite{Pei1992},  assuming $R_V=A_V/E(B-V)$=3.1 \cite{Rieke1985}.}. We fixed the redshift to $z=0.1505$ \cite{GCN32648xshooterz,GCN32686GTCz,GCN32765hostz} and froze the hydrogen column density to the best fit values from our X-ray spectral analysis of $N_H=5.36\times10^{21}$ cm$^{-2}$ \cite{Willingale2013} and $N_{H,z}=1.3\times10^{22}$ cm$^{-2}$. The MW, $E(B-V)$, and host, $E(B-V)_z$, extinction were free to vary.

We simultaneously modeled twelve (12) broadband SEDs between 0.05 and 32 d. The low- and high-energy spectral indices were tied between SEDs, but the break energy $E_c$ was free to vary. The smoothness parameter $s$ was likewise tied between SEDs, but free to vary. The best fit smoothly broken powerlaw has $s\approx1$, $\beta_{\textrm{XOIR},1}=-0.63\pm0.05$, $\beta_{\textrm{XOIR},2}=-0.995\pm0.05$ with a reduced $\chi^2=1.2$ (see Figure \ref{fig: SEDs}). The break energy $E_c$ decreases in time between $\approx$\,$10$ to $\approx$\,$0.3$ keV. We find a value of MW extinction to be $E(B-V)=1.32\pm0.01$ mag, corresponding to $A_V=4.09\pm0.03$ mag, and a negligible intrinsic extinction. We derive an upper limit to the intrinsic extinction of $E(B-V)_z<\textcolor{red}{XX}$ at the \textcolor{red}{90\%} confidence level (CL).


The results of this smoothly-broken power-law model are quite similar to the expectations for a standard synchrotron spectrum \cite{Granot2002}. In this model, the spectrum is governed by the evolution of three frequencies: the cooling frequency $\nu_c$, the peak frequency $\nu_m$, and the synchrotron self-absorption frequency $\nu_a$, in addition to the slope $p$ of the electron power-law energy distribution $N(\gamma)\propto\gamma^{-p}$. As the initial modeling is suggestive of a cooling break scenario to explain the X-ray temporal and spectral evolution, we consider a smoothly-broken power-law model where the smoothness if given by $s=1.15-0.06p$ \cite{Granot2002} and $\beta_{\textrm{XOIR},1}=\beta_{\textrm{XOIR},2}+0.5$. We derive a value of $p=2.17\pm0.03$, which yields similar spectral slopes before and after the break as derived from the initial XRT, $\beta_\textrm{WT}=(1-p)/2=-0.65\pm0.02$, and BAT data, $\beta_\textrm{BAT}=-p/2=-1.08\pm0.03$) \cite{Krimm2022}. This result is independent of including the BAT data. In this model, we fixed the cooling break $E_c$ to move in time as $t^{-0.5}$ to mimic the temporal evolution of the cooling frequency in an ISM environment \cite{Granot2002}, as opposed to leaving it completely free between epochs. The result is displayed in Figure \ref{fig: SEDs}. 



%We began by modeling the broadband (X-ray, optical, nIR) SED at multiple epochs (3.6, 4.4, 9.5, XX, XX d). We tested whether the OIR and X-ray data could lie on the same spectral segment by jointly modeling the data within \texttt{XSPEC} using an absorbed power-law model \texttt{redden$*$zdust$*$tbabs$*$ztbabs$*$powerlaw}\footnote{The command \texttt{redden} corrects for extinction within the Milky Way \cite{Cardelli1989}, whereas  \texttt{zdust} accounts for intrinsic dust extinction within the host galaxy \cite{Pei1992} assuming a Milky Way extinction curve assuming $R_V=A_V/E(B-V)$=3.1 \cite{Rieke1985}.}. We fixed the redshift to $z=0.1505$ \cite{GCN32648xshooterz,GCN32686GTCz,GCN32765hostz} and froze the hydrogen column density to the best fit values from our X-ray spectral analysis of $N_H=5.36\times10^{21}$ cm$^{-2}$ and $N_{H,z}=1.2\times10^{22}$ cm$^{-2}$.

%We initially allowed the Milky Way extinction, parameterized by $E(B-V)$, to vary. Using the optical (GMOS-S), infrared (F2), and X-ray (XRT) data at $4.4$ d, we derive $E(B-V)=1.32\pm0.03$ mag, yielding $A_V=4.09\pm0.09$ mag. We freeze this result in our following analysis. 
%\textcolor{red}{using Guver and Ozel - NHz =1.2e22 $\rightarrow$ Av=5.4+/-0.5 mag...}

%In our SED analysis we observe a softening of the spectrum from $\Gamma=1.71\pm0.01$ at 3.6 d and $\Gamma=1.79\pm0.02$ at 24 d. \textcolor{red}{Plot of Photon Index vs time?}




%\begin{table*}
%    \centering
%    \caption{Results of our broadband SED analysis. \textcolor{red}{nH, nHz, E(B-V), E(B-V)z}
 %   }
 %   \label{tab: sed}
 %   \begin{tabular}{lccccccc}
 %   \hline
 %   \hline
 %  \textbf{Time} & $E(B-V)$ & $E(B-V)_z$ &  \textbf{$\Gamma$}  & \textbf{Normalization} & \textbf{$\Gamma_1$} & \textbf{$\Gamma_2$} & \textbf{Normalization} \\
%   \textbf{(d)} & (\textbf{mag}) &  (\textbf{mag})& -- & \textbf{(XXX)} & -- & -- & \textbf{(XXX)} \\
%    \hline
%    \hline
%     & & & & & & & \\
%     \hline
%     \hline
%    \end{tabular}
%\end{table*}





\section{Results} 
\label{sec: results}

\subsection{Standard Forward Shock}



Motivated by our SED modeling, we began by exploring the simple scenario of a relativistic fireball \cite{Meszaros1997,Sari1998,Wijers1999,Granot2002} propagating into an ambient medium with density of the form $\rho_{\textrm{ext}}(r)=A\, r^{-k}$, where $k=0$ represents an interstellar medium (ISM) environment and $k=2$ a stellar wind environment. The shock-accelerated electrons cool via synchrotron radiation with a characteristic spectrum dominated by the three break frequencies: $\nu_c$, $\nu_m$, and $\nu_a$. In the following we separately consider the lightcurve evolution in the X-rays, OIR, and radio.

\subsubsection{X-ray Lightcurve}

The X-ray lightcurve displays a break at around $\sim$\,1 d with a change in slope of $\Delta\alpha_X=0.14\pm0.02$. This can be explained by the passage of $\nu_c$ through the X-ray band. 

As we observe a steepening of the X-ray spectral index in time, this is consistent with the transition from  $\nu_m<\nu<\nu_c$ to $\nu_m<\nu_c<\nu$ where the spectral index steepens from $\nu^{(1-p)/2}$ to $\nu^{-p/2}$. The change in X-ray spectral index of $\Delta\beta_X=0.46\pm0.07$ is consistent with this scenario where $\Delta\beta=0.5$. This implies that the cooling frequency $\nu_c\propto t^\frac{3k-4}{2k-8}$ must decrease in time such that $k<4/3$.


In this case\footnote{Here, G and H refer to the power-law segments defined by \cite{Granot2002}, where G corresponds to $\nu_m<\nu<\nu_c$ and H to $\nu_m<\nu_c<\nu$.}, the initial temporal decay is provided by $\alpha_G=\frac{k(3p-5)-12(p-1)}{4(4-k)}$ \cite{BGG2020}, whereas after the passage of $\nu_c$ (i.e., $\nu_m<\nu_c<\nu$) the decay is  $\alpha_H=\frac{(2-3p)}{4}$, which is independent of $k$.  %These considerations thus far ignore Inverse Compton (IC) corrections \cite{Sari2001,Zou2009,Beniamini2015,Jacovich2021}. 

The post-break slope  $\alpha_H=-1.66=(2-3p)/4$ requires a steep $p\approx2.88$. Furthermore, the change in temporal slope due to the crossing of $\nu_c$ is  $\Delta\alpha_{GH}=\alpha_G-\alpha_H=\frac{3}{4}+\frac{2}{k-4}$, which is independent of $p$. We find the requirement $\Delta\alpha\sim0.14\pm0.02$ to be satisfied by $k\approx 0.72$. 

%In addition, while these considerations easily explain the X-ray temporal and spectral evolution, they do not explain the evolution of the OIR lightcurve, or the shallower post-break OIR slope.  Thus, we exclude this simple FS scenario to explain GRB 221009A's afterglow lightcurve.

\subsubsection{Optical and Infrared Lightcurve}

The OIR lightcurve displays a shallow initial slope of $\alpha_\textrm{OIR,1}\approx-0.9$ followed by a steeper decay of $\alpha_\textrm{OIR,2}\approx-1.45$ after $\sim$\,1 d. The initial slope can be explained by optically thin synchrotron radiation in an ISM environment ($k=0$) as $\alpha=3(1-p)/4=-0.9$ for $p=2.2$. A stellar wind environment leads to significantly steeper slopes. However, utilizing the steep $p=2.88$ inferred from the X-rays is inconsistent with the initial shallow OIR slope and fails to explain the break in the OIR lightcurve. 

One alternative possibility, is that the initial OIR data at $<$\,1 d is below $\nu_m$, such that the transition from $\nu_\textrm{OIR}<\nu_m$ to $\nu_m<\nu_\textrm{OIR}$ can explain the lightcurve break. In this case, the post-break slope would be provided by $\alpha_G=-1.52$ as for the X-rays, assuming $p=2.88$ and $k=0.72$. The excess flux from the underlying supernova \cite{GCN32800,GCN32850} can then explain the observed OIR slope of $\alpha_\textrm{OIR,2}=-1.45$. 

While this scenario appears to resolve the lightcurve slopes, a major issue with these closure relations is that the inferred value of $p=2.88$ is significantly steeper than determined by our SED modeling (\S \ref{sec: SEDs}). In fact, modeling the SEDs with $p=2.88$ fails to produce a satisfactory fit the data. We further discuss these inconsistencies and possible resolutions (e.g., a jet-break) \cite{Rhoads 1999,Sari 1999} below in \S \ref{sec: scenario1} and \S \ref{sec: scenario2}. 

\subsubsection{Radio Lightcurve}

The high-frequency radio data (Table \ref{tab:Radioobservations}) obtained between 5.8 and 40.7 d display a significantly different evolution than the X-ray and OIR data (Figure \ref{fig: lightcurve}). This is not unexpected given the data could lie in separate regimes of the FS or be significantly affected by a bright RS, as found for other energetic GRBs displaying GeV emission
% (\textcolor{red}{CITE: van der Horst 2013 on 130427A, Dichiara et al. on 190829, and Rhodes et al. on 190829A}).
\cite{Stanek2003,van_der_Horst2014, Rhodes2020, Dichiara2022}.
%In our analysis we include radio data presented in GCN circulars (\textcolor{red}{CITE ALL}).
Given that the ATCA data (Figure \ref{fig: lightcurve}) is decreasing with time, we infer that it is dominated by a bright RS component, as the expected FS evolution for $\nu<\nu_m$ is $t^{(2-k)/(4-k)}$ which is rising for reasonable values of $k$, e.g., $k=0$ leads to $t^{1/2}$.






%\textcolor{purple}{These considerations thus far ignore Inverse Compton (IC) corrections \cite{Sari2001,Zou2009,Beniamini2015,Jacovich2021}, which are ubiquitous when discussing synchroton radiation and should be included when the Compton parameter $Y>1$.} 


%\textbf{\textcolor{purple}{Do we note that the GeV data may imply $Y\approx1$ at $10^5$ s, and decreasing from there???... But this is likely a lower-limit on the Y parameter as the IC peak is likely in the TeV range...}}

\subsection{Reverse shock}


The high-frequency radio data (Table \ref{tab:Radioobservations}) is likely dominated by a bright RS. In Figure \ref{fig: ATCA_SEDs} we display the multi-epoch SEDs obtained by ATCA. We observe a shallow spectral slope of $\nu^{-0.5}$ steepening to $\sim$\,$\nu^{-3}$ (Figure \ref{fig: ATCA_SEDs}). The shallow pre-break slope could indicate that the radio data is either \textit{i}) fast cooling such that $\nu_c<\nu_a<\nu<\nu_m$ or \textit{ii}) slow cooling  ($\nu_m<\nu<\nu_c$) where  $\nu^{-0.5}=\nu^{(1-p)/2}$ for $p\approx2$. The steep cut-off decreases in time, and explains the steep evolution of the high frequency radio data.

We observe that this cut-off frequency, hereafter $\nu_\textrm{cut}$, decreases in time from $\sim45-50$ GHz at 5.8 d to $\lesssim16$ GHz at 40.7 d. We attribute this to a post-shock crossing residual population of cooling electrons \cite{Kobayashi2000} \textcolor{purple}{(Any other references on this?)}, above which the flux decays exponentially. The evolution of this frequency in time is observed to be non-standard as between 5.8 and 40.7 d we require an evolution of at least $t^{-0.5}$. An evolution much steeper than this fails to explain the SEDs at 14.7 and 25.7 d. However, even assuming an evolution of $t^{-1.5}$ \cite{Kobayashi2000}, if we trace this frequency back in time we find that $\nu_\textrm{cut}<\nu_\textrm{OIR}$ at $\lesssim 1$ d. This implies that the RS is unlikely to dominate the early OIR emission. 

\textcolor{purple}{What should we say regarding the shallow radio slope of $t^{-1}$ at 16 and 21 GHz.. discussion points: 1) not typical RS, too shallow 2) RS+FS could shallow it out but then the FS needs to be dominating at late times, which we do not observe and \textbf{3) could the shallow jet structure be flattening out the RS emission...}} What is the shallowest slope we can get for a RS (thin/thick shell)? \textbf{-1.5 for PLS G in the the thin-shell case.. but -1.5 + FS could = -1...} Good to state in text and compare.

%\textcolor{purple}{add discussion of observational constraints on cutoff frequency $\nu_\textrm{cut}$ (post shock-crossing residual population of cooling electrons) and fit with $(t-to)^a$; reference https://iopscience.iop.org/article/10.1086/317869/pdf and https://iopscience.iop.org/article/10.3847/1538-4357/ab40ce} ... cutoff frequency does not explain data well because on-constant decay is observed...

\vspace{10mm}


Radio data can be affected by interstellar scintillation (ISS)
\cite{Rickett1990, Goodman1997} due to fluctuations in the density of free electrons. Following \cite{Hancock2019}, we derive a scatting measure of  SM$=4.3\times 10^{-4}$ kpc $m^{-20/3}$, a transition frequency of $\nu_0=9$ GHz between strong and weak scattering, and the angular size of the first Fresnel zone $\theta_{F0}=2.1\times10^{4}\, \textrm{SM}^{0.6}\nu_0^{-2.2}=1.6\,\mu$as  \cite{Walker1998}. At the putative redshift $z=0.1505$, an angular size of $1\,\mu$as corresponds to a physical size of $8.2\times10^{15}$ cm, such that $\theta_{F0}$ corresponds to a source size of $1.3\times 10^{16}$ cm. As the ATCA frequencies are in the weak scintillation regime $\nu_o<\nu$, we likewise compute $\theta_w=\theta_{F0}\big(\frac{\nu}{\nu_0}\big)^{-1/2}$ which yields $\theta_w=1.1\,\mu$as for $\nu=16.7$ GHz. For source sizes $\theta_s$ larger than $\theta_w$, the modulation index decreases as $\big(\frac{\theta_s}{\theta_w}\big)^{-7/6}$. This implies that the ATCA observations are unlikely to be affected by flux modulations due to scintillation. \textcolor{red}{But at the same time, it appears ISS could be at play between 15 and 27 d... Figure \ref{fig: ATCA_SEDs}.}



\begin{figure} 
\centering
\includegraphics[width=\columnwidth]{figs/GRB221009A_ATCA_SEDs_2.pdf}
\caption{Spectral energy distributions of the radio data from ATCA between $16.7-47$ GHz. We observe a steep decay of the radio data, indicative of emission from a reverse shock. 
}
\label{fig: ATCA_SEDs}
\end{figure}


\subsection{A forward-shock plus a reverse-shock}
\label{sec: scenario1}

\textcolor{purple}{Re-write this to tell a more simple and clear story and show more clearly why 'vanilla' case and RS case do not work well. Focus on the observations not the theory!}

{\bf PB: What is missing from this section is a clear description of which frequencies are dominated by FS and RS and at what times.}
As previously noted, there are two major limitations with the FS model to describe the observed afterglow behavior: \textit{i}) The post-break slope of the X-rays requires a steeper value of $p$ than implied by the broadband SEDs and \textit{ii}) the standard FS model fails to describe the early OIR slope. 

As discussed in the previous section, GRB 221009A displays a bright RS component, which likely contributes to the early OIR emission. Therefore, a significant contribution of the RS to the early ($<0.6$ d) OIR emission and a rising FS component could explain the shallow decay of the OIR at $<0.6$ d. In this scenario, OIR wavelengths would initially lie below the peak frequency such that $\nu_\textrm{OIR}<\nu_m$ with $\nu_m$ beginning to cross the OIR at around $0.5$ d {\bf PB: Throughout this section, perhaps use a different notation for frequencies corresponding to RS and FS}. The evolution of $\nu_m\propto t^{-1.5}$ is independent of both $p$ and $k$. Assuming that $\nu_m=(6-8)\times 10^{14}$ Hz at 0.5 d, by $\sim$1 d $\nu_m$ would pass through the near-infrared. 

At a similar time, $\nu_c$ would pass down through the X-rays in order to describe the evolution of the X-ray spectral index and the broadband SED modeling. Despite this, we are still left to explain the discrepancy between the steep X-ray slope above $\nu_c$ and the value of $p$ inferred by our SED modeling, which would imply $t^{(2-3p)/4}=t^{-1.15}$ for $p=2.2$. This is significantly shallower than the observed post-break decline of $t^{-1.66}$.

{\bf PB: I would leave the changing of microphysical params. to the end of the section. Only after you describe that the vanilla version doesn't work, you may want to briefly address whether adding a dependence of microphysical params with time changes this (in any case, this will not solve the fine tuning involved with different characteristic frequencies crossing through observed bands at the same time).}
In order to mitigate this, we consider breaking standard assumptions as to the evolution of the afterglow model. We consider a possible time-dependent evolution of the microphysical parameters, as applied to describe other well-sampled GRB lightcurves
(e.g., \cite{Racusin2009,Filgas2011, van_der_Horst2014}). 
Following \cite{GranotSari2022}, the flux and frequency evolution 
%in the globally slow cooling regime 
is given by:
\begin{align}
\label{eqn1}
    &F_{\nu,\textrm{G}}\propto \varepsilon_e^{p-1} \varepsilon_B^{(1+p)/4}  t^\frac{k(3p-5)-12(p-1)}{4(4-k)} \:\textrm{for}\:\nu_m<\nu<\nu_c \\
    &F_{\nu,\textrm{H}}\propto \varepsilon_e^{p-1} \varepsilon_B^{(p-2)/4} t^{(2-3p)/4} (1+Y)^{-1} \:\textrm{for}\:\nu_c<\nu \\
    &\nu_c\propto\varepsilon_B^{-3/2}t^{(3k-4)/(8-2k)} (1+Y)^{-2} \\
    &\nu_m\propto \varepsilon_e^{2} \varepsilon_B^{1/2} t^{-3/2} 
\end{align}
where $\varepsilon_e$ is the fraction of the burst kinetic energy $E_k$ in electrons, $\varepsilon_B$ is the fraction in magnetic fields, and $Y$ is the Compton parameter. We begin by considering a scenario where $Y\ll1$ by $\sim$\,$1$ d, such that the inclusion of SSC corrections can be ignored. This requirement may be difficult to reconcile with the long-lasting GeV emission (\textcolor{red}{CITE}). In fact, while the ratio of the X-ray to GeV emission at $\sim$\,$10^5$ s implies $Y\approx1$ \cite{Piran2009,Beniamini2011} this provides a lower-limit as the SSC emission peak is likely at TeV energies \cite{GCN32677}. 

Assuming that $p=2.2$, we require that the time-dependence of the microphysical parameters adds an additional $t^{-0.51\pm0.01}$ to the temporal decay above $\nu_c$. As the flux above $\nu_c$ has a very shallow dependence on $\varepsilon_B$, such that $F_{\nu,\textrm{H}}\propto \varepsilon_B^{1/20}$ for $p=2.2$, it is more practical to consider a time-evolution of $\varepsilon_e$. Furthermore, as $\nu_c$ is independent of $\varepsilon_e$ for $Y\ll1$, the requirement that the cooling frequency decreases with time is more easily satisfied. Thus, we find $\varepsilon_e\propto t^{-0.425}$ satisfies both our requirements. Given that the $\varepsilon_e$ dependence of $F_{\nu,\textrm{H}}$ and $F_{\nu,\textrm{G}}$ is the same, we can determine the value of $k$ by again using  $\Delta\alpha_{GH}=\frac{3}{4}+\frac{2}{k-4}=0.14\pm0.02$ which is satisfied by $k\approx 0.72$. In this case, $\nu_c\propto t^{-0.28}$. % and the flux below $\nu_m$ increases as $F_{\nu,\textrm{D}}=t^{(2-k)/(4-k)}=t^{0.39}$. 
Indeed the evolution of $\nu_m\propto t^{-2.35}$ is also increased, such that it can more quickly move through the OIR band. 

\textcolor{purple}{Still need to add something on actually why we disfavor this scenario due to fine-tuning and that the RS might actually not be able to contribute to OIR due to cutoff frequency... need to consider simplest way to introduce this without going into detail on the RS...}

\textcolor{purple}{Note that this case requires a lot of stuff happening at exactly the same time and is very fine-tuned so we favor the structured jet instead.}

In order for the fast $\nu_m$ evolution to be consistent with the upper limits from ATCA at 14.68 and 40.71 d, we require that the synchrotron self-absorption frequency $\nu_a$ is located above those frequencies such that $\nu_a\approx 50$ GHz at 40.71 d. As $\nu_a\propto \varepsilon_e^{-1}t^\frac{3k}{5(k-4)}=t^{-0.56}$ for the scenario described above, we would require $\nu_a\approx 400$ GHz at 1 d after the GRB.  \textcolor{red}{since we disfavor this model is it even worth noting this weird/impossible $\nu_a$ requirement ...}

\subsubsection{Constraints on the bulk Lorentz factor}

We can use the requirement that the jet must decelerate before $1$ hr (0.05 d) after the \textit{Fermi} trigger to constrain the initial bulk Lorentz factor $\Gamma_0$. 
The initial bulk Lorentz factor $\Gamma_0$ is obtained following \cite{SariPiran1999,Nappo2014}, where for a homogeneous environment \jg{What is the exact duration of the prompt GRB emission ($T_{50}$, $T_{90}$ etc.) and what constraints do we have on the afterglow onset time? This can constrain the thin vs. thick shell case for the deceleration of the GRB ejecta}\brendan{The GRB duration depends on the instrument observing it, but a typical value I think is $\sim600-700$ s. As for the afterglow onset, no afterglow follow-up happened until the Swift trigger almost an hour after the GRB because Fermi did not send a notice, so 1 hour is the best we can do.}
\begin{equation}
    \Gamma_0 > \Big[\frac{17}{64\pi}\frac{E_\textrm{kin,iso}}{c^5 n_0 m_p (\frac{t_p}{1+z})^3}\Big]^{1/8}. 
\end{equation}
Here, $c$ is the speed of light, $m_p$ is the mass of a proton, and $t_p$ is the upper limit on the peak time. Using a kinetic energy of $E_\textrm{kin,iso}\approx1\times10^{55}$ erg (and thus a gamma-ray efficiency of 15\%) \cite{Nava2014}, circumburst density $n_0=1$ cm$^{-3}$, and a peak time of $t_p<0.05$ d, we obtain $\Gamma_0>76$. This constraint is largely independent of our interpretation of the afterglow emission and relies on the early X-ray detection by \textit{Swift}/XRT. 


\subsubsection{Energetics}

In addition to being challenged to explain the observed spectral and temporal evolution, a standard jet scenario of the type addressed above, is challenged in terms of the required energetics to power the burst. The OIR and X-ray lightcurve evolve as $t^{-1.5}-t^{-1.66}$ up to at least 80 days after the trigger (at the time of writing). This is much shallower than the decay that would be expected after the jet break, $t_{\rm j}$, for a jet with a steep angular structure of the kinetic energy (typically, $t^{-p}$) \cite{Sari1999}. $t_{\rm j}$ represents the point in time at which $\Gamma$ has decelerated to $\theta_0^{-1}$ (where $\theta_0$ is the opening angle of the jet). Therefore, we can put an observational lower limit on $t_{\rm j}>t_{\rm j,l}=80$ d, which leads to a lower limit on the jet opening angle $\theta_0$. This in turn leads to a lower limit on the true (i.e. collimation-corrected) of the GRB, $E_{\rm t}\approx\frac{1}{2}\theta_0^2E_{\rm kin,iso}(\theta_{\rm obs})$, where we have assumed that the observer viewing angle relative to the jet axis is $\theta_{\rm obs}<\theta_0$. This is conservative as if this were not the case the lower limit on $E_{\rm t}$ would only increase. The limit to the energy is given by
\begin{equation}
    E_{\rm t}>E_{\rm kin,iso}(\theta_{\rm obs}) \frac{1}{2}t_{\rm j,l}^{\frac{3-k}{4-k}} \left(\frac{(3-k)E_{\rm kin,iso}(\theta_{\rm obs})}{4\pi A 2^{3-k} c^{5-k}}\right)^{\frac{1}{k-4}} 
\end{equation}
This limit generally decreases with $k$. Since $\nu_c$ is seen to decrease in time (see \S \ref{sec: SEDs}), we can in addition require that $k<4/3$. Therefore the most conservative estimate is given for $k=4/3$. Plugging either $k=0$ or $k=4/3$ we find
\begin{eqnarray}
    E_{\rm t}\!>\!\left\{ \begin{array}{ll}6\!\times \!10^{53}\mbox{ erg}\left(\frac{t_{\rm j,l}}{80\mbox{ d}}\right)^{3/4} (f(\eta_{\gamma})E_{\rm \gamma,iso,54.5})^{3/4}n_0^{1/4} & k=0 ,\\ \\
2.6\!\times \!10^{53}\mbox{ erg}\left(\frac{t_{\rm j,l}}{80\mbox{ d}}\right)^{5/8} (f(\eta_{\gamma})E_{\rm \gamma,iso,54.5})^{5/8}A_0^{3/8}  & k=\frac{4}{3}
\end{array} \right.
\end{eqnarray}
\textbf{\textcolor{purple}{where (please explain notations here, including $n_0,A_0$...)}} and $f(\eta_{\gamma})=3(1\!-\!\eta_{\gamma})/(17\eta_{\gamma})$ carries the dependence on the $\gamma-$ray efficiency and has been normalized such that it is unity for $\eta_{\gamma}=0.15$ as supported by observations of the brightest GRBs \cite{Beniamini2015}. 
\textcolor{red}{We should also put (for observers) what the constraint on $\theta_0$ is based on this - not as equation in text, but just one sentence should do...}

We see that the required (collimation-corrected) energy is extremely large and depends only weakly on the unknown external density. Such a huge energy is not readily explained by theoretical considerations. Furthermore, if this were to be the true energy of GRB 221009A, it would make it an extreme outlier to the GRB energy distribution. This possibility is therefore challenged even on statistical grounds only, assuming no priors on possible energy sources of GRBs.




%\textcolor{purple}{All of the above is assuming $Y<1$, such thatg SSC corrections can be ignored... }

%\textcolor{purple}{Need to solve for $\nu_m$, $\nu_c$, and $F_{\nu_m}$ self consistently to derive some constraints on the parameters... }

%\textcolor{purple}{Here also need to explain the post-break OIR slope as being shallower due to SN+Host... Can we say anything on host galaxy?}




\subsection{An on-axis structured shallow jet }
\label{sec: scenario2}
The similar break time between the OIR and X-rays is suggestive of an achromatic break, which suggests an origin based on the jet dynamics rather than a characteristic frequency passing through an observed band. 
{\bf PB: What about the spectral slope before and after the break? Are they consistent with no spectral break passage?} 
One common origin for an achromatic break is the so-called jet-break \cite{Rhoads1999,Sari1999}.  

Following \cite{BGG2020} Table 4, we can compute the change in slope due to an on-axis non-spreading, tophat jet. 
%These slopes provide a lower limit to the post jet-break slope given that a spreading jet can be significantly steeper with $\alpha\lesssim-p$ \textcolor{red}{Rhoads 1999}. 
The change in slope is provided by $\alpha_d-\alpha_f$, where $\alpha_f$ is the slope with no lateral spreading and thus a lower limit on the steepness of the post-break decay. The change in slope is independent of $p$ with $\Delta\alpha=\alpha_d-\alpha_f=(3-k)/(4-k)$. %This is the same change in slope for PLS D, G, and H...
This requires an incredibly steep $k\approx2.8$ to be consistent with the X-ray observations, and does not explain the larger change in slope of the OIR data. As we will show below, the value of $\Delta \alpha$ can be significantly reduced for a jet with a shallow angular structure of the kinetic energy.

The standard assumption that GRB jet's have a constant energy $dE_k/d\Omega$ within the core of the jet is likely an oversimplification (\textcolor{red}{CITE simulations?}), and a structured jet naturally arises as the GRB breaks out of its stellar environment. Therefore, we consider a GRB jet with a shallow broken power-law structure defined by %$dE_k/d\Omega\propto \Theta^{-a_1}$ for $\theta<\theta_{\rm c}$ and $dE_k/d\Omega\propto \Theta^{-a_2}$ for $\theta>\theta_c$ {\bf PB: It is probably better to have the above expression as a proper equation. Please add that when you can.}
\begin{align}
    dE_k/d\Omega\propto \Theta^{-a_1}\;\textrm{for}\;\theta<\theta_{\rm c} \\
    dE_k/d\Omega\propto \Theta^{-a_2}\;\textrm{for}\;\theta>\theta_c
\end{align}
where $\Theta=\sqrt{1+(\theta/\theta_c)^2}$ {\bf PB: and $a_1,a_2\lesssim 2$ (see ... for an exact limit for the applicability of this scenario)}. In this case, the flux and frequency evolution is dictated by the jet-structure, leading to a shallow angular structure dominated emission (sASDE) phase (see Tables 1 and 2 of) \cite{BGG2022}. %In this case, the \textcolor{purple}{change in slope due to a jet-break} is computed using \cite{BGG2022} Table 2 as $\Delta\alpha=\alpha_d-\alpha_s$. 
The flux evolution {\bf PB: is initially the same as for a spherical outflow with an isotropic equivalent energy given by the value along the line of sight. This lasts up to a time, $t_{\rm sph}$ \cite{BGG2022} when the Lorentz factor along the line of sight has decelerated to $\theta_{\rm obs}^{-1}$. After this time the flux evolves as}
in this regime is \cite{BGG2022}: \textcolor{red}{add the Ekin dependence as an equation to make it clear how these are derived? simplify eqns 10-11 for k=0 for simplicity of reading them. note for a=0, i.e., tophat jet, they simplify to the standard equations...}
\begin{align}
\label{eqn2}
    &F_{\nu,\textrm{G}}\propto  t^{-\frac{(a_1+6)kp+(a_1-2)(5k-12)-24p}{4(a_1+2k-8)}} \:\textrm{for}\:\nu_m<\nu<\nu_c \\
    &F_{\nu,\textrm{H}}\propto  t^{\frac{-a_1kp-2a_1k+8a_1-6kp+4k+24p-16}{4(a_1+2k-8)}} \:\textrm{for}\:\nu_c<\nu,
  %  &\nu_c \propto t^{\frac{(a-2)(3k-4)}{2(a+2k-8)}} \\
  %  &\nu_m\propto  t^{-3/2-\frac{a(k-3)}{2(a+2k-8)}}.
\end{align}
where the microphysical parameter dependence is identical to Equation \ref{eqn1} and we have not included IC corrections. 
{\bf This phase lasts until $t_{\rm c}$ which is the time at which $\Gamma(\theta_c)=\theta_c^{-1}$. After this time, the flux evolves in a similar way to the expressions given in \ref{eqn2}, but with $a_2 \rightarrow a_1$.}

{\bf PB: It might be a good idea to give the expression for $\Delta \alpha$ in this case, since you discuss it above for the steep jet case. This will be a natural way to lead to the discussion below.}
For an initial power-law slope of $a_1=0.6$ which steepens to $a_2=1.1$ after $\sim$\,1 d, we can identify a solution that fits the X-ray and OIR data.
Here, we have assumed that $\nu_m<\nu_\textrm{OIR}<\nu_c<\nu_X$ such that the X-rays and OIR lie on separate power-law segments. This naturally explains the different post-break slopes (Figure \ref{fig: lightcurve}). 
%\nu_m<\nu_\textrm{OIR}<\nu_c<\nu_X$ 
We find an adequate solution for $p=2.2$ and $k=0$, which yields initial pre-break slopes of  $\alpha_\textrm{\textrm{OIR},1}=-1.2$ and $\alpha_{X,1}=-1.4$, which steepen to $\alpha_\textrm{\textrm{OIR},2}=-1.45$ and $\alpha_{X,2}=-1.6$ after $\sim$\,1 d. This provides a good agreement with the observations (Figure \ref{fig: shallowjetlightcurve}). \textcolor{purple}{While these slopes provide a good qualitative description of the data, we find that adding even a slight microphysical parameter time dependence of $\varepsilon_B\propto t^{0.2}$ can create an even better agreement.} {\bf PB: Perhaps a more natural way to improve slightly the fit, is to make the structure even more gradually evolving with $\theta$ (e.g. $E_{\rm iso}\propto \theta^0$ below some $\theta_*$, transitioning to $E_{\rm iso}\propto \theta^{a_1}$ above that and continuing as described above at greater angles still.}

\textcolor{purple}{To add: solving for some parameters using constraints on nuc,num etc... Also need nua...}

%Here, we have assumed that $\nu_m<\nu_\textrm{OIR}<\nu_c<\nu_X$ such that the X-rays and OIR lie on separate power-law segments. This naturally explains the different post-break slopes (Figure \ref{fig: lightcurve}). We find an adequate solution for $p=2.2$, $k=0$, and $a=1$, which yields pre-jet break slopes of  $\alpha_\textrm{\textrm{OIR},1}=-0.9$ and $\alpha_{X,1}=-1.15$. The post-break slopes are then $\alpha_\textrm{\textrm{OIR},2}=-1.45$ and $\alpha_{X,2}=-1.6$, which is agreement with the observations (Figure \ref{fig: lightcurve}).

%This scenario easily explains the post-break slopes of both the X-rays and OIR, but instead does not explain the early X-ray slope. This may be explained by an early excess emission due to IC at $<0.5$ d. A bright IC emission component may be expected given the long-lived GeV emission detected by \textit{Fermi} LAT (\textcolor{red}{CITE}). %, but this would also lead to a large $Y$ parameter, impacting the equations used to reach these conclusions. 
%Moreover, in this case we have some trouble to re-produce the spectral evolution of the X-rays and the different slopes for the initial XRT and BAT data, which $\beta_\textrm{XRT}-\beta_\textrm{BAT}\approx 0.5$. 





%X-rays: $=(2 - 3 p)/4$ to $\alpha_{s,H}=\frac{-akp - 2 ak + 8 a - 6 kp + 4 k + 24 p - 16}{4(a + 2 k - 8)}$
%OIR: $\alpha_{s,G}= -\frac{(a + 6) kp + (a - 2) (5 k - 12) - 24 p}{4 (a + 2 k - 8)}$



%\textcolor{purple}{Can the excess be external IC of the RS? consistent with cutoff frequency? For a cutoff frequency of $\sim10^{13}$ Hz at $\sim0.2$ d would require $\gamma_c\approx 100$ at 5-10 hr after the GRB for IC to peak at 1 keV ($\gamma_c^2\nu_\textrm{cut}\approx1$ keV), but does not explain why it would be a narrow-band phenomena not impacting the OIR. But this also depends on the strength of the IC, which needs to be considered. }

%\textcolor{red}{An alternative solution is that both X-ray and OIR lie on same PL segment initially, x-rays have cooling break at similar time as jet-break but as this also requires RS and peak frequency passage in OIR it just doesn't seem as practical...}


%\subsubsection{Broken power-law jet structure}

%\textcolor{blue}{Add/refine text on shallow jet.}

%The standard assumption that GRB jet's have a constant energy $dE_k/d\Omega$ within the core of the jet is likely an oversimplification (\textcolor{red}{CITE simulations?}), and a structured jet naturally arises as the GRB breaks out of its stellar environment.  Therefore, we consider a GRB jet with a power-law energy structure $dE_k/d\Omega\propto \Theta^{-a}$ where $\Theta=\sqrt{1+(\theta/\theta_c)^2}$. 

%For an initial power-law slope of $a_1=0.6$ which steepens to $a_2=1.1$ after $\sim$\, 1 d, we can identify a solution that fits the X-ray and OIR data. Using $k=0$, $p=2.2$ and $\nu_m<\nu_\textrm{OIR}<\nu_c<\nu_\textrm{X}$, we obtain initial slopes $\alpha_\textrm{\textrm{OIR},1}=-1.2$, $\alpha_{X,1}=-1.4$, which steepen to  $\alpha_\textrm{\textrm{OIR},2}=-1.45$ and $\alpha_{X,2}=-1.6$ after $\sim$\,1 d. \textcolor{purple}{While these slopes provide a good qualitative description of the data, we find that adding even a slight microphysical parameter time dependence of $\varepsilon_B\propto t^{0.2}$ can create an even better agreement.} 


\begin{figure} 
\centering
\includegraphics[width=\columnwidth]{figs/GRB221009A_lc_shallowjet.pdf}
\caption{Multi-wavelength lightcurve of GRB 221009A. The dashed lines are determine using the structured jet model outlined in \S \ref{sec: scenario2}, and provide a good description of the X-ray and OIR data. 
}
\label{fig: shallowjetlightcurve}
\end{figure}

\begin{figure} 
\centering
\includegraphics[width=0.5\columnwidth]{figs/GRB221009A_SED_figure_shallowjet.pdf}
\includegraphics[width=0.5\columnwidth]{figs/GRB221009A_SED_figure_shallowjet_noradio.pdf}
\caption{Multi-epoch OIR and X-ray SEDs of GRB 221009A in the structured jet scenario.}
\label{fig: shallowjetSED}
\end{figure}


\subsubsection{Energetics}
%\textcolor{blue}{Text from Paz - use $E_{\gamma,\textrm{iso}}=2\times 10^{52}$. }
{\bf PB: A big advantage of the shallow structure jet scenario suggested above, is that it significantly reduces the energetic requirements relative to steep structure models. [Brendan, what is the earliest time at which we can confidently say the lightcurve evolves in the fashion that matches $a_1$? This will be used to determine an upper limit on $t_{\rm sph}$ and in turn $\theta_{\rm obs}$.] }

{\bf PB: As mentioned in \S \ref{sec: scenario2}, the viewing angle to the burst is directly related to $t_{\rm sph}$. Observationally, the latter is given by the time at which the evolution of the OIR lightcurve transitions to the ... slope and the X-ray to ... We find that $...<t_{\rm obs}<...$ [Brendan, please fill in those numbers]. The result is
\begin{equation}
    \theta_{\rm obs}=\left(\frac{(3-k)E_{\rm kin,iso}(\theta_{\rm obs})}{4\pi A 2^{3-k} c^{5-k}}\right)^{\frac{1}{2k-8}}t_{\rm sph}^{\frac{3-k}{8-2k}}
\end{equation}
which for $k=0$ (as favoured by the lightcurve evolution) implies $...<\theta_{\rm obs}<...$.
An additional angle of importance for the considered structure is $\theta_{\rm c}>\theta_{\rm obs}$ (below which $E_{\rm kin,iso}$ evolves as $\theta^{a_1}$ and above which as $\theta^{a_2}$). Since for a shallow structured jet, the observed angle at any given time evolves with time according to
\begin{eqnarray}
    \theta\!=\!\theta_{\rm obs}\left\{ \begin{array}{ll}(t/t_{\rm sph})^{\frac{3-k}{8-2k-a_1}} & t_{\rm sph}<t<t_{\rm c} ,\\ \\(t_{\rm c}/t_{\rm sph})^{\frac{3-k}{8-2k-a_1}}(t/t_{\rm c})^{\frac{3-k}{8-2k-a_2}}  \quad  & t>t_{\rm c}
\end{array} \right.
\end{eqnarray}
Therefore, $t_{\rm c}$ can be expressed as,
\begin{equation}
    \theta_{\rm c}=\left(\frac{(3-k)E_{\rm kin,iso}(\theta_{\rm obs})}{4\pi A 2^{3-k} c^{5-k}}\right)^{\frac{1}{2k-8+a_1}}t_{\rm c}^{\frac{3-k}{8-2k-a_1}}\theta_{\rm obs}^{\frac{-a_1}{8-2k-a_1}}
\end{equation}
Finally, using $\theta_{\rm obs}, \theta_{\rm c}$, we can express the required (collimated-corrected) energy in the jet considering that no steep break (i.e. traditional jet-break like) has been observed in the lightcurve up to the latest time of observation
\begin{eqnarray}
  &  E_{\rm t}=\frac{\theta(t)^2}{2} E_{\rm kin, iso}(\theta_{\rm obs}) \left(\frac{\theta_{\rm c}}{\theta_{\rm obs}}\right)^{-a_1}\left(\frac{\theta(t)}{\theta_{\rm c}}\right)^{-a_2} %\\
%  &=\frac{1}{2}E_{\rm \gamma,iso}(\theta_{\rm obs}) \theta_{\rm obs}^{\frac{6a_1}{8-a_1}} t_{\rm c}^{\frac{6-3a_1}{a_1-8}-\frac{6-3a_2}{a_2-8}} t^{\frac{6-3a_2}{a_2-8}}
\end{eqnarray}
for $k=0, a_1=0.6, a_2=1.1$, this leads to
\begin{eqnarray}
& E_{\rm t}=4.7\times 10^{52}\mbox{ erg}\left(\frac{E_{\rm \gamma,iso}(\theta_{\rm obs})f(\eta_{\gamma})}{10^{54.5}\mbox{ erg}}\right)^{0.81} \nonumber \\ & \left(\frac{\theta_{\rm obs}}{0.01}\right)^{0.49}  \left(\frac{t_{\rm c}}{0.6\mbox{ d}}\right)^{0.18} \left(\frac{t}{80\mbox{ d}}\right)^{0.39}
\end{eqnarray}
We see that the required energy is more than an order of magnitude smaller than in the standard jet case. Furthermore, notice the shallow increase in the required energy in this shallow jet scenario as a function of time. In other words, the longer no steep jet break is seen in the lightcurve, the greater the difference between the two energy estimates becomes. 
}

%\begin{equation}
%t_{j}= \Big[ \frac{ (3-k) \epsilon_c}{A^{5-k}}\Big]^{1/(3-k)} \theta_c^{(8-2k)/(3-k)},
%\end{equation}
%where $\epsilon_c$ is $dE/d\Omega$ at the jet core and A is defined such that $\rho=A r^{-k}$. \textcolor{purple}{What about gamma-ray efficiency?}






% \textcolor{red}{I think nu_KN is actually indpendent of Gamma...}
%The second constraint is due to the steep slope of \textit{Swift} BAT at $1$ hr. The value of $\Delta\beta_X=0.46\pm0.07$ between XRT and BAT is larger than the change in spectral slope due to Klein-Nishina suppression ($\nu_m<\nu_\textrm{KN}<\nu_c$) where $\Delta\beta_\textrm{KN}=0.3$ for $p=2.2$. Following \cite{Beniamini2015}, we can compute the Klein-Nishina frequency as $\nu_\textrm{KN}\leq\Gamma m_e c^2/(h(1+z)\gamma_m$, where $h$ %$h=H_0/100$ is Planck's constant. We require that $\nu_\textrm{KN}>150$ keV at 0.05 d, which leads to \textcolor{red}{$\Gamma>XXX$} where we have used that $\nu_ma\approx2\times10^{16}$ at 0.05 d, according to our first interpretation (see \S \ref{sec: scenario1}). 



\subsubsection{Rate of events}

\textcolor{blue}{Text from Paz/Yoni - why shallow jets might be more commonly associated with more energetic events.}




\subsubsection{Comparison to other GRBs}

\textcolor{purple}{Need to compare to GRB 130427A... (bright, nearby, lack of jet-break etc). This could also go in the energetics/jet-break section...} 

\textcolor{purple}{What were the GRBs that Simone found? Should they be added to the XRT lightcurve figure showing all long GRBs?}

\begin{figure} 
\centering
\includegraphics[width=0.5\columnwidth]{figs/Figure_6.png}
\includegraphics[width=0.5\columnwidth]{figs/Fermi_hist_221009A_2.pdf}
\caption{Rest-frame afterglow lightcurves in the \textit{Swift} XRT $0.3-10$ keV energy band for a sample of bright long-duration GRBs. 
}
\label{fig: bright_xrt_lightcurve}
\end{figure}

\section{Conclusions}
\label{sec: conclusions}

We have presented an in-depth analysis of the early afterglow of GRB 221009A. \textcolor{purple}{Continue... focus on the observations and speculate as to why they do not work...}

\textcolor{purple}{Need discussion of rates and energetics and focus on this being bright not just because nearby but because one of the most luminous GRBs ever. What do we learn from these bright GRBs which do not have clear jet-breaks? Why are they different? What does a wide jet mean for energetics and RATE? What did we learn from this GRB?}

\textcolor{purple}{need to explain why energy so high
and 
why are Gev bright bursts not showing clear jet-breaks. why jet so wide or structure so shallow compared to garden-variety GRBs.
Paz mentioned hydrodynamic jets are shallower than magnetohydrodynamic and more energetic hydrodynamic jets have shallower energy distributions...}



\acknowledgments

This work made use of data from the NuSTAR mission, a project led by the California Institute of Technology, managed by the Jet Propulsion Laboratory, and funded by the National Aeronautics and Space Administration.  
Based on observations obtained with XMM-Newton, an ESA science mission with instruments and contributions directly funded by ESA Member States and NASA. 
Based on observations obtained with MASTER, MASTER equipment is supported by the Development Program of Lomonosov MSU. 
Based on observations obtained at the international Gemini Observatory, a program of NSF's OIR Lab, which is managed by the Association of Universities for Research in Astronomy (AURA) under a cooperative agreement with the National Science Foundation on behalf of the Gemini Observatory partnership: the National Science Foundation (United States), National Research Council (Canada), Agencia Nacional de Investigaci\'{o}n y Desarrollo (Chile), Ministerio de Ciencia, Tecnolog\'{i}a e Innovaci\'{o}n (Argentina), Minist\'{e}rio da Ci\^{e}ncia, Tecnologia, Inova\c{c}\~{o}es e Comunica\c{c}\~{o}es (Brazil), and Korea Astronomy and Space Science Institute (Republic of Korea). 

The \textit{HST} data used in this work was obtained from the Mikulski Archive for Space Telescopes (MAST). STScI is operated by the Association of Universities for Research in Astronomy, Inc., under NASA contract NAS5-26555. Support for MAST for non-\textit{HST} data is provided by the NASA Office of Space Science via grant NNX09AF08G and by other grants and contracts. 
These results also made use of Lowell Observatory's Lowell Discovery Telescope (LDT), formerly the Discovery Channel Telescope. Lowell operates the LDT in partnership with Boston University, Northern Arizona University, the University of Maryland, and the University of Toledo. Partial support of the LDT was provided by Discovery Communications. LMI was built by Lowell Observatory using funds from the National Science Foundation (AST-1005313). 
This work made use of data supplied by the UK \textit{Swift} Science Data Centre at the University of Leicester. 

This research has made use of the XRT Data Analysis Software (XRTDAS) developed under the responsibility of the ASI Science Data Center (ASDC), Italy. 
This research has made use of the NuSTAR Data Analysis Software (NuSTARDAS) jointly developed by the ASI Space Science Data Center (SSDC, Italy) and the California Institute of Technology (Caltech, USA). 
This research has made use of data and/or software provided by the High Energy Astrophysics Science Archive Research Center (HEASARC), which is a service of the Astrophysics Science Division at NASA/GSFC. 
%We additionally made use of Astropy, a community-developed core Python package for Astronomy \cite{astropy}.

%Based on data obtained from the ESO Science Archive Facility under request number \#639813.
    %acknowledge all instruments used properly!!

%% To help institutions obtain information on the effectiveness of their 
%% telescopes the AAS Journals has created a group of keywords for telescope 
%% facilities.
%
%% Following the acknowledgments section, use the following syntax and the
%% \facility{} or \facilities{} macros to list the keywords of facilities used 
%% in the research for the paper.  Each keyword is check against the master 
%% list during copy editing.  Individual instruments can be provided in 
%% parentheses, after the keyword, but they are not verified.

\vspace{5mm}
\facilities{\textit{Swift}, \textit{NuSTAR}, \textit{XMM-Newton}, \textit{HST}, LDT, Gemini, MASTER}

%% Similar to \facility{}, there is the optional \software command to allow 
%% authors a place to specify which programs were used during the creation of 
%% the manuscript. Authors should list each code and include either a
%% citation or url to the code inside ()s when available.

\software{\texttt{HEASoft 6.29c}, \texttt{XRTDAS}, \texttt{NuSTARDAS}, \texttt{SAS}, \texttt{Dragons}, \texttt{XSPEC v12.11.0} \cite{Arnaud1996}, \texttt{IRAF} \cite{Tody1986}, \texttt{SExtractor} \cite{Bertin1996}, \texttt{Swarp} \cite{Bertin2010}, \texttt{SCAMP} \cite{Bertin2006}, \texttt{Astropy} \cite{astropy}
}

%% Appendix material should be preceded with a single \appendix command.
%% There should be a \section command for each appendix. Mark appendix
%% subsections with the same markup you use in the main body of the paper.

%% Each Appendix (indicated with \section) will be lettered A, B, C, etc.
%% The equation counter will reset when it encounters the \appendix
%% command and will number appendix equations (A1), (A2), etc. The
%% Figure and Table counter will not reset.


==> GRB 221009A Science Format (Final Version) (1)/oldcuttext.tex <==
\textcolor{purple}{Title 2:} 
A wide shallow jet explains GRB 221009A\\
\textcolor{purple}{Title 3:} 
A structured jet to explain the extreme GRB 221009A \\
\textcolor{purple}{Title 4:} 
The long-lived afterglow of GRB221009A (something more empirical and less model dependent)\\
\textcolor{purple}{Title 5:} 
GRB 221009A Afterglow Observations Constrain Its Jet Structure\\
\textcolor{purple}{Title 6:} 
GRB 221009A Afterglow Observations Suggest a Shallow Wide Jet \\ 
\textcolor{purple}{Title 7:}
The long-lived afterglow of GRB 221009A is explained by a shallow structured jet\\
\textcolor{purple}{Title 8:}
The long-lived afterglow of GRB 221009A: evidence for a shallow structured jet\\
\textcolor{purple}{Title 9:}
The long-lived afterglow of GRB 221009A reveals a shallow structured jet\\
\textcolor{purple}{Title 10:}
Multi-wavelength afterglow observations of GRB 221009A reveal a shallow structured jet\\
\textcolor{blue}{I prefer Titles 1, 9, or 10, but do not feel strongly that the others are not equally as acceptable. None stands out to me as the best; though 9 or 10 in which I combined the other ideas seem good to me.}\\ 
\textcolor{red}{I have only received votes for Title 1. (Alexander, Mike, Igor, Rosa, Brad, Erica, Carlos, Roberto, Myself). All comments beyond just saying ``title 1'' have been forwarded to you. }
}


==> authors.tex <==




% \author{
% B. O'Connor$^{1,2,3,4\ast}$, 
% E. Troja$^{5,6}$, 
% G. Ryan$^{7}$,
% P. Beniamini$^{8,9}$,
% H. van Eerten$^{10}$, \\
% J. Granot$^{8,9,1}$,
% S. Dichiara$^{11}$,
% R. Ricci$^{12,13}$,
% V. Lipunov$^{14}$, \\
% J. Gillanders$^{5}$, 
% R. Gill$^{15}$,
% M. Moss$^{1}$,
% S. Anand$^{16}$, \\
% I. Andreoni$^{4,17}$, 
% R. L. Becerra$^{18}$,
% D. A. H. Buckley$^{19}$,
% N. R. Butler$^{20}$, \\
% S. B. Cenko$^{4,17}$, 
%  A. Chasovnikov$^{14}$, 
% J. Durbak$^{3,4}$,
% C. Francile$^{21,22}$,  \\
% E. Hammerstein$^{3}$,
% A. J. van der Horst$^{1}$,
% M. Kasliwal$^{16}$, \\
% C. Kouveliotou$^{1,2}$,
% A. S. Kutyrev$^{3,4}$,
% W. H. Lee$^{23}$, \\
% G. Srinivasaragavan$^{3}$,
% V. Topolev$^{14}$,
% A. M. Watson$^{23}$,
% K. Zhirkov$^{14}$ \\ 
% \\
% \footnotesize{$^{1}$ Department of Physics, The George Washington University, 725 21st Street NW, Washington, DC 20052, USA } \\ 
% \footnotesize{$^{2}$ Astronomy, Physics and Statistics Institute of Sciences (APSIS), The George Washington University, Washington, DC 20052, USA }\\
% \footnotesize{$^{3}$ Department of Astronomy, University of Maryland, College Park, MD 20742-4111, USA }\\
% \footnotesize{$^{4}$ Astrophysics Science Division, NASA Goddard Space Flight Center, 8800 Greenbelt Rd, Greenbelt, MD 20771, USA }\\
% \footnotesize{$^{5}$ Department of Physics, University of Rome - Tor Vergata, via della Ricerca Scientifica 1, 00100 Rome, IT }\\
% \footnotesize{$^{6}$ \textcolor{red}{INAF} }\\
% \footnotesize{$^{7}$ Perimeter Institute for Theoretical Physics, 31 Caroline St. N., Waterloo, ON, N2L 2Y5, Canada }\\
% \footnotesize{$^{8}$ Department of Natural Sciences, The Open University of Israel, P.O Box 808, Ra’anana 4353701, Israel }\\
% \footnotesize{$^{9}$ Astrophysics Research Center of the Open university (ARCO), The Open University of Israel, P.O Box 808, Ra’anana 4353701, Israel }\\
% \footnotesize{$^{10}$ Physics Department, University of Bath, Claverton Down, Bath BA2 7AY, United Kingdom}\\
% \footnotesize{$^{11}$ Department of Astronomy and Astrophysics, The Pennsylvania State University, 525 Davey Lab, University Park, PA 16802, USA} \\
% \footnotesize{$^{12}$ Istituto Nazionale di Ricerche Metrologiche, I-10135 Torino, Italy}\\
% \footnotesize{$^{13}$ INAF-Istituto di Radioastronomia, via Gobetti 101, I-40129 Bologna, Italy}\\
% \footnotesize{$^{14}$ Department of Physics, Sternberg Astronomical Institute, Lomonosov Moscow State University, 119234, Universitetsky, 13, Moscow, Russia} \\
% \footnotesize{$^{15}$ Instituto de Radioastronom\'ia y Astrof\'isica, Universidad Nacional Aut\'onoma de M\'exico, Antigua Carretera a P\'atzcuaro} \\ \footnotesize{$\#$ 8701, Ex-Hda. San Jos\'e de la Huerta, Morelia, Michoac\'an, C.P. 58089, M\'exico } \\
% \footnotesize{$^{16}$ Division of Physics, Mathematics and Astronomy, California Institute of Technology, Pasadena, CA 91125, USA}\\
% \footnotesize{$^{17}$ Joint Space-Science Institute, University of Maryland, College Park, MD 20742, USA}\\
% \footnotesize{$^{18}$ Instituto de Ciencias Nucleares, Universidad Nacional Aut\'onoma de M\'exico, Apartado Postal 70-264, 04510 M\'exico, CDMX, Mexico }\\
% \footnotesize{$^{19}$ South African Astrophysical Observatory, PO Box 9, 7935 Observatory, Cape Town, South Africa}\\
% \footnotesize{$^{20}$ School of Earth and Space Exploration, Arizona State University, Tempe, AZ 85287, USA }\\
% \footnotesize{$^{21}$ Observatorio Astronomico Felix Aguilar (OAFA), Avda Benavides 8175, Rivadavia, El Leonsito, San Juan 5400, Argentina} \\
% \footnotesize{$^{22}$ Facultad de Ciencias Exactas Fisicas y Naturales, San Juan National University, Casilla de Correo 49, San Juan 5400, Argentina}\\
% \footnotesize{$^{23}$ Instituto de Astronom\'ia, Universidad Nacional Aut\'onoma de M\'exico, Apartado Postal 70-264, 04510 M\'exico, CDMX, Mexico }\\
% \footnotesize{$^\ast$Correspondence to: oconnorb@gwmail.gwu.edu}
% }


% \author{
% B. O'Connor$^{1,2,3,4\ast}$, 
% E. Troja$^{5,6}$, 
% G. Ryan$^{7}$,
% P. Beniamini$^{8,9}$,
% H. van Eerten$^{10}$, \\
% J. Granot$^{8,9,1}$, 
% S. Dichiara$^{11}$,
% R. Ricci$^{12,13}$,
% V. Lipunov$^{14}$, 
% J. Gillanders$^{5}$, 
% R. Gill$^{15}$, \\
% M. Moss$^{1}$, 
% S. Anand$^{16}$, 
% I. Andreoni$^{4,17}$, 
% R. L. Becerra$^{18}$, 
% D. A. H. Buckley$^{19}$,\\
% N. R. Butler$^{20}$, 
% S. B. Cenko$^{4,17}$, 
%  A. Chasovnikov$^{14}$, 
% J. Durbak$^{3,4}$, 
% C. Francile$^{21,22}$,   \\
% E. Hammerstein$^{3}$,
% A. J. van der Horst$^{1}$,
% M. Kasliwal$^{16}$, 
% C. Kouveliotou$^{1,2}$, \\
% A. S. Kutyrev$^{3,4}$,  
% W. H. Lee$^{23}$, 
% G. Srinivasaragavan$^{3}$, 
% V. Topolev$^{14}$, \\
% A. M. Watson$^{23}$,
% K. Zhirkov$^{14}$ \\
% \\
% \scriptsize{$^{1}$ Department of Physics, The George Washington University, 725 21st Street NW, Washington, DC 20052, USA } \\ 
% \scriptsize{$^{2}$ Astronomy, Physics and Statistics Institute of Sciences (APSIS), Washington, DC 20052, USA }\\
% \scriptsize{$^{3}$ Department of Astronomy, University of Maryland, College Park, MD 20742-4111, USA }\\
% \scriptsize{$^{4}$ Astrophysics Science Division, NASA Goddard Space Flight Center, 8800 Greenbelt Rd, Greenbelt, MD 20771, USA }\\
% \scriptsize{$^{5}$ Department of Physics, University of Rome - Tor Vergata, via della Ricerca Scientifica 1, 00100 Rome, IT }\\
% \scriptsize{$^{6}$ INAF - Istituto di Astrofisica e Planetologia Spaziali, via Fosso del Cavaliere 100, 00133 Rome, Italy} \\
% \scriptsize{$^{7}$ Perimeter Institute for Theoretical Physics, 31 Caroline St. N., Waterloo, ON, N2L 2Y5, Canada }\\
% \scriptsize{$^{8}$ Department of Natural Sciences, The Open University of Israel, P.O Box 808, Ra’anana 4353701, Israel }\\
% \scriptsize{$^{9}$ Astrophysics Research Center of the Open university (ARCO), P.O Box 808, Ra’anana 4353701, Israel }\\
% \scriptsize{$^{10}$ Physics Department, University of Bath, Claverton Down, Bath BA2 7AY, United Kingdom}\\
% \scriptsize{$^{11}$ The Pennsylvania State University, 525 Davey Lab, University Park, PA 16802, USA} \\
% \scriptsize{$^{12}$ Istituto Nazionale di Ricerche Metrologiche, I-10135 Torino, Italy}\\
% \scriptsize{$^{13}$ INAF - Istituto di Radioastronomia, via Gobetti 101, I-40129 Bologna, Italy}\\
% \scriptsize{$^{14}$ Sternberg Astronomical Institute, Lomonosov Moscow State University, 119234, Universitetsky, 13, Moscow, Russia} \\
% \scriptsize{$^{15}$ Instituto de Radioastronom\'ia y Astrof\'isica, Universidad Nacional Aut\'onoma de M\'exico, Antigua Carretera } \\ 
% \scriptsize{a P\'atzcuaro $\#$ 8701, Ex-Hda. San Jos\'e de la Huerta, Morelia, Michoac\'an, C.P. 58089, M\'exico } \\
% \scriptsize{$^{16}$ Division of Physics, Mathematics and Astronomy, California Institute of Technology, Pasadena, CA 91125, USA}\\
% \scriptsize{$^{17}$ Joint Space-Science Institute, University of Maryland, College Park, MD 20742, USA}\\
% \scriptsize{$^{18}$ Instituto de Ciencias Nucleares, Universidad Nacional Aut\'onoma de M\'exico, %Apartado Postal 70-264, 
% 04510 M\'exico, CDMX, Mexico}\\
% \scriptsize{$^{19}$ South African Astrophysical Observatory, PO Box 9, 7935 Observatory, Cape Town, South Africa}\\
% \scriptsize{$^{20}$ School of Earth and Space Exploration, Arizona State University, Tempe, AZ 85287, USA }\\
% \scriptsize{$^{21}$ Observatorio Astronomico Felix Aguilar (OAFA), %Avda Benavides 8175, Rivadavia, El Leonsito, 
% San Juan 5400, Argentina} \\
% \scriptsize{$^{22}$ Facultad de Ciencias Exactas Fisicas y Naturales, San Juan National University, San Juan 5400, Argentina}\\
% \scriptsize{$^{23}$ Instituto de Astronom\'ia, Universidad Nacional Aut\'onoma de M\'exico, 04510 M\'exico, CDMX, Mexico }\\
% \scriptsize{$^\ast$Correspondence to: oconnorb@gwmail.gwu.edu}
% }



==> custom-acronyms.tex <==

\newcommand\aj{AJ}%        % Astronomical Journal 
\newcommand\psj{PSJ}%       % Planetary Science Journal
\newcommand\araa{ARA\&A}%  % Annual Review of Astron and Astrophys 
\newcommand\apj{ApJ}%    % Astrophysical Journal 
\newcommand\apjl{ApJL}     % Astrophysical Journal, Letters 
\newcommand\apjs{ApJS}%    % Astrophysical Journal, Supplement 
\newcommand\ao{ApOpt}%   % Applied Optics 
\newcommand\apss{Ap\&SS}%  % Astrophysics and Space Science 
\newcommand\aap{A\&A}%     % Astronomy and Astrophysics 
\newcommand\aapr{A\&A~Rv}%  % Astronomy and Astrophysics Reviews 
\newcommand\aaps{A\&AS}%    % Astronomy and Astrophysics, Supplement 
\newcommand\azh{AZh}%       % Astronomicheskii Zhurnal 
\newcommand\baas{BAAS}%     % Bulletin of the AAS 
\newcommand\icarus{Icarus}% % Icarus
\newcommand\jaavso{JAAVSO}  % The Journal of the American Association of Variable Star Observers
\newcommand\jrasc{JRASC}%   % Journal of the RAS of Canada 
\newcommand\memras{MmRAS}%  % Memoirs of the RAS 
\newcommand\mnras{MNRAS}%   % Monthly Notices of the RAS 
\newcommand\pra{PhRvA}% % Physical Review A: General Physics 
\newcommand\prb{PhRvB}% % Physical Review B: Solid State 
\newcommand\prc{PhRvC}% % Physical Review C 
\newcommand\prd{PhRvD}% % Physical Review D 
\newcommand\pre{PhRvE}% % Physical Review E 
\newcommand\prl{PhRvL}% % Physical Review Letters 
\newcommand\pasp{PASP}%     % Publications of the ASP 
\newcommand\pasj{PASJ}%     % Publications of the ASJ 
\newcommand\qjras{QJRAS}%   % Quarterly Journal of the RAS 
\newcommand\skytel{S\&T}%   % Sky and Telescope 
\newcommand\solphys{SoPh}% % Solar Physics 
\newcommand\sovast{Soviet~Ast.}% % Soviet Astronomy 
\newcommand\ssr{SSRv}% % Space Science Reviews 
\newcommand\zap{ZA}%       % Zeitschrift fuer Astrophysik 
\newcommand\nat{Nature}%  % Nature 
\newcommand\iaucirc{IAUC}% % IAU Cirulars 
\newcommand\aplett{Astrophys.~Lett.}%  % Astrophysics Letters 
\newcommand\apspr{Astrophys.~Space~Phys.~Res.}% % Astrophysics Space Physics Research 
\newcommand\bain{BAN}% % Bulletin Astronomical Institute of the Netherlands 
\newcommand\fcp{FCPh}%   % Fundamental Cosmic Physics 
\newcommand\gca{GeoCoA}% % Geochimica Cosmochimica Acta 
\newcommand\grl{Geophys.~Res.~Lett.}%  % Geophysics Research Letters 
\newcommand\jcp{JChPh}%     % Journal of Chemical Physics 
\newcommand\jgr{J.~Geophys.~Res.}%     % Journal of Geophysics Research 
\newcommand\jqsrt{JQSRT}%   % Journal of Quantitiative Spectroscopy and Radiative Trasfer 
\newcommand\memsai{MmSAI}% % Mem. Societa Astronomica Italiana 
\newcommand\nphysa{NuPhA}%     % Nuclear Physics A 
\newcommand\physrep{PhR}%       % Physics Reports 
\newcommand\physscr{PhyS}%        % Physica Scripta 
\newcommand\planss{Planet.~Space~Sci.}%  % Planetary Space Science 
\newcommand\procspie{Proc.~SPIE}%      % Proceedings of the SPIE 
\newcommand\actaa{AcA}%  % Acta Astronomica
\newcommand\caa{ChA\&A}%  % Chinese Astronomy and Astrophysics
\newcommand\cjaa{ChJA\&A}%  % Chinese Journal of Astronomy and Astrophysics
\newcommand\jcap{JCAP}%  % Journal of Cosmology and Astroparticle Physics
\newcommand\na{NewA}%  % New Astronomy
\newcommand\nar{NewAR}%  % New Astronomy Review
\newcommand\pasa{PASA}%  % Publications of the Astron. Soc. of Australia
\newcommand\rmxaa{RMxAA}%  % Revista Mexicana de Astronomia y Astrofisica

%% added feb 9, 2016
\newcommand\maps{M\&PS}% Meteoritics and Planetary Science
\newcommand\aas{AAS Meeting Abstracts}% American Astronomical Society Meeting Abstracts
\newcommand\dps{AAS/DPS Meeting Abstracts}% American Astronomical Society/Division for Planetary Sciences Meeting Abstracts


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%% Some Useful Abbreviations %%%%% 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\cxo}{{\it Chandra~}}
\newcommand{\rxte}{{\it RXTE~}}
\newcommand{\asca}{{\it ASCA~}}
\newcommand{\rosat}{{\it ROSAT~}}
\newcommand{\einstein}{{\it EINSTEIN}}
\newcommand{\ginga}{{\it GINGA}}
\newcommand{\bbxrt}{{\it BBXRT}}
\newcommand{\suzaku}{{\it Suzaku}}
\newcommand{\xmm}{{\it XMM-Newton~}}
\newcommand{\sax}{{\it BeppoSAX}}
\newcommand{\ec}{$\eta$~Car}
\newcommand{\glast}{{\it GLAST}}
\newcommand{\swift}{{\it Swift~}}
\newcommand{\integral}{\textit{INTEGRAL~}}
\newcommand{\nustar}{\textit{NuSTAR~}}
\newcommand{\hst}{{\it HST}}
\newcommand{\ms}{$M_{\odot}$}
\newcommand{\rs}{$R_{\odot}$}
\newcommand{\ls}{$L_{\odot}$}
\newcommand{\kms}{km~s$^{-1}$}
\newcommand{\fluxcgs}{ergs~s$^{-1}$~cm$^{-2}$}
\newcommand{\lumcgs}{ergs~s$^{-1}$}
\def\gtrsim{\mathrel{\hbox{\rlap{\hbox{\lower4pt\hbox{$\sim$}}}\hbox{$>$}}}}

\def \arcsec {\hbox{$^{\prime\prime}$}}
\def\eg#1{\textcolor{red}{#1}}


==> obs.tex <==

\noindent \textbf{Observations and Data Analysis} 

\noindent \textbf{\textit{X-ray Observations}} 

\noindent \textit{Swift} 

The \textit{Neil Gehrels Swift Observatory} X-ray Telescope (XRT) began settled observations of GRB 221009A at 14:13:30 UT on 2022-10-09, approximately 143 s after the \textit{Swift}/BAT trigger and 3198 s after the \textit{Fermi}/GBM trigger. The afterglow was clearly detected and localized to RA, DEC (J2000) = $19^{h}13^m 03^{s}.85$, $+\ang{19;46;22.7}$ with an accuracy of \ang{;;3.5} (90$\%$ confidence level) \cite{Evans2009}. 
We obtained the XRT lightcurve from the \textit{Swift}-XRT GRB Lightcurve Repository\footnote{\url{https://www.swift.ac.uk/xrt_curves/}}. The lightcurve has been shifted in time by 3198 s to apply the \textit{Fermi}/GBM trigger as $T_0$. 
We further used the XRT Repository tools to create time-sliced spectra, in both windowed timing (WT) and photon counting (PC) modes, at multiple epochs for use in modeling the broadband spectral energy distribution of the GRB afterglow. 

\noindent \textit{XMM-Newton} 

We observed GRB 221009A using \textit{XMM-Newton} on November 10, 2022 through Directory's Discretionary Time (DDT; PI: Troja), corresponding to 32.72 d after the GRB trigger. The observations were performed in full frame mode using the thin filter, and lasted for 100 ks with a mid-time of 32.72 d. The data were reduced and analyzed using tasks with the Science Analysis System (\texttt{SAS v18.0.0}) software. We used a circular region of $60\arcsec$ to extract source photons. The background photons were taken from a nearby source-free circular region of $60\arcsec$.  We grouped the spectrum to a minimum of 1 count per bin and obtained the response matrix and ancillary response files using the \texttt{rmfgen} and \texttt{arfgen} tasks. 

\noindent \textit{NuSTAR} 

\textit{NuSTAR} observed GRB 221009A on five epochs at mid-times of 1.82, 5.92, 10.72, 23.93, and 31.95 d after the \textit{Fermi} trigger (see Table \ref{tab:Xobservations}). These data were obtained under two DDT programs (co-PIs: Margutti and Racusin; PI: Troja). The initial observations were first reported by \cite{GCN32695,GCN32788}. \textit{NuSTAR} is comprised of two identical focal plane modules, FPMA and FPMB, covering the $3-79$ keV energy range. The GRB afterglow is detected in each epoch. We reduced the data using the \textit{NuSTAR} Data Analysis Software pipeline (\texttt{NuSTARDAS}) within \texttt{HEASoft v6.29c}. The data were processed using \texttt{nupipeline}, and then lightcurves and spectra were extracted using \texttt{nuproducts}. In the initial observation at 1.8 d, source spectra were extracted from a 100\arcsec{} radius region centered on the transient. The background was similarly extracted from a 100\arcsec{} radius source-free region. For each of the latter observations, we used a 60\arcsec{} radius for both source and background regions. 


\noindent \textbf{\textit{Optical/Near-Infrared Observations}}

\noindent \textit{MASTER}

MASTER is a system of wide-field fully robotic 40-cm telescopes with identical scientific equipment and real-time auto-detection at every observatory \cite{Lipunov2004,Lipunov2010,Kornilov2012}. The MASTER telescopes are MASTER-Amur, -Tunka, -Ural, -Kislovodsk, -Tavrida (Russia), -SAAO (South Africa), -IAC (Spain), -OAFA (Argentina). The MASTER Global Robotic Net \cite{Lipunov2010} began observing GRB 221009A using MASTER-SAAO on 2022-10-09 at 17:33:54 UT, corresponding to 0.18 d after the \textit{Fermi} trigger. The MASTER auto-detection system discovered the optical counterpart, MASTER OT J191303.43+194623.1 \cite{GCN32634}, as a transient in the initial image. The observations were obtained in the \textit{clear} ($C$) filter. Further observations were obtained with MASTER-OAF starting on 2022-10-09 at 23:56:38 UT, corresponding to 0.46 d after the trigger (see Table \ref{tab:MASTERobservations}). Aperture photometry was calibrated using 20 reference stars, and we applied a further correction to convert to the AB magnitude system. We note that earlier observations by MASTER-Tunka and MASTER-Amur, beginning at 93 s after the \textit{Fermi} trigger (2022-10-09 14:11:50 UT), were severely impacted by clouds and were unable to detect the source. 


\noindent \textit{COATLI}

We observed the field of GRB 221009A with the 50-cm COATLI telescope at the Observatorio Astronómico Nacional on the Sierra de San Pedro Mártir in Baja California, México, and the HUITZI f/8 imager. We observed in $griz$ filters similar to Pan-STARRS1 (hereafter PS1; \cite{Chambers2016}) and took multiple 30 second images each night. The images were reduced using a custom pipeline, and then stacked to create a final image. Photometry was calculated for each stack using PSF fitting and calibrated relative to the PS1 catalog using all available field stars.

\noindent \textit{Gemini}

Target of Opportunity (ToO) observations of GRB 221009A were performed with the 8.1-m Gemini South Telescope in Cerro Pachon, Chile using GMOS-S and Flamingos-2 (hereafter F2) under two DDT programs (GS-2022B-DD-104, PI: O'Connor; GS-2022B-DD-103, PI: Rastinejad). The observations were first reported by \cite{GCN32749,GCN32750,GCN32860}.
Data were obtained at 4.4, 17.4 and 25.4 d. The observations were carried out in the $i$ filter with GMOS-S, and $J$, $H$, and $K_s$ filters with F2 (see Table \ref{tab:Optobservations}). We reduced and analyzed these data using the \texttt{DRAGONS}\footnote{\url{https://dragons.readthedocs.io/}} software \cite{Labrie2019}. The afterglow is clearly detected in each observation. 
%\textcolor{purple}{Using the initial images, we localize the GRB to RA, DEC (J2000) = $19^{h}13^m 03^{s}.85$, $+\ang{19;46;22.7}$ with an accuracy of $XXX\arcsec$.} 
We performed PSF photometry using \texttt{SExtractor} \cite{Bertin1996} and \texttt{PSFEx} \cite{Bertin2013}. The photometry was calibrated using nearby point-sources in the Two Micron All Sky Survey (2MASS) catalog \cite{Skrutskie2006}. We then applied a standard conversion between the Vega and AB magnitude systems.

\noindent \textit{Lowell Discovery Telescope} 

We obtained ToO observations with the Large Monolithic Imager (LMI) mounted on the 4.3-meter LDT at the Lowell Observatory in Happy Jack, AZ starting at 3.6 d after the GRB and continuing observations for 8 weeks under multiple programs (program PIs: Cenko, Hammerstein, O'Connor), see Table \ref{tab:Optobservations}. We first reported the initial observations in \cite{GCN32739,GCN32799}. The data were reduced with a custom pipeline \cite{Toy2016} that makes use of standard CCD reduction techniques in the IRAF\footnote{IRAF is distributed by the National Optical Astronomy Observatory, which is operated by the Association of Universities for Research in Astronomy (AURA) under cooperative agreement with the National Science Foundation (NSF).} package including bias subtraction, flat-fielding, and cosmic ray rejection \cite{vanDokkum2001}. Photometry was performed in the same manner as for Gemini, and calibrated against stars in the PS1 catalog. % (Pan-STARRS1, hereafter PS1) \cite{Chambers2016}. 

\noindent \textit{Palomar 200-inch}

We obtained data with the Palomar 200-in Wide InfraRed Camera (WIRC) in the $J$, $H$, and $K_s$ bands starting at 18:26:50 UT on 2022-11-02, taking 9 dithered images in each band for a total exposure of 495 s in $J$ and 330 s in $H$ and $K_s$ (Table \ref{tab:Optobservations}). The data were reduced using a \texttt{Python}-based reduction pipeline that uses standard image reduction techniques \cite{De2020}. The dithered images in each filter were astrometrically aligned and stacked to create a single composite image. The pipeline performed photometric calibration using the 2MASS point source catalog. 


\noindent \textit{Other Optical and Near-Infrared Data} 


We analyzed publicly available \textit{HST} observations (PI: Levan) obtained in WFC3/UVIS $F625W$ and $F775W$ filters and WFC3/IR $F098M$, $F125W$, and $F160W$ filters. The data were reduced and analyzed as detailed in \cite{OConnor2022}. 

We further supplemented our dataset with optical and infrared observations reported in GCN circulars \cite{GCN.32769, GCN.32818, GCN.32684, GCN.32743, GCN.32752, GCN.32652, GCN.32755, GCN.32646, GCN.32804, GCN.32678, GCN.32811, GCN.32758, GCN.32803, GCN32765hostz, GCN.32670,GCN.32662, GCN.32852, GCN.32795, GCN.32809, GCN.32753,GCN.32771, GCN.32756, GCN.32709}. 

%\textit{HST} observations were carried out at 29.7, 40.6, and 55.7 d after the GRB trigger (see Table \ref{tab:Optobservations}). Data were acquired in the WFC3/UVIS $F625W$ and $F775W$ filters and WFC3/IR $F098M$, $F125W$, and $F160W$ filters through a DDT request (PI: Levan). The initial observation was first reported by \cite{GCN32921}. 
%We reduced the data using standard procedures within the \texttt{DrizzlePac} package \cite{Gonzaga2012}. The source is clearly detected in all filters with a marginal extension of the source to the NE in the infrared filters, likely due to the underlying host galaxy at $z=0.1505$. The galaxy is not identified in the initial WFC3/UVIS images, likely due to extinction from the Milky Way, but is found in the deep $F625W$ images from 2022 December 4. %\textcolor{purple}{Based on these \textit{HST} images we derive a more precise localization of the GRB to RA, DEC = XXX....}. 
%We performed photometry of the source complex using a circular region of radius $0.3\arcsec$ centered on the transient. The zeropoints were taken from the photometry keywords in the image headers. %These measurements include the unknown host contribution. 



\noindent \textit{\textbf{Radio Observations}}

The Australia Telescope Compact Array (ATCA) observed GRB 221009A as part of the DDT project CX515 on 2022-10-15, 2022-10-24, 2022-11-04, 2022-11-19, 2022-12-28, and 2023-01-27 (Table \ref{tab:Radioobservations}). The initial observation at 5.8 d after the GRB was first reported by \cite{GCN32763,GCN32766}. In the first two epochs, the three pairs of Intermediate Frequencies (IFs) were used 16.7/21.2 GHz, 33/35 GHz, 45/47 GHz and in the next two only 16.7/21.2 GHz and 33/35 GHz were used. In the last two epochs, corresponding to 80 and 110 d after the GRB, observations were obtained at 5.5 and 9 GHz. In all observing runs the array operated in continuum mode with the Compact Array Broadband Backend using 2048 channels over 2-GHz bandwidth per IF. The radio sources used as bandpass, primary and phase calibrator were 1921-293, 1934-638 and 1923+210, respectively. The phase calibrator was also used for reference pointing checks every hour. Standard procedures in the data reduction software package \texttt{MIRIAD}
% (\textcolor{red}{CITE})
\cite{Sault1995_MIRIAD}
were used to flag, calibrate the complex gains and image the phase calibrator and target. A robustness parameter value of two was used, and a 6-km baseline antenna was deselected during imaging.

We further used the \texttt{MIRIAD} task \texttt{calred} on the phase calibrator 1923+210 to test for phase decorrelation due to atmospheric turbulence. The task \texttt{calred} estimates the triple product amplitude, and, therefore, is unaffected by atmospheric turbulence induced phase decorrelation effects. A comparison between triple product and map flux density can be used to estimate the decorrelation factor. We found no significant decorrelation in the flux densities measured on the I-stokes restored maps, apart from three frequencies (35, 45 and 47 GHz) in Epoch 2 (2022-10-24; 14.7 d post-burst) at a level of 19\%, 14\% and 12\% respectively and on Epoch 4 (2022-11-19; 41 d post-burst) at 33 and 35 GHz of 4\% and 3\%, respectively. 
Seeing monitor data show a maximum rms path length of 
$\approx$500 microns during our second epoch (14.7 d) which, for a calibration interval of 15 min, is expected to result in a 25-50\% amplitude decorrelation above 30 GHz. Due to the large uncertainties, we exclude this epoch from our spectral analysis. 
No significant decorrelation is expected for observations at frequencies below 10 GHz (e.g., 80 and 110 d). 

The resulting flux densities and 5$\sigma$ upper limits are presented in Table \ref{tab:Radioobservations}. The errors are derived from summing in quadrature the statistical and systematic uncertainty (map rms and 5\% of the total flux as residual of gain calibration, respectively).



We supplemented our radio observations with data reported in GCN circulars  \cite{GCN32653,GCN32655,GCN32949,GCN32676}. 


==> oldapj.tex <==

\textcolor{purple}{Below are the contents of the ApJ Version as of 1/18/22.}

\begin{sciabstract}
 ABSTRACT GOES HERE
\end{sciabstract}

\section*{Introduction}
\label{sec: intro}


Gamma-ray bursts (GRBs) are among the peculiar and enigmatic phenomena in the universe. They consist of brief flashes of gamma-ray radiation detected by low orbit satellites with an all sky rate of about 1 or 2 events per day. Their fluence (flux integrated over the duration of the gamma-ray signal) ranges between few times $10^{-7}$ to $10^{-4}$ erg cm$^{-2}$ in the $10-1000$ keV energy band (as observed by Fermi/GBM; \cite{vonKienlin2020}).
They are grouped into two main sub-classes based on their duration and spectral hardness \cite{Kouveliotou1993}. Long duration GRBs (lasting $\gtrsim 2$ s) are produced by the core-collapse of rapidly-rotating massive stars (collapsars) \cite{Woosley2006}.
%\textcolor{purple}{Link supernova detections from nearby GRBs to how we know they are produced by massive-stars... no more than 1 sentence on environment/star forming regions...}


These explosions display a broad range of gamma-ray energy between $E_{\gamma,\textrm{iso}}=10^{48-54}$ erg. Due to their extreme energy, they are detectable by high-energy satellites in the early Universe ($z\approx 2-4$), with only the most energetic detectable further back in time. 

Despite the large number of GRBs detected so far, only few of them were observed at very high energies (VHE; $>$100 GeV): GRB 180720B \cite{Abdalla2019}, GRB 190114C \cite{Magic2019}, GRB 190829A \cite{Hess2021} and GRB 201216C
% (Blanch O. et al., 2020, GCN Circ., 29075, 1).
\cite{Blanch2020GCN}.
The study of this signal can provides key information about the nature of the emission and the radiative processes in play. %\textcolor{red}{(This paper states 201216C is the fith, so are we missing one? https://arxiv.org/pdf/2204.05811.pdf)}\textcolor{blue}{it really depends if you consider also 201015A or not. but that was reported as a tentative detection https://gcn.gsfc.nasa.gov/gcn3/28659.gcn3}

In this paper we present an analysis of the multi-wavelength observations obtained for the \textit{Swift} and \textit{Fermi} detected GRB 221009A. The combination of its close proximity ($z=0.1505$; \cite{GCN32648xshooterz}), and extreme energetics ($E_{\gamma,\textrm{iso}}\approx2\times 10^{54}$ erg, 10-1000 keV; \cite{GCN32642}) led to GRB 221009A being the brightest GRB ever observed in nearly 55 years of observations (with a measured fluence that is more than 1 orders of magnitude brighter than GRB 130427A, the second brightest event observed by \textit{Fermi} so far). In addition, GRB 221009A broke the record for highest energy photon detected from a GRB (18 TeV; \cite{GCN32677}), and is only the fifth GRB associated with very high energy (VHE; $>100$ GeV) photons \cite{Abdalla2019,Magic2019,Hess2021}. A claim of a 250 TeV photon-like air shower associated to this GRB was made Carpet-2 \cite{ATel15669}, but later refuted due to a coincident Galactic TeV source \cite{ATel15675}.

Nearby events represent a unique tool to probe theoretical models of multi-wavelength afterglow emission up to very high energy. The standard paradigm (e.g., fireball model; \cite{Rees1992}) features a forward shock (FS) that amplifies the magnetic field and accelerates the electrons in the shocked circumburst medium to a relativistic power-law energy distribution, which then cool via synchrotron radiation (e.g., \cite{Granot2002}. Unless the outflow is highly magnetized as it is decelerated by the external medium, this deceleration is mediated by a reverse shock (RS) that forms and travels back into the ejecta (e.g., \cite{Kobayashi2000}).

 %Inverse Compton (IC) effects should also be taken into account in the parametrization of these radiative processes in order to have a self consistent modeling (...). 
Low redshift events provide a unique probe of emission processes not detectable at larger distances.
In point of fact, inverse Compton (IC) could be recognized as the mechanism responsible for the VHE TeV emission in recent GRBs (e.g., \cite{Abdalla2019, Magic2019}). This component can only be seen at low redshift due to the effect of the extragalactic background scattering \cite{Franceschini2008, Dominguez2011, Gilmore2012, Finke2022}. The proximity of GRB 221009A combined with its outstanding brightness provide us with a once-in-a-lifetime opportunity to constrain the physics of the afterglow and the jet structure of a nearby collapsar GRB.

We present observations optical and infrared obtained with MASTER, the Lowell Discovery Telescope (LDT), Palomar 200-inch (P200), Gemini-South, \textit{Hubble Space Telescope} (\textit{HST}), X-ray observations with \textit{XMM-Newton} and \textit{NuSTAR}, and radio observations from the Australia Telescope Compact Array (ATCA). We interpret the observed multi-wavelength emission as originating from the combination of a reverse- and forward-shock (RS and FS, respectively).


The paper is outlined as follows: \textcolor{purple}{Fill in once we have a final structure of the paper...}

In this work, we adopt a standard $\Lambda$-CDM cosmology \cite{Planck18}. Confidence intervals are expressed at the $1\sigma$ level, and upper limits at $3\sigma$. We apply the convention $F_\nu\propto t^{\alpha}\nu^{\beta}$ throughout. 

\textcolor{purple}{Make sure FS, RS, OIR is all defined in the right place...}


\section{Observations and Data Reduction}
\label{sec: observations}

\subsection{Prompt gamma-rays}


GRB 221009A triggered \textit{Fermi} GBM \cite{GCN32636,GCN32642} and \textit{Fermi} LAT \cite{GCN32658}, among many other high-energy satellites (\textit{INTEGRAL}, \textit{Konus-Wind}, \textit{AGILE}, \textit{SRG}, \textit{GRBAlpha}) \cite{GCN32660,GCN32663,GCN32668, GCN32685, GCN32650} on 2022-10-09 at 13:16:59 UT (hereafter referred to as $T_0$). Due to an issue with the \textit{Fermi} automatic notice, the GRB was not identified until $\sim$ 1 hour later when, after exiting the SAA, \textit{Swift} BAT triggered on the afterglow \cite{GCN32632}. 

The GRB emission had a duration of a few hundred seconds, with multiple emission episodes. Due to the GRB's extreme brightness, the majority of satellites were saturated during the main emission episode. A lower limit to the GRB fluence was reported for \textit{Fermi} GBM as $\sim2.9\times 10^{-2}$ erg cm$^{-2}$ s$^{-1}$ in the 10-1000 keV energy band \cite{GCN32642}, \textit{Konus-Wind} reported $\sim5.2\times 10^{-2}$ erg cm$^{-2}$ s$^{-1}$ (20 keV - 10 MeV) \cite{GCN32668}, and \textit{INTEGRAL} determined $\sim1.3\times 10^{-2}$ erg cm$^{-2}$ s$^{-1}$ (75 keV - 1 MeV) \cite{GCN32660}. Despite these estimates being lower limits, this event is the brightest GRB ever detected by almost two orders of magnitude. At the putative redshift of $z=0.1505$ \cite{GCN32648xshooterz,GCN32686GTCz,GCN32765hostz}, these values correspond to an isotropic equivalent energy in the range $8\times 10^{53}$ erg (75 keV - 1 MeV) to $3\times 10^{54}$ erg (20 keV - 10 MeV), among a short list of the most energetic GRBs to date \cite{Atteia2017} and very similar to GRB 160625B \cite{Zhang2018}. 






\subsection{\textit{Swift}}
\label{sec: Swift}

The \textit{Swift} X-ray Telescope (XRT) began settled observations of GRB 221009A at 14:13:30 UT on 2022-10-09, approximately 143 s after the \textit{Swift}/BAT trigger and 3198 s after the \textit{Fermi}/GBM trigger. The afterglow was clearly detected and localized to RA, DEC (J2000) = $19^{h}13^m 03^{s}.85$, $+\ang{19;46;22.7}$ with an accuracy of \ang{;;3.5} (90$\%$ confidence level (CL)) \cite{Evans2009}. 
We obtained the XRT lightcurve from the \textit{Swift}-XRT GRB Lightcurve Repository\footnote{\url{https://www.swift.ac.uk/xrt_curves/}}. The lightcurve has been shifted in time by 3198 s to apply the \textit{Fermi}/GBM trigger as $T_0$. 
We further used the XRT Repository tools to create time-sliced spectra, in both windowed timing (WT) and photon counting (PC) modes, at multiple epochs for use in modeling the broadband spectral energy distribution (SED) of the GRB afterglow. 



\subsection{\textit{XMM-Newton}}
\label{sec: XMM}


%https://xmmweb.esac.esa.int/cgi-bin/xmmobs/public/obs_view.tcl?search_instrument=0&action=Get+Selection&search_obs_id=0913991901


We observed GRB 221009A using \textit{XMM-Newton} on November 10, 2022 through Directory's Discretionary Time (PI: Troja), corresponding to 32.72 d after the GRB trigger. The observations were performed in full frame mode using the thin filter, and lasted for 100 ks with a mid-time of 32.72 d. The data were reduced and analyzed using tasks with the Science Analysis System (\texttt{SAS v18.0.0}) software. We used a circular region of $60\arcsec$ to extract source photons. The background photons were taken from a nearby source-free circular region of $60\arcsec$.  We grouped the spectrum to a minimum of 1 count per bin and obtained the response matrix and ancillary response files using the \texttt{rmfgen} and \texttt{arfgen} tasks. 


\subsection{\textit{NuSTAR}}
\label{sec: nustar}


\textit{NuSTAR} observed GRB 221009A on five epochs at mid-times of 1.82, 5.92, 10.72, 23.93, and 31.95 d after the \textit{Fermi} trigger (see Table \ref{tab:Xobservations}). These data were obtained under two DDT programs (co-PIs: Margutti and Racusin; PI: Troja). The initial observations were first reported by \cite{GCN32695,GCN32788}. \textit{NuSTAR} is comprised of two identical focal plane modules, FPMA and FPMB, covering the $3-79$ keV energy range. The GRB afterglow is detected in each epoch. We reduced the data using the \textit{NuSTAR} Data Analysis Software pipeline (\texttt{NuSTARDAS}) within \texttt{HEASoft v6.29c}. The data were processed using \texttt{nupipeline}, and then lightcurves and spectra were extracted using \texttt{nuproducts}. In the initial observation at 1.8 d, source spectra were extracted from a 100\arcsec{} radius region centered on the transient. The background was similarly extracted from a 100\arcsec{} radius source-free region. For each of the latter observations, we used a 60\arcsec{} radius for both source and background regions. 


\subsection{Gemini}
\label{sec: gemini}

Target of Opportunity (ToO) observations of GRB 221009A were performed with the 8.1-m Gemini South Telescope in Cerro Pachon, Chile using GMOS-S and Flamingos-2 (hereafter F2) under two Director's Discretionary Time Programs (GS-2022B-DD-104, PI: O'Connor; GS-2022B-DD-103, PI: Rastinejad). The observations were first reported by \cite{GCN32749,GCN32750,GCN32860}.
Data were obtained at 4.4, 17.4, 25.4, and 26.4 d. The observations were carried out in the $i$ filter with GMOS-S, and $J$, $H$ $K_s$ filters with F2 (see Table \ref{tab:Optobservations}). We reduced and analyzed these data using the \texttt{DRAGONS}\footnote{\url{https://dragons.readthedocs.io/}} software \cite{Labrie2019}. The afterglow is clearly detected in each observation. 
%\textcolor{purple}{Using the initial images, we localize the GRB to RA, DEC (J2000) = $19^{h}13^m 03^{s}.85$, $+\ang{19;46;22.7}$ with an accuracy of $XXX\arcsec$.} 
We performed PSF photometry using \texttt{SExtractor} \cite{Bertin1996} and \texttt{PSFEx} \cite{Bertin2013}. The photometry was calibrated using nearby point-sources in the Two Micron All Sky Survey (2MASS;) \cite{Skrutskie2006} catalog. We then applied a standard conversion between the Vega and AB magnitude systems.

%First, we ran \texttt{SExtractor} to identify bright, unsaturated and isolated point-like objects.  We selected them based on their SNR, FWHM, \texttt{CLASS\_STAR} parameter ($>$\,$0.8$), and ellipticity ($<$\,$0.2$). We further imposed  \texttt{FLAGS}\,$<$\,$1$, which excludes sources that are saturated, blended, or too close to the image boundary. These point-like sources were then passed to \texttt{PSFEx} \cite{Bertin2011,Bertin2013} to estimate the image PSF. This was then fed to \texttt{SExtractor}


\subsection{Lowell Discovery Telescope}
\label{sec: LDT}

We obtained ToO observations with the Large Monolithic Imager (LMI) mounted on the 4.3-meter LDT at the Lowell Observatory in Happy Jack, AZ starting at 3.6 d after the GRB (PI: Cenko) and continuing observations for 8 weeks (see Table \ref{tab:Optobservations}). We first reported the initial observations in \cite{GCN32739,GCN32799}. The data were reduced with a custom pipeline \cite{Toy2016} that makes use of standard CCD reduction techniques in the IRAF\footnote{IRAF is distributed by the National Optical Astronomy Observatory, which is operated by the Association of Universities for Research in Astronomy (AURA) under cooperative agreement with the National Science Foundation (NSF).} package including bias subtraction, flat-fielding, and cosmic ray rejection \cite{vanDokkum2001}. Photometry was performed in the same manner as for Gemini, and calibrated against stars in the catalog (Pan-STARRS1, hereafter PS1) \cite{Chambers2016}. 

\subsection{MASTER}
\label{sec: master}

MASTER is a system of wide-field fully robotic 40-cm telescopes with identical scientific equipment and real-time auto-detection at every observatory \cite{Lipunov2004,Lipunov2010,Kornilov2012}. The MASTER telescopes are MASTER-Amur, -Tunka, -Ural, -Kislovodsk, -Tavrida (Russia), -SAAO (South Africa), -IAC (Spain), -OAFA (Argentina). The MASTER Global Robotic Net \cite{Lipunov2010} began observing GRB 221009A using MASTER-SAAO on 2022-10-09 at 17:33:54 UT, corresponding to 0.18 d after the \textit{Fermi} trigger. The MASTER auto-detection system discovered the optical counterpart, MASTER OT J191303.43+194623.1 \cite{GCN32634}, as a transient in the initial image. The observations were obtained in the \textit{clear} ($C$) filter. Further observations were obtained with MASTER-OAF starting on 2022-10-09 at 23:56:38 UT, corresponding to 0.46 d after the trigger (see Table \ref{tab:MASTERobservations}). Aperture photometry was calibrated using 20 reference stars, and we applied a further correction to convert to the AB magnitude system. We note that earlier observations by MASTER-Tunka and MASTER-Amur, beginning at 93 s after the \textit{Fermi} trigger (2022-10-09 14:11:50 UT), were severely impacted by clouds and were unable to detect the source. 



%MASTER network usually works in the Johnson-Cousins UBVRI photometric system. Thus, we use a conversion coefficient to work in AB system: $m_{AB} = m_{C}+k_{AB}$ where $k_{AB} = -2.5\log_{10}(\frac{F_{Vega}}{3631 Jy\cdot \Delta \nu })\approx -0.09$. $F_{Vega} = 1.6\cdot 10^{18}$ is zero point of MASTER clear band in UBVRI photometric system. MASTER work only in visible range, thus $ \Delta \nu = (7.89-3.84)\cdot 10^{14}=4.05\cdot 10^{14}$ marks constraints of this range. The \textit{clear} filter is similar to the \textit{GAIA} $G$-band.

%Best fit temporal slope for MASTER is $-0.84 \pm 0.16$ which agrees with that derived from the other bands (approx 0.9).

\subsection{Hubble Space Telescope}
\label{sec: HST}

%\begin{figure} 
%\centering
%\includegraphics[width=\columnwidth]{figs/GRB221009A_FC_HST_RGB.pdf}
%\caption{RGB image of the field of GRB 221009A: red is $\textit{HST}/F160W$, green is $\textit{HST}/F098M$, blue is $\textit{HST}/F606W$. The position of the GRB is marked by the white circle. An extension of the source to the North-East is due to the underlying host galaxy at $z=0.1505$. 
%}
%\label{fig: FC}
%\end{figure}

\textit{HST} observations were carried out at 29.7, 40.6, and 55.7 d after the GRB trigger (see Table \ref{tab:Optobservations}). Data were acquired in the WFC3/UVIS $F625W$ and $F775W$ filters and WFC3/IR $F098M$, $F125W$, and $F160W$ filters through a DDT request (PI: Levan). The initial observation was first reported by \cite{GCN32921}. 
We reduced the data using standard procedures within the \texttt{DrizzlePac} package \cite{Gonzaga2012}. The source is clearly detected in all filters with a marginal extension of the source to the NE in the infrared filters (see Figure \ref{fig: FC}), likely due to the underlying host galaxy at $z=0.1505$. %The galaxy is not identified in the initial WFC3/UVIS images, likely due to extinction from the Milky Way, but is found in the deep $F625W$ images from 2022 December 4. %\textcolor{purple}{Based on these \textit{HST} images we derive a more precise localization of the GRB to RA, DEC = XXX....}. 
We performed photometry of the source complex using a circular region of radius $0.3\arcsec$ centered on the transient. The zeropoints were taken from the photometry keywords in the image headers. %These measurements include the unknown host contribution. 



%\textcolor{purple}{In order to estimate the host contribution we also performed aperture photometry in a $1\arcsec$ aperture (DOES THIS MESS WITH STAR SPIKE?? USE DECEMBER 4 EPOCH TO AVOID THAT) and find a difference of XX mag, leading to an inferred host galaxy contribution of XX (can also do in December 4 F625W epoch)}


\subsection{\textit{ATCA}}
\label{sec: ATCA}

The Australia Telescope Compact Array (ATCA) observed GRB 221009A as part of the DDT project CX515 on 2022-10-15, 2022-10-24, 2022-11-04, 2022-11-19 and 2022-12-28 (Table \ref{tab:Radioobservations}). The initial observation at 5.8 d after the GRB was first reported by \cite{GCN32763,GCN32766}. In the initial two epochs, the three pairs of Intermediate Frequencies (IFs) were used 16.7/21.2 GHz, 33/35 GHz, 45/47 GHz and in the next two only 16.7/21.2 GHz and 33/35 GHz were used. In the last epoch, corresponding to 80 d after the GRB, observations were obtained at 5.5 and 9 GHz. In all observing runs the array operated in continuum mode with the Compact Array Broadband Backend using 2048 channels over 2-GHz bandwidth per IF. The radio sources used as bandpass, primary and phase calibrator were 1921-293, 1934-638 and 1923+210, respectively. The phase calibrator was also used for reference pointing checks every hour. Standard procedures in the data reduction software package \texttt{MIRIAD}
% (\textcolor{red}{CITE})
\cite{Sault1995_MIRIAD}
were used to flag, calibrate the complex gains and image the phase calibrator and target. A robustness parameter value of two and 6-km baseline antenna was deselected during imaging. The resulting flux densities and 3$\sigma$ upper limits are presented in Table \ref{tab:Radioobservations}. The errors are derived from summing in quadrature the statistical and systematic uncertainty (map rms and 5\% of the total flux as residual of gain calibration, respectively).


\section{Data Analysis}
\label{sec: analysis}


\subsection{Multi-wavelength Lightcurve}
\label{sec: lightcurve}

The afterglow of GRB 221009A displays a single break in the temporal decay of both the X-ray and optical/infrared (OIR) lightcurves (Figure \ref{fig: lightcurve}). By modeling the X-ray lightcurve with a broken power-law, we determine an initial decay index $\alpha_{\textrm{X},1}=-1.52\pm0.01$ steepening to $\alpha_{\textrm{X},2}=-1.66\pm0.01$ after $t_{\textrm{break},X}=0.82\pm0.07$ d. 

On the other hand, the OIR lightcurves, spanning $grizJHK$ and the MASTER \textit{C} filter, display a shallower decay and a more significant temporal break. We find an initial power-law decay of $\alpha_{\textrm{OIR},1}=-0.88\pm0.05$, which steepens to $\alpha_{\textrm{OIR},2}=-1.42\pm0.11$ at around $t_{\textrm{break,OIR}}=0.63\pm0.13$ d. In this analysis we have supplemented our dataset with observations reported in GCN Circulars
% (\textcolor{red}{CITE ALL THE GCNs}).
% \jg{these are the refs for all GCNs included in the email I received... 
% 32662, 32646, 32652, 32755, 32795, 32743, 32670, 32684, 32709, 32678, 32753, 32752, 32765, 32758, 32771, 32769, 32811, 32804, 32809, 32803, 32818, 32852}
\cite{
GCN.32769, GCN.32818, GCN.32684, GCN.32743, GCN.32752,
GCN.32652, GCN.32755, GCN.32646, GCN.32804, GCN.32678,
GCN.32811, GCN.32758, GCN.32803, GCN32765hostz, GCN.32670,
GCN.32662, GCN.32852, GCN.32795, GCN.32809, GCN.32753,
GCN.32771, GCN.32709}.

%We note that while the initial GCN data provides a sparse view of the early optical evolution, the data obtained by MASTER over this period is significantly more well-sampled. It is important to note that the observed decay based on GCN data alone is slightly shallower than the inferences from MASTER alone which yields an initial decay of $\alpha_{\textrm{MASTER},1}=-0.66\pm0.10$ with a break at around $0.6$ d.

The OIR and X-ray break times are separated by $0.19\pm0.15$ d. This may suggest that while the break could be achromatic, it is not immediately favored by the best-fit models. %This may be an artifact of the transition between WT mode and PC mode data obtained by \textit{Swift} XRT, as when masking\footnote{\url{https://www.swift.ac.uk/xrt_live_cat/01126853/}} the data obtained between 0.64 and 1.03 d, the best-fit break time is $\sim$\,$0.57$ d.  

Using the multi-epoch ATCA observations at 16.7 and 21.2 GHz we find that the temporal decline is well-described by a $t^{-1.0\pm0.2}$ evolution. Moreover, we observe a very steep decay of at least $t^{-2.4}$ at 45 GHz and 47 GHz between 5.78 and 14.72 d, hinting that the radio emission may be dominated by a separate component than the X-ray and OIR. 


\begin{figure} 
\centering
%\includegraphics[width=\columnwidth]{figs/GRB221009A_lc.pdf}
\includegraphics[width=\columnwidth]{figs/GRB221009A_lc_wRadio.pdf}
\caption{Multi-wavelength lightcurve of GRB 221009A. The OIR data is not corrected for Galactic extinction $A_V=4.09$ mag. The XRT and \textit{XMM-Newton} represent the X-ray flux density at 1 keV, whereas the flux density from \textit{NuSTAR} observations is obtained at 5 keV. OIR data represented as empty squares were compiled from GCN circulars.
}
\label{fig: lightcurve}
\end{figure}




\subsection{X-ray Spectroscopy}

%\textcolor{red}{Need to mention the harder initial WT mode spectrum... very important to the discussion and significance of spectral evolution while also showing independent of this initial spectrum the NuSTAR data shows an evolution, as observed for GRB 130427A (Kouveliotou et al. 2013).}

We began by analyzing the \textit{Swift}/XRT data ($0.3-10$ keV) obtained in Photon Counting (PC) mode between $10^5$ and $10^6$ s after the BAT trigger with a total exposure of 52.6 ks. We modeled the spectra using \texttt{XSPEC v12.12.0} \cite{Arnaud1996}. We applied the ISM abundance table from \cite{Wilms2000} and the photoelectric absorption cross-sections from \cite{Verner1996}. The best fit model parameters were determined by minimizing the Cash statistic \cite{Cash1979}. We applied the model \texttt{tbabs$*$ztbabs$*$pow} with fixed redshift $z=0.1505$ \cite{GCN32648xshooterz,GCN32686GTCz,GCN32765hostz}. The Galactic hydrogen column density was frozen to $N_H=5.36\times10^{21}$ cm$^{-2}$ \cite{Willingale2013}. The best fit parameters in this time range are $N_{H,z}=(1.3\pm0.1)\times 10^{22}$ cm$^{-2}$ and photon index $\Gamma=-1.73\pm0.05$. 

As a comparison, we analyzed the initial WT mode spectra obtained by XRT starting at $\sim$\,1 hr after the \textit{Fermi} trigger. This initial spectra displays a harder photon index of $\Gamma=-1.65\pm0.02$, hinting at spectral evolution in the X-rays from early times.

To further explore the X-ray spectral evolution, we turned to the \textit{NuSTAR} data ($3-79$ keV). We fit the FPMA and FPMB spectra simultaneously, allowing for the normalization of FMPB to vary. The normalization of FPMA was fixed to unity. The FPMB normalization varied by $\lesssim5\%$ compared to unity, likely due to a rip in the multi-layer insulation of FPMB \cite{Madsen+2020}. We applied the model \texttt{con$*$tbabs$*$ztbabs$*$pow} with $N_H$ and $N_{H,z}$ fixed to the values identified from our fit to the XRT data. The unabsorbed flux was derived using the \texttt{cflux} command. The data obtained at 23.93 and 31.95 d were fit between the 3-50 keV energy range, as this was where we found that the background began to dominate. The results of the \textit{NuSTAR} analysis are displayed in Table \ref{tab: nustar}. We observe a softening of the photon index between $-1.81\pm0.1$ at 1.82 d and $-2.1\pm0.17$ at 31.95 d. The latter value is consistent with the initial photon index, $\Gamma=-2.08\pm0.03$,  determined by \textit{Swift} BAT \cite{Krimm2022}.

We additionally analyzed the \textit{XMM-Newton} data obtained at 32.72 d by performing a joint fit with the \textit{NuSTAR} data obtained in a similar period, allowing for a normalization factor between the two spectra. We derive $N_{H,z}=(1.4\pm0.2)\times 10^{22}$ cm$^{-2}$ and photon index $\Gamma=-1.97\pm0.09$. 

A joint fit including X-ray data obtained at $<1$ d with XRT in WT mode (0.05, 0.25 and 0.44 d), XRT and \textit{NuSTAR} data at 1.8, 5.9, 10.72, and 23.93, and \textit{XMM-Newton} and \textit{NuSTAR} at $\sim$ 32 d yields a value of $N_{H,z}=(1.31\pm0.02)\times 10^{22}$ cm$^{-2}$, which is consistent with our estimates based on individual spectra. The photon index and normalization were allowed to vary between epochs. If we exclude the data obtained during the first orbit (0.05 d) and link the photon index as well, we derive $N_{H,z}=(1.29\pm0.02)\times 10^{22}$ cm$^{-2}$ and $\Gamma=-1.85\pm0.01$. Thus, $\Gamma=-1.85$ is the mean photon index obtained between 0.25 and 32 d. 



\begin{table}
    \centering
    \caption{Results of our \textit{NuSTAR} spectral analysis.  \textcolor{red}{[[[It is crucial to have a similar table for Swift/XRT as well as the optical/NIR spectral slope for different times (despite the "systematic" uncertainty due to extinction, the time dependence has important relevant information)]]]}
    }
    \label{tab: nustar}
    \begin{tabular}{lccc}
    \hline
    \hline
   \textbf{Time} & \textbf{$\Gamma$} & \textbf{$F_X$ (3-79 keV)} \\
   \textbf{(d)} & --   & \textbf{(erg cm$^{-2}$ s$^{-1}$)} \\
    \hline
    \hline
     1.82   & $1.81\pm0.01$ &  $(3.21\pm0.03)\times 10^{-10}$\\ %Cstat = 110 for 1153 dof
     5.92   & $1.89\pm0.03$ &  $(4.65\pm0.11)\times 10^{-11}$  \\ %Cstat = 537 for 546 bins
     10.72  & $1.88\pm0.05$ &  $(1.53\pm0.08)\times 10^{-11}$ \\ %Cstat = 218 for 226 dof
     23.93  & $1.94\pm0.12$ &  $(3.4\pm0.4)\times 10^{-12}$ \\ %Fit between 0-30 keV
     31.95 & $2.10\pm0.17$  & $(1.8\pm0.3)\times 10^{-12}$ \\ %Fit between 0-20 keV / Cstat = 820 for 845 dof
     \hline
     \hline
    \end{tabular}
\end{table}


\begin{figure} 
\centering
\includegraphics[width=0.5\columnwidth]{figs/GRB221009A_SED_figure.pdf}
\includegraphics[width=0.5\columnwidth]{figs/GRB221009A_gamma_times.pdf}
\caption{Observed spectral energy distributions (SEDs) of GRB 221009A between 0.05 and 41 d. The solid line is the combination of a FS and RS, while the dotted line shows the RS contribution. The data have been corrected for extinction and absorption: $E(B-V)=1.3$ mag and $N_H=1.3\times10^{22}$ cm$^{-2}$. 
}
\label{fig: SEDs}
\end{figure}

\subsection{Spectral Energy Distributions}
\label{sec: SEDs}

Based on our analysis of the X-ray spectra, we observe an evolving photon index from harder to softer values.  Due to this, in what follows we model the broadband spectral energy distributions (SEDs) with a smoothly broken power-law to account for possible spectral evolution with time. Moreove, the distinct decay slopes between the OIR and X-ray bands may suggest that the X-ray and OIR data lie on separate power-law segments of the synchrotron spectrum \cite{Granot2002}.


We utilized \texttt{XSPEC} to model the SEDs using an absorbed smoothly-broken power-law model. We took into account both absorption and extinction in the Milky Way and the host galaxy using the commands \texttt{redden$*$zdust$*$tbabs$*$ztbabs}\footnote{The \texttt{XSPEC} command \texttt{redden} takes into account extinction within the Milky Way \cite{Cardelli1989}, whereas  \texttt{zdust} corrects for dust in the host galaxy \cite{Pei1992},  assuming $R_V=A_V/E(B-V)$=3.1 \cite{Rieke1985}.}. We fixed the redshift to $z=0.1505$ \cite{GCN32648xshooterz,GCN32686GTCz,GCN32765hostz} and froze the hydrogen column density to the best fit values from our X-ray spectral analysis of $N_H=5.36\times10^{21}$ cm$^{-2}$ \cite{Willingale2013} and $N_{H,z}=1.3\times10^{22}$ cm$^{-2}$. The MW, $E(B-V)$, and host, $E(B-V)_z$, extinction were free to vary.

We simultaneously modeled twelve (12) broadband SEDs between 0.05 and 32 d. The low- and high-energy spectral indices were tied between SEDs, but the break energy $E_c$ was free to vary. The smoothness parameter $s$ was likewise tied between SEDs, but free to vary. The best fit smoothly broken powerlaw has $s\approx1$, $\beta_{\textrm{XOIR},1}=-0.63\pm0.05$, $\beta_{\textrm{XOIR},2}=-0.995\pm0.05$ with a reduced $\chi^2=1.2$ (see Figure \ref{fig: SEDs}). The break energy $E_c$ decreases in time between $\approx$\,$10$ to $\approx$\,$0.3$ keV. We find a value of MW extinction to be $E(B-V)=1.32\pm0.01$ mag, corresponding to $A_V=4.09\pm0.03$ mag, and a negligible intrinsic extinction. We derive an upper limit to the intrinsic extinction of $E(B-V)_z<\textcolor{red}{XX}$ at the \textcolor{red}{90\%} confidence level (CL).


The results of this smoothly-broken power-law model are quite similar to the expectations for a standard synchrotron spectrum \cite{Granot2002}. In this model, the spectrum is governed by the evolution of three frequencies: the cooling frequency $\nu_c$, the peak frequency $\nu_m$, and the synchrotron self-absorption frequency $\nu_a$, in addition to the slope $p$ of the electron power-law energy distribution $N(\gamma)\propto\gamma^{-p}$. As the initial modeling is suggestive of a cooling break scenario to explain the X-ray temporal and spectral evolution, we consider a smoothly-broken power-law model where the smoothness if given by $s=1.15-0.06p$ \cite{Granot2002} and $\beta_{\textrm{XOIR},1}=\beta_{\textrm{XOIR},2}+0.5$. We derive a value of $p=2.17\pm0.03$, which yields similar spectral slopes before and after the break as derived from the initial XRT, $\beta_\textrm{WT}=(1-p)/2=-0.65\pm0.02$, and BAT data, $\beta_\textrm{BAT}=-p/2=-1.08\pm0.03$) \cite{Krimm2022}. This result is independent of including the BAT data. In this model, we fixed the cooling break $E_c$ to move in time as $t^{-0.5}$ to mimic the temporal evolution of the cooling frequency in an ISM environment \cite{Granot2002}, as opposed to leaving it completely free between epochs. The result is displayed in Figure \ref{fig: SEDs}. 



%We began by modeling the broadband (X-ray, optical, nIR) SED at multiple epochs (3.6, 4.4, 9.5, XX, XX d). We tested whether the OIR and X-ray data could lie on the same spectral segment by jointly modeling the data within \texttt{XSPEC} using an absorbed power-law model \texttt{redden$*$zdust$*$tbabs$*$ztbabs$*$powerlaw}\footnote{The command \texttt{redden} corrects for extinction within the Milky Way \cite{Cardelli1989}, whereas  \texttt{zdust} accounts for intrinsic dust extinction within the host galaxy \cite{Pei1992} assuming a Milky Way extinction curve assuming $R_V=A_V/E(B-V)$=3.1 \cite{Rieke1985}.}. We fixed the redshift to $z=0.1505$ \cite{GCN32648xshooterz,GCN32686GTCz,GCN32765hostz} and froze the hydrogen column density to the best fit values from our X-ray spectral analysis of $N_H=5.36\times10^{21}$ cm$^{-2}$ and $N_{H,z}=1.2\times10^{22}$ cm$^{-2}$.

%We initially allowed the Milky Way extinction, parameterized by $E(B-V)$, to vary. Using the optical (GMOS-S), infrared (F2), and X-ray (XRT) data at $4.4$ d, we derive $E(B-V)=1.32\pm0.03$ mag, yielding $A_V=4.09\pm0.09$ mag. We freeze this result in our following analysis. 
%\textcolor{red}{using Guver and Ozel - NHz =1.2e22 $\rightarrow$ Av=5.4+/-0.5 mag...}

%In our SED analysis we observe a softening of the spectrum from $\Gamma=1.71\pm0.01$ at 3.6 d and $\Gamma=1.79\pm0.02$ at 24 d. \textcolor{red}{Plot of Photon Index vs time?}




%\begin{table*}
%    \centering
%    \caption{Results of our broadband SED analysis. \textcolor{red}{nH, nHz, E(B-V), E(B-V)z}
 %   }
 %   \label{tab: sed}
 %   \begin{tabular}{lccccccc}
 %   \hline
 %   \hline
 %  \textbf{Time} & $E(B-V)$ & $E(B-V)_z$ &  \textbf{$\Gamma$}  & \textbf{Normalization} & \textbf{$\Gamma_1$} & \textbf{$\Gamma_2$} & \textbf{Normalization} \\
%   \textbf{(d)} & (\textbf{mag}) &  (\textbf{mag})& -- & \textbf{(XXX)} & -- & -- & \textbf{(XXX)} \\
%    \hline
%    \hline
%     & & & & & & & \\
%     \hline
%     \hline
%    \end{tabular}
%\end{table*}





\section{Results} 
\label{sec: results}

\subsection{Standard Forward Shock}



Motivated by our SED modeling, we began by exploring the simple scenario of a relativistic fireball \cite{Meszaros1997,Sari1998,Wijers1999,Granot2002} propagating into an ambient medium with density of the form $\rho_{\textrm{ext}}(r)=A\, r^{-k}$, where $k=0$ represents an interstellar medium (ISM) environment and $k=2$ a stellar wind environment. The shock-accelerated electrons cool via synchrotron radiation with a characteristic spectrum dominated by the three break frequencies: $\nu_c$, $\nu_m$, and $\nu_a$. In the following we separately consider the lightcurve evolution in the X-rays, OIR, and radio.

\subsubsection{X-ray Lightcurve}

The X-ray lightcurve displays a break at around $\sim$\,1 d with a change in slope of $\Delta\alpha_X=0.14\pm0.02$. This can be explained by the passage of $\nu_c$ through the X-ray band. 

As we observe a steepening of the X-ray spectral index in time, this is consistent with the transition from  $\nu_m<\nu<\nu_c$ to $\nu_m<\nu_c<\nu$ where the spectral index steepens from $\nu^{(1-p)/2}$ to $\nu^{-p/2}$. The change in X-ray spectral index of $\Delta\beta_X=0.46\pm0.07$ is consistent with this scenario where $\Delta\beta=0.5$. This implies that the cooling frequency $\nu_c\propto t^\frac{3k-4}{2k-8}$ must decrease in time such that $k<4/3$.


In this case\footnote{Here, G and H refer to the power-law segments defined by \cite{Granot2002}, where G corresponds to $\nu_m<\nu<\nu_c$ and H to $\nu_m<\nu_c<\nu$.}, the initial temporal decay is provided by $\alpha_G=\frac{k(3p-5)-12(p-1)}{4(4-k)}$ \cite{BGG2020}, whereas after the passage of $\nu_c$ (i.e., $\nu_m<\nu_c<\nu$) the decay is  $\alpha_H=\frac{(2-3p)}{4}$, which is independent of $k$.  %These considerations thus far ignore Inverse Compton (IC) corrections \cite{Sari2001,Zou2009,Beniamini2015,Jacovich2021}. 

The post-break slope  $\alpha_H=-1.66=(2-3p)/4$ requires a steep $p\approx2.88$. Furthermore, the change in temporal slope due to the crossing of $\nu_c$ is  $\Delta\alpha_{GH}=\alpha_G-\alpha_H=\frac{3}{4}+\frac{2}{k-4}$, which is independent of $p$. We find the requirement $\Delta\alpha\sim0.14\pm0.02$ to be satisfied by $k\approx 0.72$. 

%In addition, while these considerations easily explain the X-ray temporal and spectral evolution, they do not explain the evolution of the OIR lightcurve, or the shallower post-break OIR slope.  Thus, we exclude this simple FS scenario to explain GRB 221009A's afterglow lightcurve.

\subsubsection{Optical and Infrared Lightcurve}

The OIR lightcurve displays a shallow initial slope of $\alpha_\textrm{OIR,1}\approx-0.9$ followed by a steeper decay of $\alpha_\textrm{OIR,2}\approx-1.45$ after $\sim$\,1 d. The initial slope can be explained by optically thin synchrotron radiation in an ISM environment ($k=0$) as $\alpha=3(1-p)/4=-0.9$ for $p=2.2$. A stellar wind environment leads to significantly steeper slopes. However, utilizing the steep $p=2.88$ inferred from the X-rays is inconsistent with the initial shallow OIR slope and fails to explain the break in the OIR lightcurve. 

One alternative possibility, is that the initial OIR data at $<$\,1 d is below $\nu_m$, such that the transition from $\nu_\textrm{OIR}<\nu_m$ to $\nu_m<\nu_\textrm{OIR}$ can explain the lightcurve break. In this case, the post-break slope would be provided by $\alpha_G=-1.52$ as for the X-rays, assuming $p=2.88$ and $k=0.72$. The excess flux from the underlying supernova \cite{GCN32800,GCN32850} can then explain the observed OIR slope of $\alpha_\textrm{OIR,2}=-1.45$. 

While this scenario appears to resolve the lightcurve slopes, a major issue with these closure relations is that the inferred value of $p=2.88$ is significantly steeper than determined by our SED modeling (\S \ref{sec: SEDs}). In fact, modeling the SEDs with $p=2.88$ fails to produce a satisfactory fit the data. We further discuss these inconsistencies and possible resolutions (e.g., a jet-break) \cite{Rhoads 1999,Sari 1999} below in \S \ref{sec: scenario1} and \S \ref{sec: scenario2}. 

\subsubsection{Radio Lightcurve}

The high-frequency radio data (Table \ref{tab:Radioobservations}) obtained between 5.8 and 40.7 d display a significantly different evolution than the X-ray and OIR data (Figure \ref{fig: lightcurve}). This is not unexpected given the data could lie in separate regimes of the FS or be significantly affected by a bright RS, as found for other energetic GRBs displaying GeV emission
% (\textcolor{red}{CITE: van der Horst 2013 on 130427A, Dichiara et al. on 190829, and Rhodes et al. on 190829A}).
\cite{Stanek2003,van_der_Horst2014, Rhodes2020, Dichiara2022}.
%In our analysis we include radio data presented in GCN circulars (\textcolor{red}{CITE ALL}).
Given that the ATCA data (Figure \ref{fig: lightcurve}) is decreasing with time, we infer that it is dominated by a bright RS component, as the expected FS evolution for $\nu<\nu_m$ is $t^{(2-k)/(4-k)}$ which is rising for reasonable values of $k$, e.g., $k=0$ leads to $t^{1/2}$.






%\textcolor{purple}{These considerations thus far ignore Inverse Compton (IC) corrections \cite{Sari2001,Zou2009,Beniamini2015,Jacovich2021}, which are ubiquitous when discussing synchroton radiation and should be included when the Compton parameter $Y>1$.} 


%\textbf{\textcolor{purple}{Do we note that the GeV data may imply $Y\approx1$ at $10^5$ s, and decreasing from there???... But this is likely a lower-limit on the Y parameter as the IC peak is likely in the TeV range...}}

\subsection{Reverse shock}


The high-frequency radio data (Table \ref{tab:Radioobservations}) is likely dominated by a bright RS. In Figure \ref{fig: ATCA_SEDs} we display the multi-epoch SEDs obtained by ATCA. We observe a shallow spectral slope of $\nu^{-0.5}$ steepening to $\sim$\,$\nu^{-3}$ (Figure \ref{fig: ATCA_SEDs}). The shallow pre-break slope could indicate that the radio data is either \textit{i}) fast cooling such that $\nu_c<\nu_a<\nu<\nu_m$ or \textit{ii}) slow cooling  ($\nu_m<\nu<\nu_c$) where  $\nu^{-0.5}=\nu^{(1-p)/2}$ for $p\approx2$. The steep cut-off decreases in time, and explains the steep evolution of the high frequency radio data.

We observe that this cut-off frequency, hereafter $\nu_\textrm{cut}$, decreases in time from $\sim45-50$ GHz at 5.8 d to $\lesssim16$ GHz at 40.7 d. We attribute this to a post-shock crossing residual population of cooling electrons \cite{Kobayashi2000} \textcolor{purple}{(Any other references on this?)}, above which the flux decays exponentially. The evolution of this frequency in time is observed to be non-standard as between 5.8 and 40.7 d we require an evolution of at least $t^{-0.5}$. An evolution much steeper than this fails to explain the SEDs at 14.7 and 25.7 d. However, even assuming an evolution of $t^{-1.5}$ \cite{Kobayashi2000}, if we trace this frequency back in time we find that $\nu_\textrm{cut}<\nu_\textrm{OIR}$ at $\lesssim 1$ d. This implies that the RS is unlikely to dominate the early OIR emission. 

\textcolor{purple}{What should we say regarding the shallow radio slope of $t^{-1}$ at 16 and 21 GHz.. discussion points: 1) not typical RS, too shallow 2) RS+FS could shallow it out but then the FS needs to be dominating at late times, which we do not observe and \textbf{3) could the shallow jet structure be flattening out the RS emission...}} What is the shallowest slope we can get for a RS (thin/thick shell)? \textbf{-1.5 for PLS G in the the thin-shell case.. but -1.5 + FS could = -1...} Good to state in text and compare.

%\textcolor{purple}{add discussion of observational constraints on cutoff frequency $\nu_\textrm{cut}$ (post shock-crossing residual population of cooling electrons) and fit with $(t-to)^a$; reference https://iopscience.iop.org/article/10.1086/317869/pdf and https://iopscience.iop.org/article/10.3847/1538-4357/ab40ce} ... cutoff frequency does not explain data well because on-constant decay is observed...

\vspace{10mm}


Radio data can be affected by interstellar scintillation (ISS)
\cite{Rickett1990, Goodman1997} due to fluctuations in the density of free electrons. Following \cite{Hancock2019}, we derive a scatting measure of  SM$=4.3\times 10^{-4}$ kpc $m^{-20/3}$, a transition frequency of $\nu_0=9$ GHz between strong and weak scattering, and the angular size of the first Fresnel zone $\theta_{F0}=2.1\times10^{4}\, \textrm{SM}^{0.6}\nu_0^{-2.2}=1.6\,\mu$as  \cite{Walker1998}. At the putative redshift $z=0.1505$, an angular size of $1\,\mu$as corresponds to a physical size of $8.2\times10^{15}$ cm, such that $\theta_{F0}$ corresponds to a source size of $1.3\times 10^{16}$ cm. As the ATCA frequencies are in the weak scintillation regime $\nu_o<\nu$, we likewise compute $\theta_w=\theta_{F0}\big(\frac{\nu}{\nu_0}\big)^{-1/2}$ which yields $\theta_w=1.1\,\mu$as for $\nu=16.7$ GHz. For source sizes $\theta_s$ larger than $\theta_w$, the modulation index decreases as $\big(\frac{\theta_s}{\theta_w}\big)^{-7/6}$. This implies that the ATCA observations are unlikely to be affected by flux modulations due to scintillation. \textcolor{red}{But at the same time, it appears ISS could be at play between 15 and 27 d... Figure \ref{fig: ATCA_SEDs}.}



\begin{figure} 
\centering
\includegraphics[width=\columnwidth]{figs/GRB221009A_ATCA_SEDs_2.pdf}
\caption{Spectral energy distributions of the radio data from ATCA between $16.7-47$ GHz. We observe a steep decay of the radio data, indicative of emission from a reverse shock. 
}
\label{fig: ATCA_SEDs}
\end{figure}


\subsection{A forward-shock plus a reverse-shock}
\label{sec: scenario1}

\textcolor{purple}{Re-write this to tell a more simple and clear story and show more clearly why 'vanilla' case and RS case do not work well. Focus on the observations not the theory!}

{\bf PB: What is missing from this section is a clear description of which frequencies are dominated by FS and RS and at what times.}
As previously noted, there are two major limitations with the FS model to describe the observed afterglow behavior: \textit{i}) The post-break slope of the X-rays requires a steeper value of $p$ than implied by the broadband SEDs and \textit{ii}) the standard FS model fails to describe the early OIR slope. 

As discussed in the previous section, GRB 221009A displays a bright RS component, which likely contributes to the early OIR emission. Therefore, a significant contribution of the RS to the early ($<0.6$ d) OIR emission and a rising FS component could explain the shallow decay of the OIR at $<0.6$ d. In this scenario, OIR wavelengths would initially lie below the peak frequency such that $\nu_\textrm{OIR}<\nu_m$ with $\nu_m$ beginning to cross the OIR at around $0.5$ d {\bf PB: Throughout this section, perhaps use a different notation for frequencies corresponding to RS and FS}. The evolution of $\nu_m\propto t^{-1.5}$ is independent of both $p$ and $k$. Assuming that $\nu_m=(6-8)\times 10^{14}$ Hz at 0.5 d, by $\sim$1 d $\nu_m$ would pass through the near-infrared. 

At a similar time, $\nu_c$ would pass down through the X-rays in order to describe the evolution of the X-ray spectral index and the broadband SED modeling. Despite this, we are still left to explain the discrepancy between the steep X-ray slope above $\nu_c$ and the value of $p$ inferred by our SED modeling, which would imply $t^{(2-3p)/4}=t^{-1.15}$ for $p=2.2$. This is significantly shallower than the observed post-break decline of $t^{-1.66}$.

{\bf PB: I would leave the changing of microphysical params. to the end of the section. Only after you describe that the vanilla version doesn't work, you may want to briefly address whether adding a dependence of microphysical params with time changes this (in any case, this will not solve the fine tuning involved with different characteristic frequencies crossing through observed bands at the same time).}
In order to mitigate this, we consider breaking standard assumptions as to the evolution of the afterglow model. We consider a possible time-dependent evolution of the microphysical parameters, as applied to describe other well-sampled GRB lightcurves
(e.g., \cite{Racusin2009,Filgas2011, van_der_Horst2014}). 
Following \cite{GranotSari2022}, the flux and frequency evolution 
%in the globally slow cooling regime 
is given by:
\begin{align}
\label{eqn1}
    &F_{\nu,\textrm{G}}\propto \varepsilon_e^{p-1} \varepsilon_B^{(1+p)/4}  t^\frac{k(3p-5)-12(p-1)}{4(4-k)} \:\textrm{for}\:\nu_m<\nu<\nu_c \\
    &F_{\nu,\textrm{H}}\propto \varepsilon_e^{p-1} \varepsilon_B^{(p-2)/4} t^{(2-3p)/4} (1+Y)^{-1} \:\textrm{for}\:\nu_c<\nu \\
    &\nu_c\propto\varepsilon_B^{-3/2}t^{(3k-4)/(8-2k)} (1+Y)^{-2} \\
    &\nu_m\propto \varepsilon_e^{2} \varepsilon_B^{1/2} t^{-3/2} 
\end{align}
where $\varepsilon_e$ is the fraction of the burst kinetic energy $E_k$ in electrons, $\varepsilon_B$ is the fraction in magnetic fields, and $Y$ is the Compton parameter. We begin by considering a scenario where $Y\ll1$ by $\sim$\,$1$ d, such that the inclusion of SSC corrections can be ignored. This requirement may be difficult to reconcile with the long-lasting GeV emission (\textcolor{red}{CITE}). In fact, while the ratio of the X-ray to GeV emission at $\sim$\,$10^5$ s implies $Y\approx1$ \cite{Piran2009,Beniamini2011} this provides a lower-limit as the SSC emission peak is likely at TeV energies \cite{GCN32677}. 

Assuming that $p=2.2$, we require that the time-dependence of the microphysical parameters adds an additional $t^{-0.51\pm0.01}$ to the temporal decay above $\nu_c$. As the flux above $\nu_c$ has a very shallow dependence on $\varepsilon_B$, such that $F_{\nu,\textrm{H}}\propto \varepsilon_B^{1/20}$ for $p=2.2$, it is more practical to consider a time-evolution of $\varepsilon_e$. Furthermore, as $\nu_c$ is independent of $\varepsilon_e$ for $Y\ll1$, the requirement that the cooling frequency decreases with time is more easily satisfied. Thus, we find $\varepsilon_e\propto t^{-0.425}$ satisfies both our requirements. Given that the $\varepsilon_e$ dependence of $F_{\nu,\textrm{H}}$ and $F_{\nu,\textrm{G}}$ is the same, we can determine the value of $k$ by again using  $\Delta\alpha_{GH}=\frac{3}{4}+\frac{2}{k-4}=0.14\pm0.02$ which is satisfied by $k\approx 0.72$. In this case, $\nu_c\propto t^{-0.28}$. % and the flux below $\nu_m$ increases as $F_{\nu,\textrm{D}}=t^{(2-k)/(4-k)}=t^{0.39}$. 
Indeed the evolution of $\nu_m\propto t^{-2.35}$ is also increased, such that it can more quickly move through the OIR band. 

\textcolor{purple}{Still need to add something on actually why we disfavor this scenario due to fine-tuning and that the RS might actually not be able to contribute to OIR due to cutoff frequency... need to consider simplest way to introduce this without going into detail on the RS...}

\textcolor{purple}{Note that this case requires a lot of stuff happening at exactly the same time and is very fine-tuned so we favor the structured jet instead.}

In order for the fast $\nu_m$ evolution to be consistent with the upper limits from ATCA at 14.68 and 40.71 d, we require that the synchrotron self-absorption frequency $\nu_a$ is located above those frequencies such that $\nu_a\approx 50$ GHz at 40.71 d. As $\nu_a\propto \varepsilon_e^{-1}t^\frac{3k}{5(k-4)}=t^{-0.56}$ for the scenario described above, we would require $\nu_a\approx 400$ GHz at 1 d after the GRB.  \textcolor{red}{since we disfavor this model is it even worth noting this weird/impossible $\nu_a$ requirement ...}

\subsubsection{Constraints on the bulk Lorentz factor}

We can use the requirement that the jet must decelerate before $1$ hr (0.05 d) after the \textit{Fermi} trigger to constrain the initial bulk Lorentz factor $\Gamma_0$. 
The initial bulk Lorentz factor $\Gamma_0$ is obtained following \cite{SariPiran1999,Nappo2014}, where for a homogeneous environment \jg{What is the exact duration of the prompt GRB emission ($T_{50}$, $T_{90}$ etc.) and what constraints do we have on the afterglow onset time? This can constrain the thin vs. thick shell case for the deceleration of the GRB ejecta}\brendan{The GRB duration depends on the instrument observing it, but a typical value I think is $\sim600-700$ s. As for the afterglow onset, no afterglow follow-up happened until the Swift trigger almost an hour after the GRB because Fermi did not send a notice, so 1 hour is the best we can do.}
\begin{equation}
    \Gamma_0 > \Big[\frac{17}{64\pi}\frac{E_\textrm{kin,iso}}{c^5 n_0 m_p (\frac{t_p}{1+z})^3}\Big]^{1/8}. 
\end{equation}
Here, $c$ is the speed of light, $m_p$ is the mass of a proton, and $t_p$ is the upper limit on the peak time. Using a kinetic energy of $E_\textrm{kin,iso}\approx1\times10^{55}$ erg (and thus a gamma-ray efficiency of 15\%) \cite{Nava2014}, circumburst density $n_0=1$ cm$^{-3}$, and a peak time of $t_p<0.05$ d, we obtain $\Gamma_0>76$. This constraint is largely independent of our interpretation of the afterglow emission and relies on the early X-ray detection by \textit{Swift}/XRT. 


\subsubsection{Energetics}

In addition to being challenged to explain the observed spectral and temporal evolution, a standard jet scenario of the type addressed above, is challenged in terms of the required energetics to power the burst. The OIR and X-ray lightcurve evolve as $t^{-1.5}-t^{-1.66}$ up to at least 80 days after the trigger (at the time of writing). This is much shallower than the decay that would be expected after the jet break, $t_{\rm j}$, for a jet with a steep angular structure of the kinetic energy (typically, $t^{-p}$) \cite{Sari1999}. $t_{\rm j}$ represents the point in time at which $\Gamma$ has decelerated to $\theta_0^{-1}$ (where $\theta_0$ is the opening angle of the jet). Therefore, we can put an observational lower limit on $t_{\rm j}>t_{\rm j,l}=80$ d, which leads to a lower limit on the jet opening angle $\theta_0$. This in turn leads to a lower limit on the true (i.e. collimation-corrected) of the GRB, $E_{\rm t}\approx\frac{1}{2}\theta_0^2E_{\rm kin,iso}(\theta_{\rm obs})$, where we have assumed that the observer viewing angle relative to the jet axis is $\theta_{\rm obs}<\theta_0$. This is conservative as if this were not the case the lower limit on $E_{\rm t}$ would only increase. The limit to the energy is given by
\begin{equation}
    E_{\rm t}>E_{\rm kin,iso}(\theta_{\rm obs}) \frac{1}{2}t_{\rm j,l}^{\frac{3-k}{4-k}} \left(\frac{(3-k)E_{\rm kin,iso}(\theta_{\rm obs})}{4\pi A 2^{3-k} c^{5-k}}\right)^{\frac{1}{k-4}} 
\end{equation}
This limit generally decreases with $k$. Since $\nu_c$ is seen to decrease in time (see \S \ref{sec: SEDs}), we can in addition require that $k<4/3$. Therefore the most conservative estimate is given for $k=4/3$. Plugging either $k=0$ or $k=4/3$ we find
\begin{eqnarray}
    E_{\rm t}\!>\!\left\{ \begin{array}{ll}6\!\times \!10^{53}\mbox{ erg}\left(\frac{t_{\rm j,l}}{80\mbox{ d}}\right)^{3/4} (f(\eta_{\gamma})E_{\rm \gamma,iso,54.5})^{3/4}n_0^{1/4} & k=0 ,\\ \\
2.6\!\times \!10^{53}\mbox{ erg}\left(\frac{t_{\rm j,l}}{80\mbox{ d}}\right)^{5/8} (f(\eta_{\gamma})E_{\rm \gamma,iso,54.5})^{5/8}A_0^{3/8}  & k=\frac{4}{3}
\end{array} \right.
\end{eqnarray}
\textbf{\textcolor{purple}{where (please explain notations here, including $n_0,A_0$...)}} and $f(\eta_{\gamma})=3(1\!-\!\eta_{\gamma})/(17\eta_{\gamma})$ carries the dependence on the $\gamma-$ray efficiency and has been normalized such that it is unity for $\eta_{\gamma}=0.15$ as supported by observations of the brightest GRBs \cite{Beniamini2015}. 
\textcolor{red}{We should also put (for observers) what the constraint on $\theta_0$ is based on this - not as equation in text, but just one sentence should do...}

We see that the required (collimation-corrected) energy is extremely large and depends only weakly on the unknown external density. Such a huge energy is not readily explained by theoretical considerations. Furthermore, if this were to be the true energy of GRB 221009A, it would make it an extreme outlier to the GRB energy distribution. This possibility is therefore challenged even on statistical grounds only, assuming no priors on possible energy sources of GRBs.




%\textcolor{purple}{All of the above is assuming $Y<1$, such thatg SSC corrections can be ignored... }

%\textcolor{purple}{Need to solve for $\nu_m$, $\nu_c$, and $F_{\nu_m}$ self consistently to derive some constraints on the parameters... }

%\textcolor{purple}{Here also need to explain the post-break OIR slope as being shallower due to SN+Host... Can we say anything on host galaxy?}




\subsection{An on-axis structured shallow jet }
\label{sec: scenario2}
The similar break time between the OIR and X-rays is suggestive of an achromatic break, which suggests an origin based on the jet dynamics rather than a characteristic frequency passing through an observed band. 
{\bf PB: What about the spectral slope before and after the break? Are they consistent with no spectral break passage?} 
One common origin for an achromatic break is the so-called jet-break \cite{Rhoads1999,Sari1999}.  

Following \cite{BGG2020} Table 4, we can compute the change in slope due to an on-axis non-spreading, tophat jet. 
%These slopes provide a lower limit to the post jet-break slope given that a spreading jet can be significantly steeper with $\alpha\lesssim-p$ \textcolor{red}{Rhoads 1999}. 
The change in slope is provided by $\alpha_d-\alpha_f$, where $\alpha_f$ is the slope with no lateral spreading and thus a lower limit on the steepness of the post-break decay. The change in slope is independent of $p$ with $\Delta\alpha=\alpha_d-\alpha_f=(3-k)/(4-k)$. %This is the same change in slope for PLS D, G, and H...
This requires an incredibly steep $k\approx2.8$ to be consistent with the X-ray observations, and does not explain the larger change in slope of the OIR data. As we will show below, the value of $\Delta \alpha$ can be significantly reduced for a jet with a shallow angular structure of the kinetic energy.

The standard assumption that GRB jet's have a constant energy $dE_k/d\Omega$ within the core of the jet is likely an oversimplification (\textcolor{red}{CITE simulations?}), and a structured jet naturally arises as the GRB breaks out of its stellar environment. Therefore, we consider a GRB jet with a shallow broken power-law structure defined by %$dE_k/d\Omega\propto \Theta^{-a_1}$ for $\theta<\theta_{\rm c}$ and $dE_k/d\Omega\propto \Theta^{-a_2}$ for $\theta>\theta_c$ {\bf PB: It is probably better to have the above expression as a proper equation. Please add that when you can.}
\begin{align}
    dE_k/d\Omega\propto \Theta^{-a_1}\;\textrm{for}\;\theta<\theta_{\rm c} \\
    dE_k/d\Omega\propto \Theta^{-a_2}\;\textrm{for}\;\theta>\theta_c
\end{align}
where $\Theta=\sqrt{1+(\theta/\theta_c)^2}$ {\bf PB: and $a_1,a_2\lesssim 2$ (see ... for an exact limit for the applicability of this scenario)}. In this case, the flux and frequency evolution is dictated by the jet-structure, leading to a shallow angular structure dominated emission (sASDE) phase (see Tables 1 and 2 of) \cite{BGG2022}. %In this case, the \textcolor{purple}{change in slope due to a jet-break} is computed using \cite{BGG2022} Table 2 as $\Delta\alpha=\alpha_d-\alpha_s$. 
The flux evolution {\bf PB: is initially the same as for a spherical outflow with an isotropic equivalent energy given by the value along the line of sight. This lasts up to a time, $t_{\rm sph}$ \cite{BGG2022} when the Lorentz factor along the line of sight has decelerated to $\theta_{\rm obs}^{-1}$. After this time the flux evolves as}
in this regime is \cite{BGG2022}: \textcolor{red}{add the Ekin dependence as an equation to make it clear how these are derived? simplify eqns 10-11 for k=0 for simplicity of reading them. note for a=0, i.e., tophat jet, they simplify to the standard equations...}
\begin{align}
\label{eqn2}
    &F_{\nu,\textrm{G}}\propto  t^{-\frac{(a_1+6)kp+(a_1-2)(5k-12)-24p}{4(a_1+2k-8)}} \:\textrm{for}\:\nu_m<\nu<\nu_c \\
    &F_{\nu,\textrm{H}}\propto  t^{\frac{-a_1kp-2a_1k+8a_1-6kp+4k+24p-16}{4(a_1+2k-8)}} \:\textrm{for}\:\nu_c<\nu,
  %  &\nu_c \propto t^{\frac{(a-2)(3k-4)}{2(a+2k-8)}} \\
  %  &\nu_m\propto  t^{-3/2-\frac{a(k-3)}{2(a+2k-8)}}.
\end{align}
where the microphysical parameter dependence is identical to Equation \ref{eqn1} and we have not included IC corrections. 
{\bf This phase lasts until $t_{\rm c}$ which is the time at which $\Gamma(\theta_c)=\theta_c^{-1}$. After this time, the flux evolves in a similar way to the expressions given in \ref{eqn2}, but with $a_2 \rightarrow a_1$.}

{\bf PB: It might be a good idea to give the expression for $\Delta \alpha$ in this case, since you discuss it above for the steep jet case. This will be a natural way to lead to the discussion below.}
For an initial power-law slope of $a_1=0.6$ which steepens to $a_2=1.1$ after $\sim$\,1 d, we can identify a solution that fits the X-ray and OIR data.
Here, we have assumed that $\nu_m<\nu_\textrm{OIR}<\nu_c<\nu_X$ such that the X-rays and OIR lie on separate power-law segments. This naturally explains the different post-break slopes (Figure \ref{fig: lightcurve}). 
%\nu_m<\nu_\textrm{OIR}<\nu_c<\nu_X$ 
We find an adequate solution for $p=2.2$ and $k=0$, which yields initial pre-break slopes of  $\alpha_\textrm{\textrm{OIR},1}=-1.2$ and $\alpha_{X,1}=-1.4$, which steepen to $\alpha_\textrm{\textrm{OIR},2}=-1.45$ and $\alpha_{X,2}=-1.6$ after $\sim$\,1 d. This provides a good agreement with the observations (Figure \ref{fig: shallowjetlightcurve}). \textcolor{purple}{While these slopes provide a good qualitative description of the data, we find that adding even a slight microphysical parameter time dependence of $\varepsilon_B\propto t^{0.2}$ can create an even better agreement.} {\bf PB: Perhaps a more natural way to improve slightly the fit, is to make the structure even more gradually evolving with $\theta$ (e.g. $E_{\rm iso}\propto \theta^0$ below some $\theta_*$, transitioning to $E_{\rm iso}\propto \theta^{a_1}$ above that and continuing as described above at greater angles still.}

\textcolor{purple}{To add: solving for some parameters using constraints on nuc,num etc... Also need nua...}

%Here, we have assumed that $\nu_m<\nu_\textrm{OIR}<\nu_c<\nu_X$ such that the X-rays and OIR lie on separate power-law segments. This naturally explains the different post-break slopes (Figure \ref{fig: lightcurve}). We find an adequate solution for $p=2.2$, $k=0$, and $a=1$, which yields pre-jet break slopes of  $\alpha_\textrm{\textrm{OIR},1}=-0.9$ and $\alpha_{X,1}=-1.15$. The post-break slopes are then $\alpha_\textrm{\textrm{OIR},2}=-1.45$ and $\alpha_{X,2}=-1.6$, which is agreement with the observations (Figure \ref{fig: lightcurve}).

%This scenario easily explains the post-break slopes of both the X-rays and OIR, but instead does not explain the early X-ray slope. This may be explained by an early excess emission due to IC at $<0.5$ d. A bright IC emission component may be expected given the long-lived GeV emission detected by \textit{Fermi} LAT (\textcolor{red}{CITE}). %, but this would also lead to a large $Y$ parameter, impacting the equations used to reach these conclusions. 
%Moreover, in this case we have some trouble to re-produce the spectral evolution of the X-rays and the different slopes for the initial XRT and BAT data, which $\beta_\textrm{XRT}-\beta_\textrm{BAT}\approx 0.5$. 





%X-rays: $=(2 - 3 p)/4$ to $\alpha_{s,H}=\frac{-akp - 2 ak + 8 a - 6 kp + 4 k + 24 p - 16}{4(a + 2 k - 8)}$
%OIR: $\alpha_{s,G}= -\frac{(a + 6) kp + (a - 2) (5 k - 12) - 24 p}{4 (a + 2 k - 8)}$



%\textcolor{purple}{Can the excess be external IC of the RS? consistent with cutoff frequency? For a cutoff frequency of $\sim10^{13}$ Hz at $\sim0.2$ d would require $\gamma_c\approx 100$ at 5-10 hr after the GRB for IC to peak at 1 keV ($\gamma_c^2\nu_\textrm{cut}\approx1$ keV), but does not explain why it would be a narrow-band phenomena not impacting the OIR. But this also depends on the strength of the IC, which needs to be considered. }

%\textcolor{red}{An alternative solution is that both X-ray and OIR lie on same PL segment initially, x-rays have cooling break at similar time as jet-break but as this also requires RS and peak frequency passage in OIR it just doesn't seem as practical...}


%\subsubsection{Broken power-law jet structure}

%\textcolor{blue}{Add/refine text on shallow jet.}

%The standard assumption that GRB jet's have a constant energy $dE_k/d\Omega$ within the core of the jet is likely an oversimplification (\textcolor{red}{CITE simulations?}), and a structured jet naturally arises as the GRB breaks out of its stellar environment.  Therefore, we consider a GRB jet with a power-law energy structure $dE_k/d\Omega\propto \Theta^{-a}$ where $\Theta=\sqrt{1+(\theta/\theta_c)^2}$. 

%For an initial power-law slope of $a_1=0.6$ which steepens to $a_2=1.1$ after $\sim$\, 1 d, we can identify a solution that fits the X-ray and OIR data. Using $k=0$, $p=2.2$ and $\nu_m<\nu_\textrm{OIR}<\nu_c<\nu_\textrm{X}$, we obtain initial slopes $\alpha_\textrm{\textrm{OIR},1}=-1.2$, $\alpha_{X,1}=-1.4$, which steepen to  $\alpha_\textrm{\textrm{OIR},2}=-1.45$ and $\alpha_{X,2}=-1.6$ after $\sim$\,1 d. \textcolor{purple}{While these slopes provide a good qualitative description of the data, we find that adding even a slight microphysical parameter time dependence of $\varepsilon_B\propto t^{0.2}$ can create an even better agreement.} 


\begin{figure} 
\centering
\includegraphics[width=\columnwidth]{figs/GRB221009A_lc_shallowjet.pdf}
\caption{Multi-wavelength lightcurve of GRB 221009A. The dashed lines are determine using the structured jet model outlined in \S \ref{sec: scenario2}, and provide a good description of the X-ray and OIR data. 
}
\label{fig: shallowjetlightcurve}
\end{figure}

\begin{figure} 
\centering
\includegraphics[width=0.5\columnwidth]{figs/GRB221009A_SED_figure_shallowjet.pdf}
\includegraphics[width=0.5\columnwidth]{figs/GRB221009A_SED_figure_shallowjet_noradio.pdf}
\caption{Multi-epoch OIR and X-ray SEDs of GRB 221009A in the structured jet scenario.}
\label{fig: shallowjetSED}
\end{figure}


\subsubsection{Energetics}
%\textcolor{blue}{Text from Paz - use $E_{\gamma,\textrm{iso}}=2\times 10^{52}$. }
{\bf PB: A big advantage of the shallow structure jet scenario suggested above, is that it significantly reduces the energetic requirements relative to steep structure models. [Brendan, what is the earliest time at which we can confidently say the lightcurve evolves in the fashion that matches $a_1$? This will be used to determine an upper limit on $t_{\rm sph}$ and in turn $\theta_{\rm obs}$.] }

{\bf PB: As mentioned in \S \ref{sec: scenario2}, the viewing angle to the burst is directly related to $t_{\rm sph}$. Observationally, the latter is given by the time at which the evolution of the OIR lightcurve transitions to the ... slope and the X-ray to ... We find that $...<t_{\rm obs}<...$ [Brendan, please fill in those numbers]. The result is
\begin{equation}
    \theta_{\rm obs}=\left(\frac{(3-k)E_{\rm kin,iso}(\theta_{\rm obs})}{4\pi A 2^{3-k} c^{5-k}}\right)^{\frac{1}{2k-8}}t_{\rm sph}^{\frac{3-k}{8-2k}}
\end{equation}
which for $k=0$ (as favoured by the lightcurve evolution) implies $...<\theta_{\rm obs}<...$.
An additional angle of importance for the considered structure is $\theta_{\rm c}>\theta_{\rm obs}$ (below which $E_{\rm kin,iso}$ evolves as $\theta^{a_1}$ and above which as $\theta^{a_2}$). Since for a shallow structured jet, the observed angle at any given time evolves with time according to
\begin{eqnarray}
    \theta\!=\!\theta_{\rm obs}\left\{ \begin{array}{ll}(t/t_{\rm sph})^{\frac{3-k}{8-2k-a_1}} & t_{\rm sph}<t<t_{\rm c} ,\\ \\(t_{\rm c}/t_{\rm sph})^{\frac{3-k}{8-2k-a_1}}(t/t_{\rm c})^{\frac{3-k}{8-2k-a_2}}  \quad  & t>t_{\rm c}
\end{array} \right.
\end{eqnarray}
Therefore, $t_{\rm c}$ can be expressed as,
\begin{equation}
    \theta_{\rm c}=\left(\frac{(3-k)E_{\rm kin,iso}(\theta_{\rm obs})}{4\pi A 2^{3-k} c^{5-k}}\right)^{\frac{1}{2k-8+a_1}}t_{\rm c}^{\frac{3-k}{8-2k-a_1}}\theta_{\rm obs}^{\frac{-a_1}{8-2k-a_1}}
\end{equation}
Finally, using $\theta_{\rm obs}, \theta_{\rm c}$, we can express the required (collimated-corrected) energy in the jet considering that no steep break (i.e. traditional jet-break like) has been observed in the lightcurve up to the latest time of observation
\begin{eqnarray}
  &  E_{\rm t}=\frac{\theta(t)^2}{2} E_{\rm kin, iso}(\theta_{\rm obs}) \left(\frac{\theta_{\rm c}}{\theta_{\rm obs}}\right)^{-a_1}\left(\frac{\theta(t)}{\theta_{\rm c}}\right)^{-a_2} %\\
%  &=\frac{1}{2}E_{\rm \gamma,iso}(\theta_{\rm obs}) \theta_{\rm obs}^{\frac{6a_1}{8-a_1}} t_{\rm c}^{\frac{6-3a_1}{a_1-8}-\frac{6-3a_2}{a_2-8}} t^{\frac{6-3a_2}{a_2-8}}
\end{eqnarray}
for $k=0, a_1=0.6, a_2=1.1$, this leads to
\begin{eqnarray}
& E_{\rm t}=4.7\times 10^{52}\mbox{ erg}\left(\frac{E_{\rm \gamma,iso}(\theta_{\rm obs})f(\eta_{\gamma})}{10^{54.5}\mbox{ erg}}\right)^{0.81} \nonumber \\ & \left(\frac{\theta_{\rm obs}}{0.01}\right)^{0.49}  \left(\frac{t_{\rm c}}{0.6\mbox{ d}}\right)^{0.18} \left(\frac{t}{80\mbox{ d}}\right)^{0.39}
\end{eqnarray}
We see that the required energy is more than an order of magnitude smaller than in the standard jet case. Furthermore, notice the shallow increase in the required energy in this shallow jet scenario as a function of time. In other words, the longer no steep jet break is seen in the lightcurve, the greater the difference between the two energy estimates becomes. 
}

%\begin{equation}
%t_{j}= \Big[ \frac{ (3-k) \epsilon_c}{A^{5-k}}\Big]^{1/(3-k)} \theta_c^{(8-2k)/(3-k)},
%\end{equation}
%where $\epsilon_c$ is $dE/d\Omega$ at the jet core and A is defined such that $\rho=A r^{-k}$. \textcolor{purple}{What about gamma-ray efficiency?}






% \textcolor{red}{I think nu_KN is actually indpendent of Gamma...}
%The second constraint is due to the steep slope of \textit{Swift} BAT at $1$ hr. The value of $\Delta\beta_X=0.46\pm0.07$ between XRT and BAT is larger than the change in spectral slope due to Klein-Nishina suppression ($\nu_m<\nu_\textrm{KN}<\nu_c$) where $\Delta\beta_\textrm{KN}=0.3$ for $p=2.2$. Following \cite{Beniamini2015}, we can compute the Klein-Nishina frequency as $\nu_\textrm{KN}\leq\Gamma m_e c^2/(h(1+z)\gamma_m$, where $h$ %$h=H_0/100$ is Planck's constant. We require that $\nu_\textrm{KN}>150$ keV at 0.05 d, which leads to \textcolor{red}{$\Gamma>XXX$} where we have used that $\nu_ma\approx2\times10^{16}$ at 0.05 d, according to our first interpretation (see \S \ref{sec: scenario1}). 



\subsubsection{Rate of events}

\textcolor{blue}{Text from Paz/Yoni - why shallow jets might be more commonly associated with more energetic events.}




\subsubsection{Comparison to other GRBs}

\textcolor{purple}{Need to compare to GRB 130427A... (bright, nearby, lack of jet-break etc). This could also go in the energetics/jet-break section...} 

\textcolor{purple}{What were the GRBs that Simone found? Should they be added to the XRT lightcurve figure showing all long GRBs?}

\begin{figure} 
\centering
\includegraphics[width=0.5\columnwidth]{figs/Figure_6.png}
\includegraphics[width=0.5\columnwidth]{figs/Fermi_hist_221009A_2.pdf}
\caption{Rest-frame afterglow lightcurves in the \textit{Swift} XRT $0.3-10$ keV energy band for a sample of bright long-duration GRBs. 
}
\label{fig: bright_xrt_lightcurve}
\end{figure}

\section{Conclusions}
\label{sec: conclusions}

We have presented an in-depth analysis of the early afterglow of GRB 221009A. \textcolor{purple}{Continue... focus on the observations and speculate as to why they do not work...}

\textcolor{purple}{Need discussion of rates and energetics and focus on this being bright not just because nearby but because one of the most luminous GRBs ever. What do we learn from these bright GRBs which do not have clear jet-breaks? Why are they different? What does a wide jet mean for energetics and RATE? What did we learn from this GRB?}

\textcolor{purple}{need to explain why energy so high
and 
why are Gev bright bursts not showing clear jet-breaks. why jet so wide or structure so shallow compared to garden-variety GRBs.
Paz mentioned hydrodynamic jets are shallower than magnetohydrodynamic and more energetic hydrodynamic jets have shallower energy distributions...}



\acknowledgments

This work made use of data from the NuSTAR mission, a project led by the California Institute of Technology, managed by the Jet Propulsion Laboratory, and funded by the National Aeronautics and Space Administration.  
Based on observations obtained with XMM-Newton, an ESA science mission with instruments and contributions directly funded by ESA Member States and NASA. 
Based on observations obtained with MASTER, MASTER equipment is supported by the Development Program of Lomonosov MSU. 
Based on observations obtained at the international Gemini Observatory, a program of NSF's OIR Lab, which is managed by the Association of Universities for Research in Astronomy (AURA) under a cooperative agreement with the National Science Foundation on behalf of the Gemini Observatory partnership: the National Science Foundation (United States), National Research Council (Canada), Agencia Nacional de Investigaci\'{o}n y Desarrollo (Chile), Ministerio de Ciencia, Tecnolog\'{i}a e Innovaci\'{o}n (Argentina), Minist\'{e}rio da Ci\^{e}ncia, Tecnologia, Inova\c{c}\~{o}es e Comunica\c{c}\~{o}es (Brazil), and Korea Astronomy and Space Science Institute (Republic of Korea). 

The \textit{HST} data used in this work was obtained from the Mikulski Archive for Space Telescopes (MAST). STScI is operated by the Association of Universities for Research in Astronomy, Inc., under NASA contract NAS5-26555. Support for MAST for non-\textit{HST} data is provided by the NASA Office of Space Science via grant NNX09AF08G and by other grants and contracts. 
These results also made use of Lowell Observatory's Lowell Discovery Telescope (LDT), formerly the Discovery Channel Telescope. Lowell operates the LDT in partnership with Boston University, Northern Arizona University, the University of Maryland, and the University of Toledo. Partial support of the LDT was provided by Discovery Communications. LMI was built by Lowell Observatory using funds from the National Science Foundation (AST-1005313). 
This work made use of data supplied by the UK \textit{Swift} Science Data Centre at the University of Leicester. 

This research has made use of the XRT Data Analysis Software (XRTDAS) developed under the responsibility of the ASI Science Data Center (ASDC), Italy. 
This research has made use of the NuSTAR Data Analysis Software (NuSTARDAS) jointly developed by the ASI Space Science Data Center (SSDC, Italy) and the California Institute of Technology (Caltech, USA). 
This research has made use of data and/or software provided by the High Energy Astrophysics Science Archive Research Center (HEASARC), which is a service of the Astrophysics Science Division at NASA/GSFC. 
%We additionally made use of Astropy, a community-developed core Python package for Astronomy \cite{astropy}.

%Based on data obtained from the ESO Science Archive Facility under request number \#639813.
    %acknowledge all instruments used properly!!

%% To help institutions obtain information on the effectiveness of their 
%% telescopes the AAS Journals has created a group of keywords for telescope 
%% facilities.
%
%% Following the acknowledgments section, use the following syntax and the
%% \facility{} or \facilities{} macros to list the keywords of facilities used 
%% in the research for the paper.  Each keyword is check against the master 
%% list during copy editing.  Individual instruments can be provided in 
%% parentheses, after the keyword, but they are not verified.

\vspace{5mm}
\facilities{\textit{Swift}, \textit{NuSTAR}, \textit{XMM-Newton}, \textit{HST}, LDT, Gemini, MASTER}

%% Similar to \facility{}, there is the optional \software command to allow 
%% authors a place to specify which programs were used during the creation of 
%% the manuscript. Authors should list each code and include either a
%% citation or url to the code inside ()s when available.

\software{\texttt{HEASoft 6.29c}, \texttt{XRTDAS}, \texttt{NuSTARDAS}, \texttt{SAS}, \texttt{Dragons}, \texttt{XSPEC v12.11.0} \cite{Arnaud1996}, \texttt{IRAF} \cite{Tody1986}, \texttt{SExtractor} \cite{Bertin1996}, \texttt{Swarp} \cite{Bertin2010}, \texttt{SCAMP} \cite{Bertin2006}, \texttt{Astropy} \cite{astropy}
}

%% Appendix material should be preceded with a single \appendix command.
%% There should be a \section command for each appendix. Mark appendix
%% subsections with the same markup you use in the main body of the paper.

%% Each Appendix (indicated with \section) will be lettered A, B, C, etc.
%% The equation counter will reset when it encounters the \appendix
%% command and will number appendix equations (A1), (A2), etc. The
%% Figure and Table counter will not reset.


==> oldcuttext.tex <==
\textcolor{purple}{Title 2:} 
A wide shallow jet explains GRB 221009A\\
\textcolor{purple}{Title 3:} 
A structured jet to explain the extreme GRB 221009A \\
\textcolor{purple}{Title 4:} 
The long-lived afterglow of GRB221009A (something more empirical and less model dependent)\\
\textcolor{purple}{Title 5:} 
GRB 221009A Afterglow Observations Constrain Its Jet Structure\\
\textcolor{purple}{Title 6:} 
GRB 221009A Afterglow Observations Suggest a Shallow Wide Jet \\ 
\textcolor{purple}{Title 7:}
The long-lived afterglow of GRB 221009A is explained by a shallow structured jet\\
\textcolor{purple}{Title 8:}
The long-lived afterglow of GRB 221009A: evidence for a shallow structured jet\\
\textcolor{purple}{Title 9:}
The long-lived afterglow of GRB 221009A reveals a shallow structured jet\\
\textcolor{purple}{Title 10:}
Multi-wavelength afterglow observations of GRB 221009A reveal a shallow structured jet\\
\textcolor{blue}{I prefer Titles 1, 9, or 10, but do not feel strongly that the others are not equally as acceptable. None stands out to me as the best; though 9 or 10 in which I combined the other ideas seem good to me.}\\ 
\textcolor{red}{I have only received votes for Title 1. (Alexander, Mike, Igor, Rosa, Brad, Erica, Carlos, Roberto, Myself). All comments beyond just saying ``title 1'' have been forwarded to you. }
}

